Detecting Data Errors with Statistical Constraints

A powerful approach to detecting erroneous data is to check which potentially dirty data records are incompatible with a user's domain knowledge. Previous approaches allow the user to specify domain knowledge in the form of logical constraints (e.g., functional dependency and denial constraints). We extend the constraint-based approach by introducing a novel class of statistical constraints (SCs). An SC treats each column as a random variable, and enforces an independence or dependence relationship between two (or a few) random variables. Statistical constraints are expressive, allowing the user to specify a wide range of domain knowledge, beyond traditional integrity constraints. Furthermore, they work harmoniously with downstream statistical modeling. We develop CODED, an SC-Oriented Data Error Detection system that supports three key tasks: (1) Checking whether an SC is violated or not on a given dataset, (2) Identify the top-k records that contribute the most to the violation of an SC, and (3) Checking whether a set of input SCs have conflicts or not. We present effective solutions for each task. Experiments on synthetic and real-world data illustrate how SCs apply to error detection, and provide evidence that CODED performs better than state-of-the-art approaches.

==> consistency-long-oct18.tex <==
\section{Consistency Checking} \label{cck}

\oliver{Jiannan's plan. Move this to end. How about we make a final section on repair? This is like the paper on conditional functional dependencies. Then we can a) discuss repair systems (like Holoclean) and b) discuss consistency checking and whether it's important.} 

%We further study two properties of Statistical Constraints, and one fundamental problem associated with Statistical Constraints.
In this section, we first define and motivate the consistency checking problem, then discuss different approaches for different use cases.
%based on the well-known Graphoid Axioms~\cite{pearl2}, and then propose a consistent-checking algorithm. 
%Unfortunately, the algorithm has an exponential time complexity. We 
Intuitively, if a set of \SCs $\Sigma$ is consistent, it means that $\Sigma$ has no conflict. That is, there exists a joint distribution that satisfies $\Sigma$. Definition~\ref{def:consistency} presents a formal definition.

\begin{Definition}[Consistency]\label{def:consistency}
Given a set $\Sigma$ of \SCs, let $\set{V}$ denote the set of random variables that appear in $\Sigma$. The consistency problem is to determine whether there exists a joint distribution $P(\set{V})$ that satisfies every \SC in $\Sigma$. 
\end{Definition}


\begin{figure}[t]
   \centering 
   \includegraphics[width=0.9\linewidth]{fig/joint-new.pdf} 
   \vspace{-1em}
   \caption{An example of a joint distribution that satisfies $\Sigma = \{A \indep B,\; A \nindep B| C\}$}\label{fig:joint}\vspace{-1.5em}
\end{figure}

For example, consider $\Sigma = \{A \indep B,\; A \nindep B| C\}$. Since there are three random variables in $\Sigma$, we have $\set{V} = \{A, B, C\}$. As shown in Figure~\ref{fig:joint}, we can construct a joint distribution $P(A, B, C)$ that satisfies $\Sigma$, thus $\Sigma$ is consistent. If we are given $\Sigma' = \{A \indep B,\; A \nindep B\}$, it is impossible to construct a joint distribution that satisfies $\Sigma'$, thus $\Sigma'$ is inconsistent. 

Assuming that the user has in mind a consistent set of constraints, with an inconsistent set of constraints, one or more of the constraints must contradict the user's domain knowledge. A consistency checking method is therefore useful for the interactive setting because it helps catch misspecifications \cite{function-dependency}. In the automatic setting, if the constraints are not consistent, %when applying it to error detection, 
checking the constraints against the data will lead to contradictory error-detection results, where some constraint is violated regardless of what the data are. 
%Being able to check whether a given set $\Sigma$ of \SCs is consistent or not is important because 



\subsection{Mixed-Initiative Consistency Checking} The assumptions correspond to different ways of eliciting the constraints, as discussed above in Section~\ref{subsec:sc-discovery} above presented different ways of interacting with the user to elicit statistical constraints. We describe corresponding consistency-checking methods. 


\paragraph{Constraints represented by a complete model.} In Section~\ref{subsec:sc-discovery}, we described methods for representing the user's domain knowledge in a complete model that incorporates known statistical constraints. An attractive feature of the model-specification approach is that the incorporated constraints are {\em guaranteed to be consistent} because the elicited model defines a probability distribution $P(\set{V})$ that satisfies the constraints.

\paragraph{Saturated CI statements}  In the case where the given CI constraints are saturated and elementary,
%meaning that they connect exactly two variables $\Xvariable$ and $\Yvariable$, 
Heckerman et al. show that a set of CIs is consistent if and only if it satisfies symmetry \cite{heckerman}. This is easy to check for a user or an algorithm.

\paragraph{General CI statements: Interactive Inconsistency Resolution} 

Consider the interactive use of \system as shown in Figure~\ref{fig:coded}. We can expect that one of the effects of the interaction between user and data is to correct the constraints that contradict the user's domain knowledge, for the following reason: Consider such an erroneous constraint. Following the example of Figure~\ref{fig:sc-discovery}, suppose the user has correctly specified the independence constraint $\textsf{Color} \indep \textsf{Model}$ and erroneously specified the dependence constraint $\textsf{Color} \nindep \textsf{Model}$. If the data contradict the erroneous constraint, the user will review the constraint carefully, and we can expect her to remove the constraint rather than modify the data. For example, if the data indicate that $\textsf{Color} \nindep \textsf{Model}$ does not hold, we can expect the user to reconsider and remove this constraint. If the data do not contradict the erroneous constraint, they will instead contradict a true constraint. Again the user can be expected to review the true constraint carefully, and use drill-down analysis to repair the data. The repaired data will be consistent with the true constraint, hence inconsistent with the false constraint, which will be reconsidered and removed. For example, if the data indicate that $\textsf{Color} \nindep \textsf{Model}$ holds, then they contradict the true constraint $\textsf{Color} \indep \textsf{Model}$. Using drill-down analysis, the user can repair the dirty data so that $\textsf{Color} \indep \textsf{Model}$, and therefore $\textsf{Color} \nindep \textsf{Model}$ will be removed. We next consider consistency checking in the automated setting where the user is not available to correct constraints or repair data. The complete model and saturated CI statement cases are trivial and easy, respectively, to check for an algorithm. We therefore focus on automated methods for the general CI case.





\subsection{Algorithmic Consistency Checking} \label{subsec:consistency}

Algorithmically determining the consistency of general CI statements is a very difficult problem; it is not even known whether it is decidable \cite{niepert}. Nonetheless, because of the importance of CI statements, AI researchers have developed a number of heuristic approaches~\cite{pearl2, niepert, studeny}. A principled approach is to use an \textbf{inference framework}~\cite{pearl2}: first divide $\Sigma$ into two disjoint sets $\mathcal{I}$ and $\mathcal{D}$, where $\mathcal{I}$ (resp. $\mathcal{D}$) represents the set of independence (resp. dependence) statements in $\Sigma$. For each $\lambda \in \mathcal{D}$, it checks whether $\mathcal{I}$ implies $\lnot \lambda$. If the answer is no for all $\lambda$, then $\Sigma$ is consistent; otherwise, it is not consistent. The correctness of the framework was proved in~\cite{pearl2}.\oliver{what does "correctness" mean? If no contradiction is entailed, then the set is consistent?} For example, consider $\Sigma = \{A \indep B,\; A \nindep B| C\}$. We have $\mathcal{I} = \{A \indep B\}$  and $\mathcal{D} = \{A \nindep B| C\}$. We can see that $\mathcal{D}$ does not imply  $\lnot \lambda = A \indep B| C$, thus $\Sigma$ is consistent. A similar approach of iteratively inferring new constraints from previous ones is used to check the consistency of a set of functional dependencies \cite{bohannon2007conditional}. 
%Whereas the consistency of CIs has received extensive attention by AI researchers \cite{pearl-G, niepert, studeny}, the general problem is very difficult; it is not even known  We therefore consider methods for different assumptions about the set of statistical constraints. 


To apply the implication framework,\oliver{should that be "entailment"? Check Niepert}
%to solve the problem in Definition~\ref{def:consistency}, the key challenge is how to efficiently check whether $\mathcal{I}$ implies $\lnot \lambda$ or not.  In other words, 
we aim to determine whether an independence \SC $\gamma$ can be inferred from $\mathcal{I}$ using $\mathcal{G}$.  Definition~\ref{def:implication} formally defines the implication problem. 

\begin{Definition}[Implication]\label{def:implication}
Given a set $\mathcal{I}$ of independence \SCs, and another independence \SC $\gamma$, the implication problem is to determine whether $\gamma$ can be inferred from $\mathcal{I}$ using $\mathcal{G}$, i.e., check whether $\mathcal{I} \vdash_{\mathcal{G}} \gamma$ holds or not.
\end{Definition}

\paragraph{Inferring \SCs} We propose an iterative algorithm. The algorithm starts with $\mathcal{I}^* = \mathcal{I}$, and then iteratively expands $\mathcal{I}^*$ with new \SCs. At each iteration, the algorithm checks which inference rule in $\mathcal{G}$ can be used to generate a new \SC, and then adds it to $\mathcal{I}^*$. The algorithm terminates when $\mathcal{I}^*$ cannot be further expanded. After that, the algorithm checks whether $\gamma \in \mathcal{I}^*$ holds. If so, then $\mathcal{I}$ implies  $\gamma$; otherwise, $\mathcal{I}$ does not imply $\gamma$. An inference system consists of  a collection of inference rules, where each rule is in the form of 
\[\SC_1 ~~\&~~ \SC_2 \cdots ~~\&~~ \SC_n \quad \Longrightarrow \quad \SC_{new},\]
which states that if the left-hand side \SCs hold, then the right-hand side \SC must hold. 
%Having an inference system is essential to solve the consistency problem. 

\paragraph{Consistency Checking by Implication} \oliver{need to settle terminology: inference or implication or entailment?} We can develop a consistency-checking algorithm using the implication algorithm. See the pseudo-code in Algorithm~\ref{alg:check}. The algorithm first computes $\mathcal{I}^*$. Then, for each $\lambda \in \mathcal{D}$, it checks whether $\lnot\lambda \in \mathcal{I}^*$ holds or not. If no for all $\lambda$, then $\Sigma$ is consistent; otherwise, $\Sigma$ is inconsistent. 

For example,  suppose we are given three constraints:
\[\Sigma = \{\SC_1:  A \indep B, ~~~~\SC_2:  A \indep C | B, ~~~~\SC_3: A \nindep C\}.\] 
Applying the rule (see Definition~\ref{def:new-inference}):
\[(A \indep B) \quad  \&  \quad  (A \indep C | B) \quad  \Longrightarrow \quad A \indep C,\]
shows that $\Sigma$ is inconsistent because $\SC_1$ and $\SC_2$ imply $\neg \SC_3$. 

%there exists $\lambda \in \mathcal{D}$ such that $\lnot\lambda \in \mathcal{I}^*$, it means that $\mathcal{I}$ implies $\lnot\lambda$. Since $\lambda \in \mathcal{D}$, then $\Sigma$ is inconsistent. If there does not exist $\lambda  \in \mathcal{D}$ such that $\lnot\lambda \in \mathcal{I}^*$, then $\Sigma$ is consistent. 
% \na{To JN: do we need the pseudo-code algorithm for this?}


\begin{algorithm}[t]
	\caption{Consistency-checking By Implication}\label{alg:check}
	\KwIn{A set of \SCs: $\Sigma$}
	\KwOut{Consistent or not (YES or NO)}
	\vspace{0.5em}
	Divide $\Sigma$ into $\mathcal{I}$ and $\mathcal{D}$\;
	Use the implication algorithm to obtain $\mathcal{I}^*$\;
	\For{$\lambda \in \mathcal{D}$}
	{
	    \If{$\lnot \lambda \in \mathcal{I}^*$}
	    {
	        {\bf return} NO\; 
	    }
	}
	{\bf return} YES\;
\end{algorithm}

 \paragraph{Resolving Inconsistency in the interactive setting} Once an inconsistency is derived by implication, we help the user to resolve the inconsistency.  Specifically, suppose the consistency-checking algorithm finds a conflict: $\mathcal{I}$ implies $A \indep B$ but $A \nindep B$ is in $\Sigma$. We ask the user to check which one is correct. If the former is correct, then $A \nindep B$ should not be in $\Sigma$, and we remove $A \nindep B$ from $\Sigma$. Otherwise, we show the derivation of $A \indep B$  from $\mathcal{I}$ and then ask the user to remove the incorrect \SCs involved in the derivation. In the automated setting, a failed consistency check can be used to stop the system from relying on the inconsistent \SCs for error detection. The implication approach requires an inference system for CIs, which we describe in the next subsection. 
 
% Before applying \SCs to error detection, we need to investigate a number of basic properties of \SCs. In this section, we first present an inference system for \SCs, and then study two fundamental properties associated with \SCs: (1) \emph{Consistency}: whether a set of \SCs have conflicts; (2) \emph{Implication}: whether a set of \SCs imply (entail) another \SC. %We first present an inference system for statistical constraints in Section~\ref{subsec:infer}, and then propose our solutions to the consistency and redundancy problems in Section~\ref{subsec:consistency} and Section~\ref{subsec:implication}, respectively.

% For the space of saturated CI statements only, Pearl and Geiger provide a sound and complete inference system known as system S \cite{pearl2}.

%  In the following, we first formally define the consistency problem, and then present a consistency-checking framework. In order to apply the framework, the key is to solve the implication problem. Therefore, we define the implication problem and propose an efficient implication algorithm. 
 

{\noindent \bf Completeness.} Algorithm~\ref{alg:check_graph} is sound since the system G is. However,  Therefore the system G is not complete, and neither is our algorithm. Niepert et al. propose a different system A, which is complete but not sound. They suggest applying both G and A to a given set of constraints, which allows a system to both falsify some cases of inconsistent CIs (via G) and validate some cases of consistent CIs (via A). We leave experimenting with system A for future work. 
%

% \subsection{A General Inference System for {\large \bf \SCs}}
% \label{subsec:infer}

% \paragraph{The general CI case} Geiger and Pearl~\cite{pearl2} proposed a framework to solve the consistency problem. They first divide $\Sigma$ into two disjoint sets $\mathcal{I}$ and $\mathcal{D}$, where $\mathcal{I}$ (resp. $\mathcal{D}$) represents the set of independence (resp. dependence) statements in $\Sigma$. For each $\lambda \in \mathcal{D}$, it checks whether $\mathcal{I}$ implies $\lnot \lambda$. If the answer is no for all $\lambda$, then $\Sigma$ is consistent; otherwise, it is not consistent. The correctness of the framework was proved in~\cite{pearl2}. For example, consider $\Sigma = \{A \indep B,\; A \nindep B| C\}$. We have $\mathcal{I} = \{A \indep B\}$  and $\mathcal{D} = \{A \nindep B| C\}$. We can see that $\mathcal{D}$ does not imply  $\lnot \lambda = A \indep B| C$, thus $\Sigma$ is consistent.    

%\oliver{can we add saturated CIs? That would be a significant generalization. - Jiannan says that no, because the G rules may turn saturated CIs into non-saturated ones} 




\subsubsection{Inference Systems  for CI statements}

A commonly used set of axioms is Geiger and Pearl's system $\mathcal{A}$~\cite{pearl2}.\oliver{check consistency of notation with Niepert}. \oliver{I suggest adding composition}


% Xu et al. develop  for DCs. A natural question is: can we develop a sound and complete inference system for \SCs? In the following, we first introduce some background knowledge about the well-known \emph{Graphoid Axioms}~\cite{pearl2}, and then present our inference system derived from the axioms. 


%{\noindent \bf Graphoid Axioms.} %In the Statistics field, 
%Geiger and Pearl~\cite{pearl2} showed that conditional independence statements satisfy the following  axioms.
%(inference rules).
%known as the \emph{Graphoid Axioms} $\mathcal{A}$. 

\begin{Definition}\label{def:graphoid-axioms}
Let $\set{X}$, $\set{Y}$, $\set{Z}$, and $\set{W}$ denote four disjoint sets of random variables. The \emph{graphoid Axioms} $\mathcal{A}$ are the following:

{\noindent \emph{Symmetry}}: 
\[\set{X} \indep \set{Y} \mid \set{Z}  \quad \Longleftrightarrow \quad  \set{Y} \indep \set{X} \mid \set{Z}\]

{\noindent \emph{Decomposition}}: 	
\[
\set{X} \indep \set{YW} \mid \set{Z}  \quad  \Longrightarrow \quad 
\begin{cases}
\set{X} \indep \set{Y} \mid \set{Z} \\
\set{X} \indep \set{W} \mid \set{Z}
\end{cases} 
\]

{\noindent \emph{Weak Union}}:
\[\set{X} \indep \set{YW} \mid \set{Z}  \quad \Longrightarrow  \quad \set{X} \indep \set{Y} \mid \set{ZW}\]

{\noindent \emph{Contraction}}:
\[\big (\set{X} \indep \set{Y} \mid \set{Z} \big ) ~~ \& ~~ \big (\set{X} \indep \set{W} \mid \set{YZ} \big ) \quad \Longrightarrow \quad  \set{X} \indep \set{YW} \mid \set{Z}\]

% {\noindent \emph{Intersection}}:
% \[\big (\set{X} \indep \set{Y} \mid \set{Z}\big )  ~~ \& ~~  \big (\set{X} \indep \set{W} \mid \set{Z}\big ) \quad \Longrightarrow \quad   \set{X} \indep \set{YW} \mid \set{Z}\]
\end{Definition}

\noindent Note that $\set{Z}$ can be the empty set.
%thus the above axioms also hold without $\set{Z}$. 
For example, for the symmetry axiom, we have $\set{X} \indep \set{Y}   \Longrightarrow \set{Y} \indep \set{X}.$ The system $\composition$ results from adding to $\mathcal{A}$ the composition principle:




\todo{need a new example}

\todo{should switch notation to X,Y,Z to be consistent}

% \begin{example}~\label{exa:implication}
% Given a set of independence \SCs $\mathcal{I} = \{A\indep B, A \indep C | B, B\indep C,  C \indep E | D\}$ over attributes $M=\{A, B, C, D, \\
% E\}$. To compute $\mathcal{I}^*$, we initially set $\mathcal{I}^* = \mathcal{I}$, and then apply the implication algorithm.

% \noindent {\underline{Step 1: Constructing Hash Table}}. $H=\{\{A,B\},\{B,C\}\}$ will be generated according to the marginal \SCs  in  $\mathcal{I}^*$, i.e., $A \indep B$ and $B \indep C $.

% \noindent {\underline{Step 2: Employing Inference System $\mathcal{G}$}}. We check each conditional \SC in $\mathcal{I}^*$. For $\SC_1:A \indep C | B $, we first check whether $\{A,B\}$ or $\{B,C\}$ exists. Obviously, we have both of them in the $H$. Applying the \emph{contraction-weak-union-decomposition} inference rule in $\mathcal{G}$, we can obtain three new \SCs: $A\indep B|C$, $B \indep C |A$, and $A \indep C$. We add them into $\mathcal{I}^*$, and hash $A \indep C$ as $\{A,C\}$ and add it into $H$. 

% \noindent {\underline{Step 3: Repeating}}. Repeat Step 1 and Step 2 till there are no more \SCs that can be inferred. In this example, we eventually arrive at $\mathcal{I}^* = \{A\indep B, A\indep C, B\indep C, A \indep B|C, A \indep C | B, B \indep C |A,  C \indep E | D\}$. 

% \end{example}

\paragraph{Soundness and Completeness.}
For existing row-oriented constraints, FDs have a sound and complete inference system that is known as Armstrong's Axioms~\cite{abiteboul1995foundations}. Wenfei et al. extend Armstrong's Axioms to CFDs and prove that the new inference system is also sound and complete~\cite{bohannon2007conditional} \oliver{but NP-hard?}. Unfortunately, inference for CI statements is a much harder problem: a major negative result due to Studeny is that no finite set of axioms is both sound and complete for general CIs \cite{studeny1990conditional}.  The system $\mathcal{A}$ is sound~\cite{pearl2}, but by Studeny's result, not complete. The situation for general CIs is thus comparable to that for DCs, where we currently have a set of sound (but not complete) inference rules~\cite{chu2013holistic}. 

% \vspace{.5em}

% {\noindent \bf A General Inference System for \SCs.} 


{\noindent \bf Time Complexity.} The implication algorithm needs $\mathcal{O}(|\mathcal{I}^*|)$ iterations, and each iteration needs $\mathcal{O}(|\mathcal{I}^*|)$ time. The total time complexity is $\mathcal{O}(|\mathcal{I}^*|^2) = \mathcal{O}((6|\mathcal{I}|)^2) = \mathcal{O}(|\mathcal{I}|^2)$. For the consistency-checking algorithm, the main bottleneck is spent in running the implication algorithm to compute $\mathcal{I}^*$ (see Line 2 in Algorithm~\ref{alg:check}), thus the total time complexity is $\mathcal{O}(|\mathcal{I}|^2)$.



\paragraph{Time Complexity for $\set{V}_k$ Inferences} We next show that the inference method based on system $\mathcal{A}$ is efficient if the number of variables that appear in any of the input \SCs is relatively small. More precisely, if $k$ is the maximum number of variables in any input \SC, the complexity is pseudo-polynomial in the parameter $k$.\footnote{Even more precisely, the time complexity is  $O(\sum_{m=0}^{k} \binom{m}{n} \times 3^m)$.}

To analyze the time complexity of the implication algorithm, we answer two  questions:\\
\indent \emph{Q1. What is the time complexity of generating a new \SC?} \\
\indent \emph{Q2. How many new \SCs can be generated in total?}

\vspace{0.25em}

\noindent For $Q1$, consider the two inference rules in Definition~\ref{def:new-inference}. The algorithm first checks whether the symmetry rule can be used to generate a new \SC or not. The time complexity of this process is $\mathcal{O}(|\mathcal{I}^*|)$. For the contraction-weak-union-decomposition rule, a naive way is to enumerate every pair of \SCs in $\mathcal{I}^*$ and then check whether the rule can be used or not. It needs $\mathcal{O}(|\mathcal{I}^*|^2)$ time. In fact, we can utilize a hash table to reduce the time complexity to $\mathcal{O}(|\mathcal{I}^*|)$. Specifically, we build a hash table for marginal \SCs (e.g., $A \indep B$), and then for each conditional \SC (e.g.,  $A \indep C | B$), we check whether $A \indep B$ or $C \indep B$ exists in the hash table. %This avoids $n^2$ comparisons. In total, our algorithm needs $\mathcal{O}(|\mathcal{I}^*|)$ time to generate a new \SC at each iteration.      

\vspace{0.25em}





\noindent For $Q2$, we seek to compute an upper bound for the number of newly generated \SCs. The key observation is that for any inference rule in $\mathcal{G}$, its right-hand side will not introduce any new variable that is not on the left-hand side. For example, consider the contraction-weak-union-decomposition rule. The left-hand side has three variables $\{A, B, C\}$, and the right-hand side has the same three variables, without introducing any new variable.      


% \na{TO JN: do we need to like say, this observation is the coverage problem like CFD and DC said. }

Based on this observation, we find that there is a relationship between $|\mathcal{I}|$  and $|\mathcal{I}^*|$. That is, $|\mathcal{I}^*| \leq 12 |\mathcal{I}|$. If we consider symmetry \SCs (e.g., $A \indep B$ and $B \indep A$) are the same, then $|\mathcal{I}^*| \leq 6 |\mathcal{I}|$.  We give the intuition below, and provide a formal proof in Lemma~\ref{lem:upper-bound}. 

We say $\SC_1$ \emph{covers} $\SC_2$ if the variable set of $\SC_1$ is a superset of the variable set of $\SC_2$. %For example, suppose $\SC_1: A \indep B$. The variable set of $\SC_1$ is $\{A, B\}$. Then, it covers two different \SCs:
%\[A \indep B, \;\; B \indep A.\]
%\na{I changed a little bit of the example here, is it right?}
%
For example, suppose $\SC_1: A \indep B | C$. Then, it covers 6 different \SCs:
\begin{align*}
A \indep B,\;\; A \indep C,\;\; B \indep C,\;\; A \indep B | C,\;\; A \indep C | B,\;\; B \indep C | A
\end{align*}
The above observation implies the \SCs in $\mathcal{I}$ can cover all the \SCs in $\mathcal{I}^*$. Since each $\SC \in \mathcal{I}$ can cover at most 6 different \SCs, then we have that $|\mathcal{I}^*| \leq 6 |\mathcal{I}|$. Lemma~\ref{lem:upper-bound} formally proves this result.


\begin{Lemma}\label{lem:upper-bound}
Given a set $\mathcal{I}$ of independence \SCs, let $\mathcal{I}^*$ denote the set of all the independence \SCs implied from $\mathcal{I}$. Then, we have $|\mathcal{I}^*| \leq 6 |\mathcal{I}|$.     
\end{Lemma}

%\begin{proof}
%Sketch. Applying the axioms introduced in Definition.~\ref{def:new-inference}, we can find that the inference system cannot generate any further more information beyond variables involved. It can be proved by contradiction. Furthermore, we apply the combination theory, where there are $2 \binom{3}{2}$ possible outcomes. \end{proof} . 



%Since the implication algorithm needs at most $\mathcal{O}(|\mathcal{I}|)$  is $\mathcal{O}(|\mathcal{I}|^2)$. Next, we 


\vspace{.5em}

\oliver{what is this an example for?}

\begin{example}
Given a set of \SCs $\Sigma=\{A\indep B, A \indep C | B, A \nindep C, B\indep C,  C \nindep D,  C \indep E | D, E \nindep F \}$, we check the consistency of $\Sigma$ as follows: 

\noindent {\underline{Step 1: Dividing}}.  Divide $\Sigma$ into $\mathcal{I} = \{A\indep B, A \indep C | B, B\indep C,  C \indep E | D\}$ and $\mathcal{D} =\{A \nindep C, C \nindep D, E \nindep F\}$;

\noindent {\underline{Step 2: Computing $\mathcal{I}^*$}}. By employing the implication algorithm on $\mathcal{I}$, we are able to acquire  $\mathcal{I}^*$. Similar to Example.~\ref{exa:implication}, we can obtain $\mathcal{I}^* = \{A\indep B, A\indep C, B\indep C, A \indep B|C, A \indep C | B, B \indep C |A,  C \indep E | D\}$. 

\noindent {\underline{Step 3: Checking the Implication}}. Check that whether there exists $\lambda \in \mathcal{D}$ such that $\lnot\lambda \in \mathcal{I}^*$ holds. We see that $\lnot\lambda: A \indep C$ is in $\mathcal{I}^*$, thus $\Sigma$ is inconsistent. 
\end{example}


{\noindent \bf Time Complexity.} The implication algorithm needs $\mathcal{O}(|\mathcal{I}^*|)$ iterations, and each iteration needs $\mathcal{O}(|\mathcal{I}^*|)$ time. The total time complexity is $\mathcal{O}(|\mathcal{I}^*|^2) = \mathcal{O}((6|\mathcal{I}|)^2) = \mathcal{O}(|\mathcal{I}|^2)$. For the consistency-checking algorithm, the main bottleneck is spent in running the implication algorithm to compute $\mathcal{I}^*$ (see Line 2 in Algorithm~\ref{alg:check}), thus the total time complexity is $\mathcal{O}(|\mathcal{I}|^2)$.



\subsubsection{An inference system for three random variables}

Graphoid Axioms $\mathcal{A}$ are applicable to any conditional independence statement. Since this paper only considers those conditional independence statements with no more than three variables, we can simplify $\mathcal{A}$.
%and derive a new inference system $\mathcal{G}$. 

\begin{Definition}\label{def:new-inference}
Let $A$, $B$, $C$ denote three random variables. The inference system $\mathcal{G}$ for \SCs consists of the following %inference 
rules.

{\noindent \emph{Symmetry}}:
\[A \indep B \mid C  \quad \Longleftrightarrow \quad B \indep A \mid C \]
%\[A \indep B \mid C  \quad \Longleftrightarrow \quad B \indep A \mid C\]

{\noindent \emph{Contraction-weak-union-decomposition}}:
\[\big (A \indep B\big)  ~~ \& ~~ \big (A \indep C \mid B\big ) \quad \Longrightarrow \quad  
\begin{cases}
A \indep C \\
A \indep B \mid C
\end{cases}\]
\end{Definition}

We can prove that Definition~\ref{def:graphoid-axioms} and Definition~\ref{def:new-inference} are equivalent for \SCs involving at most three random variables. Therefore, we only need to consider the two inference rules in $\mathcal{G}$ rather than all the rules in $\mathcal{A}$. Lemma~\ref{lem:equivalence} formally proves their equivalence. 

\begin{Lemma}\label{lem:equivalence}
    For any set $\mathcal{I}$ of \SCs involving at most three random variables, and any single \SC $\gamma$, we have that
    (i) if $\mathcal{I} \vdash_{\mathcal{A}} \gamma$, then $\mathcal{I} \vdash_{\mathcal{G}} \gamma$;
    (2) if $\mathcal{I} \vdash_{\mathcal{G}} \gamma$, then $\mathcal{I} \vdash_{\mathcal{A}} \gamma$,
    where $\mathcal{I} \vdash_{\mathcal{A}} \gamma$ (resp. $\mathcal{I} \vdash_{\mathcal{G}} \gamma$) denotes that  $\mathcal{I}$ implies $\gamma$ using $\mathcal{A}$ (resp. $\mathcal{G}$).
\end{Lemma}

\begin{proof}
    All the proofs of this paper can be found in Appendix.
\end{proof}

%\oliver{maybe add extension to future work}

We next discuss the soundness and completeness of the new inference system $\mathcal{G}$. 

\vspace{.5em}

{\noindent \bf Soundness.} Graphoid Axioms $\mathcal{A}$ have been proved to be sound ~\cite{pearl2014probabilistic}. Since $\mathcal{G}$ and $\mathcal{A}$ are equivalent for \SCs (Lemma~\ref{lem:equivalence}), we conclude that $\mathcal{G}$ is also sound.

\vspace{.5em}

{\noindent \bf Completeness.} When Graphoid Axioms were first developed, they were conjectured to be a complete inference system ~\cite{pearl2014probabilistic}. In 1990s, Studeny proved that the conjecture ~\cite{studeny1990conditional} was {\em incorrect}. However, Studeny's proof assumes that each independence statement is allowed to contain an arbitrary number of random variables, thus it is still an open question whether the system $\mathcal{A}$ is complete under the assumption that each independence statement contains no more than three variables. For this reason, we conjecture that \emph{when each independence statement contains no more than three variables, Graphoid Axioms $\mathcal{A}$ are complete}. If the conjecture is true, Lemma~\ref{lem:equivalence} entails that $\mathcal{G}$ is complete.   %We defer to future work.  in this situation. Based on the conjecture, we can easily prove that $\mathcal{I}$ is complete using Lemma~\ref{lem:equivalence}. 

% {\noindent \bf Remark.} To resolve the possibility of false positive detections by the $\mathcal{G}$, we further propose a \emph{sound} and \emph{complete} system \emph{$\mathcal{G}^{m}$} in Sec. \ref{cck_general} for any given \SCs.


%\vspace{.5em}

%{\noindent \bf Remark.}


%Please note that the above axioms also hold when $\set{Z}$ is empty, i.e., removing $\set{Z}$ from the condition of each conditional independence. For example, for the decomposition axiom, we have 
%\[\set{X} \indep \set{YW}   \Longrightarrow \set{X} \indep \set{Y} ~~ \& ~~ \set{X} \indep \set{W}.\]




%{\noindent \bf Remark.} The Graphoid Axioms was conjectured to be both sound and complete~[Pearl's paper??]. However, in 1990, Studeny proved that it is not complete, and the author further proved that there does not exist a finite set of axioms that are complete~\cite{studeny1990conditional}. However, in this paper, we assume that each \SC has no more than three variables. It is still an open question that when each condition dependence has no more than variables, whether the Graphoid Axioms is complete or not. In this paper, 


%only sound but not complete, it is widely used in practice (e.g., multivariate modeling and causality analysis). Thus, in this paper, we only 



%Geiger and Pearl~\cite{pearl2} has showed for the conditional independence and marginal independence can be governed by a set of axioms under certain assumptions. The axiom is called \textbf{Graphoid Axioms} $\mathcal{A}$ and it is complete and sound~\cite{pearl1}. 





\paragraph{Time Complexity for 3-Variable Inferences}

To analyze the time complexity of the implication algorithm, we answer two  questions:\\
\indent \emph{Q1. What is the time complexity of generating a new \SC?} \\
\indent \emph{Q2. How many new \SCs can be generated in total?}

\vspace{0.25em}

\noindent For $Q1$, consider the two inference rules in Definition~\ref{def:new-inference}. The algorithm first checks whether the symmetry rule can be used to generate a new \SC or not. The time complexity of this process is $\mathcal{O}(|\mathcal{I}^*|)$. For the contraction-weak-union-decomposition rule, a naive way is to enumerate every pair of \SCs in $\mathcal{I}^*$ and then check whether the rule can be used or not. It needs $\mathcal{O}(|\mathcal{I}^*|^2)$ time. In fact, we can utilize a hash table to reduce the time complexity to $\mathcal{O}(|\mathcal{I}^*|)$. Specifically, we build a hash table for marginal \SCs (e.g., $A \indep B$), and then for each conditional \SC (e.g.,  $A \indep C | B$), we check whether $A \indep B$ or $C \indep B$ exists in the hash table. %This avoids $n^2$ comparisons. In total, our algorithm needs $\mathcal{O}(|\mathcal{I}^*|)$ time to generate a new \SC at each iteration.      

\vspace{0.25em}





\noindent For $Q2$, we seek to compute an upper bound for the number of newly generated \SCs. The key observation is that for any inference rule in $\mathcal{G}$, its right-hand side will not introduce any new variable that is not on the left-hand side. For example, consider the contraction-weak-union-decomposition rule. The left-hand side has three variables $\{A, B, C\}$, and the right-hand side has the same three variables, without introducing any new variable.      


% \na{TO JN: do we need to like say, this observation is the coverage problem like CFD and DC said. }

Based on this observation, we find that there is a relationship between $|\mathcal{I}|$  and $|\mathcal{I}^*|$. That is, $|\mathcal{I}^*| \leq 12 |\mathcal{I}|$. If we consider symmetry \SCs (e.g., $A \indep B$ and $B \indep A$) are the same, then $|\mathcal{I}^*| \leq 6 |\mathcal{I}|$.  We give the intuition below, and provide a formal proof in Lemma~\ref{lem:upper-bound}. 

We say $\SC_1$ \emph{covers} $\SC_2$ if the variable set of $\SC_1$ is a superset of the variable set of $\SC_2$. %For example, suppose $\SC_1: A \indep B$. The variable set of $\SC_1$ is $\{A, B\}$. Then, it covers two different \SCs:
%\[A \indep B, \;\; B \indep A.\]
%\na{I changed a little bit of the example here, is it right?}
%
For example, suppose $\SC_1: A \indep B | C$. Then, it covers 6 different \SCs:
\begin{align*}
A \indep B,\;\; A \indep C,\;\; B \indep C,\;\; A \indep B | C,\;\; A \indep C | B,\;\; B \indep C | A
\end{align*}
The above observation implies the \SCs in $\mathcal{I}$ can cover all the \SCs in $\mathcal{I}^*$. Since each $\SC \in \mathcal{I}$ can cover at most 6 different \SCs, then we have that $|\mathcal{I}^*| \leq 6 |\mathcal{I}|$. Lemma~\ref{lem:upper-bound} formally proves this result.


\begin{Lemma}\label{lem:upper-bound}
Given a set $\mathcal{I}$ of independence \SCs, let $\mathcal{I}^*$ denote the set of all the independence \SCs implied from $\mathcal{I}$. Then, we have $|\mathcal{I}^*| \leq 6 |\mathcal{I}|$.     
\end{Lemma}

%\begin{proof}
%Sketch. Applying the axioms introduced in Definition.~\ref{def:new-inference}, we can find that the inference system cannot generate any further more information beyond variables involved. It can be proved by contradiction. Furthermore, we apply the combination theory, where there are $2 \binom{3}{2}$ possible outcomes. \end{proof} . 



%Since the implication algorithm needs at most $\mathcal{O}(|\mathcal{I}|)$  is $\mathcal{O}(|\mathcal{I}|^2)$. Next, we 


\vspace{.5em}



\begin{example}
Given a set of \SCs $\Sigma=\{A\indep B, A \indep C | B, A \nindep C, B\indep C,  C \nindep D,  C \indep E | D, E \nindep F \}$, we check the consistency of $\Sigma$ as follows: 

\noindent {\underline{Step 1: Dividing}}.  Divide $\Sigma$ into $\mathcal{I} = \{A\indep B, A \indep C | B, B\indep C,  C \indep E | D\}$ and $\mathcal{D} =\{A \nindep C, C \nindep D, E \nindep F\}$;

\noindent {\underline{Step 2: Computing $\mathcal{I}^*$}}. By employing the implication algorithm on $\mathcal{I}$, we are able to acquire  $\mathcal{I}^*$. Similar to Example.~\ref{exa:implication}, we can obtain $\mathcal{I}^* = \{A\indep B, A\indep C, B\indep C, A \indep B|C, A \indep C | B, B \indep C |A,  C \indep E | D\}$. 

\noindent {\underline{Step 3: Checking the Implication}}. Check that whether there exists $\lambda \in \mathcal{D}$ such that $\lnot\lambda \in \mathcal{I}^*$ holds. We see that $\lnot\lambda: A \indep C$ is in $\mathcal{I}^*$, thus $\Sigma$ is inconsistent. 
\end{example}


{\noindent \bf Time Complexity.} The implication algorithm needs $\mathcal{O}(|\mathcal{I}^*|)$ iterations, and each iteration needs $\mathcal{O}(|\mathcal{I}^*|)$ time. The total time complexity is $\mathcal{O}(|\mathcal{I}^*|^2) = \mathcal{O}((6|\mathcal{I}|)^2) = \mathcal{O}(|\mathcal{I}|^2)$. For the consistency-checking algorithm, the main bottleneck is spent in running the implication algorithm to compute $\mathcal{I}^*$ (see Line 2 in Algorithm~\ref{alg:check}), thus the total time complexity is $\mathcal{O}(|\mathcal{I}|^2)$.


\vspace{.5em}







% \subsection{A Sound and Complete Algorithm for Consistency checking}\label{cck_general}

% {\noindent \bf ~ Graph-induced Graphoid Axioms}. \cite{pearl2014probabilistic} showed that conditional independence statements based on graph-induced axioms satisfy the following rules, and it is proved that the systems $\mathcal{A}^m$ consisted of following rules is \emph{complete} and \emph{sound}   for graph-induced graphoids. 

% \begin{Definition}\label{def:grapho-induced-axioms}
% Let $\set{X}$, $\set{Y}$, $\set{Z}$, and $\set{W}$ denote four disjoint sets of random variables.\todo{Wikipedia does not assume disjointness} The \emph{graphoid Axioms} $\mathcal{A}^{m}$ are the following:

%     {\noindent \emph{Symmetry}}: 
% \[\set{X} \indep \set{Y} \mid \set{Z}  \quad \Longleftrightarrow \quad  \set{Y} \indep \set{X} \mid \set{Z}\]

% {\noindent \emph{Decomposition}}: 	
% \[
% \set{X} \indep \set{YW} \mid \set{Z}  \quad  \Longrightarrow \quad 
% \begin{cases}
% \set{X} \indep \set{Y} \mid \set{Z} \\
% \set{X} \indep \set{W} \mid \set{Z}
% \end{cases} 
% \]

% {\noindent \emph{Intersection}}:
% \[\big (\set{X} \indep \set{W} \mid \set{YZ} \big ) ~~ \& ~~ \big (\set{X} \indep \set{Y} \mid \set{WZ} \big ) \quad \Longrightarrow \quad  \set{X} \indep \set{YW} \mid \set{Z}\]


% {\noindent \emph{Strong Union}}:
% \[\set{X} \indep \set{Y} \mid \set{Z}  \quad \Longrightarrow \quad  \set{X} \indep \set{Y} \mid \set{ZW}\]

% {\noindent \emph{Transitivity}}: 	
% \[
% \set{X} \indep \set{Y} \mid \set{Z}  \quad  \Longrightarrow \quad \forall \gamma \notin \set{X} \cup \set{Y} \cup \set{Z}, ~\set{X} \indep \gamma \mid \set{Z}~ or ~ \set{Y} \indep \gamma \mid \set{Z}
% \]

% \end{Definition}


% Naturally, we also have $X \indep Y  \Longrightarrow \neg X\nindep Y$. By Definition ~\ref{def:grapho-induced-axioms}, we can consider \emph{Transitivity} as applying to dependence statements, and have a new axiom. 

% \vspace{1em}
% \begin{Lemma}
% {\noindent \emph{Dependence Transitivity}}:
% \[\exists \gamma \notin \set{X} \cup \set{Y} \cup \set{Z}, ~ \big (\set{X} \nindep \set{\gamma} \mid \set{Z} \big ) ~~ \& ~~ \big (\set{\gamma} \nindep \set{Y} \mid \set{Z} \big ) ~ \Longrightarrow ~ \set{X} \nindep \set{Y} \mid \set{Z}  \]

% \end{Lemma}




% % \begin{Definition}
% %     The inference system $\mathcal{G}^{m}$ of induced graph consists of five axioms in Definition ~\ref{def:grapho-induced-axioms} and \emph{Dependence Transitivity}
% % \end{Definition}

% The (conditional) independence and dependence are governed by six  properties proposed in Definition \ref{def:grapho-induced-axioms}. Simply applying the algorithm to resolve the inconsistency among given independence and dependence statements arises exponential computational costs. In the following, we propose a new class of dependence statements to refine axioms, and also brings a $O(n \times m^2)$ algorithm to resolve the inconsistency where $n$ is the numer of attributes of the given dataset, and $m$ is the number of given \SCs. 

% One key observation while handling multiple \SCs is that some of the information entailed by one group of \SCs can be completely covered by another group of \SCs. Intuitively, the idea is to replace some of \SCs with more powerful but straight forward \SCs in terms of implication. 

% \begin{Definition}[Refinement]
% Let $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ denote three disjoint sets of random variables. $\set{X}$, $\set{Y}$, $\set{Z}$ are not necessarily proper supersets of $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ respectively. Refinement means $X \indep Y | Z$ refines $X^{'} \indep Y^{'}~|~Z^{'}$, which can be written as $X \indep Y ~|~Z \geq X^{'} \indep Y^{'}~|~Z{'}$. Note that $X \indep Y ~|~Z > X^{'} \indep Y^{'}~|~Z{'}$ if and only if $X \indep Y ~|~Z \geq X^{'} \indep Y^{'}~|~Z{'}$ but $X^{'} \indep Y^{'}~|~Z{'} \geq X \indep Y ~|~Z$ doesn't hold.
% \end{Definition}

% \begin{Lemma}
%  Let $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ denote three disjoint sets of random variables. $\set{X}$, $\set{Y}$, $\set{Z}$ are not necessarily proper supersets of $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ respectively. If  $X \indep Y ~|~Z \geq X^{'} \indep Y^{'}~|~Z{'}$, then  $X \indep Y ~|~Z \longrightarrow X^{'} \indep Y^{'}~|~Z{'}$. 
% \end{Lemma}




% \begin{Definition}\label{def:cande}
% Let $\set{X}$, $\set{Y}$, $\set{Z}$, and $\set{W}$ denote four disjoint sets of random variables. The \emph{inference system} $\mathcal{G}^{m}$ for induced graph are the following:

% {\noindent \emph{Fast Intersection}}:
% \[\big (\set{X} \indep \set{Y} \mid \set{ZW} \big ) ~~ \& ~~ \big (\set{X} \indep \set{W} \mid \set{ZY} \big ) ~\Longleftrightarrow~ (\set{X} \indep \set{Y} \mid \set{Z}) ~~ \& ~~ (\set{X} \indep \set{W} \mid \set{Z}) \]

% % \vspace{0.5em}
% % Replace Independence \SCs: $~\set{X} \indep \set{Y} \mid \set{ZW}, \set{X} \indep \set{ZW} \mid \set{Y}$ by $\set{X} \indep \set{Y} \mid \set{Z}, \set{X} \indep \set{Z} \mid \set{W}$ 
% % \vspace{0.5em}

% {\noindent \emph{Dependence Transitivity}}:
% \[\big (\set{X} \nindep \set{\gamma} \mid \set{Z} \big ) ~~ \& ~~ \big (\set{\gamma^{'}} \nindep \set{\gamma} \mid \set{Z} \big ) \quad \Longrightarrow \quad \set{X} \nindep \set{\gamma^{'}} \mid \set{Z}\]
% \end{Definition}

% \begin{Lemma}[Dependence \SCs Upper Bound]\label{dep:upper}
%     Given a databset $D$ with $n$ attributes and $m$ dependence \SCs, by applying the \emph{Dependence Transitivity}, there will be at most $m\times n$ independence \SCs finally.
% \end{Lemma}

% Importantly, based on the refinement, we can use the \emph{Fast Intersection} Rule to deduce the given pairs when applying the axioms. By this way, the number of independence \SCs will not increase all the time. Meanwhile, leveraging dependence transitivity will bring more dependence \SCs, the largest number of inferred dependence \SCs can be bounded as shown in Lemma.\ref{dep:upper}. 

% \begin{Definition}[Consistency]\label{def:consistency_graph}
% For any given \SCs, if their \emph{Compressing} and \emph{Expanding} output a pair \SC: ~~$\set{X} \nindep \set{Y} \mid \set{Z}$ and $\set{X}^{'} \indep \set{Y}^{'} \mid \set{Z}^{'}$ such that $X \indep Y ~|~Z \geq X^{'} \indep Y^{'}~|~Z{'}$, the given \SCs are \textbf{inconsistent} otherwise given \SCs are \textbf{consistent} here $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ are three disjoint sets of random variables, and  $\set{X}$, $\set{Y}$, $\set{Z}$ are not necessarily proper supersets of $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ respectively.
% \end{Definition}


% Combing Definition.\ref{def:cande} and Definition.\ref{def:consistency_graph}, we get the Consistency Checking algorithm based on graph-induced inference system. Algorithm.\ref{alg:check_graph} elaborates the detailed pseudo-code. 

% \vspace{.5em}

% \noindent \textbf{Complexity Analysis.} For a given dataset $D$ with $n$ attributes, and $m$ \SCs. The consistency checking algorithm takes three steps. The first step is compressing independence \SCs if $\set{X}\indep \set{Y} \mid \set{Z}$ will be placed by $\set{X}\indep \set{Y} \mid \set{Z}^{'}$ where ${Z}^{'}$ contain fewer variables than ${Z}$. Each independence \SC can be replaced by \emph{at most} $n$ times. Hence, the number of compressing steps is $n \times m$ and the complexity is $O(mn)$. Similarly, in expanding step, for each dependence \SC will add \emph{at most} $n$ new \SCs. Obviously, the computational cost is $O(mn)$. Finally, we could possibly have at most $m$ independence \SCs to be checked against $m \times n$ dependence \SCs. Therefore, the complexity of the consistency checking algorithm is $O(m^2 \times n)$.


% \begin{Lemma}[Soundness]
% The \emph{Consistency Checking} based on $\mathcal{G}^{m}$ for induced graph is Sound.
% \end{Lemma}

% \begin{proof}
%     Sketch. To prove the soundness of the consistency checking algorithm, we need to prove the soundness of \emph{Fast-intersection}, \emph{Dependence Transitivity} and \emph{Refinement Consistency Checking}. By applying \emph{Decomposition, Intersection, and Strong Union}, it is easy to show the soundness of Fast Intersection. 
    
%     The soundness of compressing and expanding step. The
% \end{proof}

% \begin{Lemma}[Completeness]
% The \emph{Consistency Checking} based on $\mathcal{G}^{m}$ for induced graph is Complete.
% \end{Lemma}

% \begin{proof}
%     Sketch. 
% \end{proof}



% \begin{example}

% \end{example}


% \begin{algorithm}[t]
% \caption{Consistency-checking Algorithm}\label{alg:check_graph}
% 	\KwIn{A set of \SCs: $\Sigma$}
% 	\KwOut{Consistent or not (YES or NO)}
% 	\vspace{0.5em}
% 	Divide $\Sigma$ into $\mathcal{I}$ and $\mathcal{D}$\;
% 	Compressing $\mathcal{I}$ to obtain $\mathcal{I}^{'}$ by Fast Intersection \;
% 	Expanding $\mathcal{D}$ to obtain $\mathcal{D}^{'}$ by Dependence Transitivity\;
% 	\For{$\lambda \in \mathcal{D}^{'}$}
% 	{
% 	    \If{there $\exists~\omega$ in $I^{'}$ such that $\lnot \lambda \geq  I $}
% 	   {
% 	        {\bf return} NO\; 
% 	    }
% 	}
% 	{\bf return} YES\;
% \end{algorithm}






% Employing the refinement, we can rewrite the independence and dependence statements, and moreover, we can compress the (conditional) independence.


% \begin{Lemma}
%  Let $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ denote three disjoint sets of random variables. $\set{X}$, $\set{Y}$, $\set{Z}$ are not necessarily proper supersets of $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ respectively. If  $X \indep Y ~|~Z \geq X^{'} \indep Y^{'}~|~Z{'}$, then $X \indep Y ~|~Z$  is derivable from  $X^{'} \indep Y^{'}~|~Z{'}$, which can be written as $X \indep Y ~|~Z \longrightarrow X^{'} \indep Y^{'}~|~Z{'}$. 
% \end{Lemma}


% \begin{Proof}
% If $X \indep Y ~|~Z \geq X^{'} \indep Y^{'}~|~Z{'}$, then we can rewrite the claim as 
% \end{Proof}





\iffalse 
    













\subsection{Implication Problem} \label{subsec:implication}



\subsection{Consistency and Implication}


\subsection{Consistency Checking Problem}

\iffalse
\begin{Definition}[Consistency]
	A set of Statistical Constraints $\SC$ is \defterm{consistent} if and only if there exists a probability distribution $\prob$ that satisfies all (in)dependence statements in $\SC$. We use $\SC \sim \mathbb{P}$ to denote this. \oliver{a bit unusual notation, maybe check Pearl's or other papers. update: Pearl uses subscript notation Ch. 3.1., so maybe this is okay.} 
	%If there is no probability distribution $\mathbb{P}$ satisfies the statistical constraints $\Sigma$, we say that the set $\Sigma$ is not consistent, or the statistical constraints has the consistency violation. 
\end{Definition}
\fi


\subsection{Efficient Consistency checking}

In this section, we present an algorithm for checking the internal consistency of a set of constraints~\cite{cck}. The most general version of the consistency problem is known to be \oliver{undecidable?}. Our algorithm works in the case where statistical constraints are limited to 3 variables. While this is a strong assumption, it covers a range of natural (in)dependence constraints, sufficient for us to evaluate the efficacy of our approach for data cleaning. Under future work we discuss a number of ways in which the limitation to 3 variables can be overcome. 
Based on previous inference system, we construct a new system ~\ref{inference} to solve the consistency checking problem introduced in ~\ref{cck}. 
 %And we further extend to support all statistical constraints(Sec.~\ref{extension}). 
 
 \oliver{I'm confused about two things. 1) If we assume 3 variables only, do we need any axioms? 2) I would think Geiger and Pearl look at implication only, not consistency. They usually look at independence statements only which are always consistent.}
 
 \na{Yes, we still need the axioms for the inference. Since we omit one and compress another two axioms.}


%We further investigate the fundamental problem: Consistency Checking problem (Sec.~\ref{}), and propose a new inference system and algorithm to support Statistical Constraints introduced in this paper(Sec.~\ref{inference}, Sec.~\ref{checking}), and we further extend to support all statistical constraints(Sec.~\ref{extension}). 
%In this section, we propose the problem on consistency checking. We first give the problem definition of consistency checking. Later, we provide the solution to this problem. We show that our algorithm can bound the time complexity to $O(n^2)$. Furthermore, we provide a method to repair the statistical constraints under certain budget. 


%\subsection{Consistency and Consistency Checking}

% The consistency and implication are two fundamental properties in Statistical Constraints, and are proposed in ~\cite{pearl2,Banjo,pearl1}. The consistency measures the agreement between constraints, that is whether there exists any contradiction between constraints. The implication between statistical constraints is whether the given statistical constraints can entail other statistical constraints. 



A key observations here is that, if we are given the set of random variables, $U=\{x_1,x_2,x_3,...\}$, the maximum number of constraints over $U$ is bounded. 

\begin{Lemma}[Consistent Constraints Bound]
	Given a set of constraints $\Sigma$ following the input in this paper, the maximum number of $|\Sigma|$  is  $\frac{n(n-1)(n-2)}{2}$.
\end{Lemma}

\na {TO JN: Do we need to have a motivation example here? To highlight the significance of this problem, just use the example in the slides? }

\quad Consistency problem of independence problem is first proposed by Dan Geiger and Judea Pearl~\cite{pearl2} in 1992. The formal definition of the consistency given the set of statistical constraints is below.

\begin{Problem}[Consistency Checking]
	Given a set of statistical constraints $S$ over set of variables $X$, whether $S$ is consistent or not.
\end{Problem}

Obviously, to solve this problem, we need to find whether there are some contradictory between statistical constraints. A observation here is that simply check the constraints between the independence set $I$ and the dependence set $D$ is not applicable since the statistical constraint have the capacity to entail other statistical constraints. Therefore, we need an inference system to infer all constraints that can be entailed by the given constraints. 



\subsection{A new Inference System for SCs} \label{inference}

% The implication between statistical constraints is whether the given statistical constraints can entail other statistical constraints.
~\cite{ pearl2} has showed for the conditional independence and marginal independence can be governed by a set of axioms under certain assumptions. The axiom is called \textbf{Graphoid Axioms} $\mathcal{A}$ and it is complete and sound~\cite{pearl1}.  

However, in this paper, our statistical constraints is a special type of the independence and dependence. Under the same assumption in ~\cite{pearl1}, we introduce our new axioms and prove it is complete and sound. 
\begin{Definition}[Graphoid Axioms $\mathcal{A}$]
	Let $X$, $Y$ and $Z$ be three random variables, and $W$ be the further variable. The following conditions hold for the independence relationship 
\end{Definition}	
	
	Symmetry: 
\begin{equation}
 			 I(X,Z,Y) \longleftrightarrow I(Y,Z,X)
\end{equation}
	
	Decomposition: 
\begin{equation}
      I(X,Z,Y\cup W) \longrightarrow I(X,Z,Y)  \quad \& \quad  I(X,Z,W) 
\end{equation}

	Weak Union: 
\begin{equation}
    I(X,Z,Y\cup W) \longrightarrow I(X,Z\cup W,Y)
\end{equation}

  Contraction: 
\begin{equation}
	I(X,Z,Y) \&  I(X,Z\cup W,Y)  \longrightarrow I(X,Z,Y\cup W)
\end{equation}

	Intersection:
\begin{equation}
	I(X,Z,Y)  \quad \& \quad  I(X,Z,W) \longrightarrow   I(X,Z,Y\cup W) 
\end{equation}

The $\mathcal{A}$ here is applicable for all independence relationship. However, considered our statistical constraints(no more than three variables for one constraint), it is not that useful since some of  for our statistical constraints is not applicable to  them.


The below we introduce our new Graphoid Axioms $\mathcal{A^+}$.

\begin{Definition}[New Graphoid Axioms $\mathcal{A^+}$]
	Let $X$, $Y$ and $Z$ be three random variables, and $W$ be the further variable. The following conditions hold for the independence relationship 
\end{Definition}	

Symmetry: 
\begin{equation}\label{sym}
	I(X,Z,Y) \longleftrightarrow I(Y,Z,X)
\end{equation}

Contraction-union-decomposition: 
\begin{equation}\label{con}
\begin{split}
	I(X,\varnothing,Y) \&  I(X,Y,W) \longleftrightarrow & I(X,\varnothing,Y\cup W) \\ \longrightarrow & I(X,\varnothing, Y)  \&  I(X,\varnothing,W) \\&   I(X,Y,W)  \&  I(X,W,Y) 
\end{split}
\end{equation}

%Intersection-union-decomposition: 
%\begin{equation}\label{in}
%\begin{split}
%I(X,Y,W) \&  I(X,Y,W) \longleftrightarrow & I(X,\varnothing,Y\cup W) \\ \longrightarrow & I(X,\varnothing, Y)  \&  I(X,\varnothing,W) \\&  I(X,\varnothing,Y) \&  I(X,Y,W)
%\end{split}
%\end{equation}
%
%If we combine the equation \ref{con} and equation \ref{in}, we can have a new axiom to replace the two. 
%
%\begin{equation}\label{in}
%\begin{split}
%I(X,Y,W) \&  I(X,Y,W) & \longleftrightarrow  I(X,\varnothing,Y\cup W) \\&   \longleftrightarrow  I(X,\varnothing,Y) \&  I(X,Y,W) \\ &  \longrightarrow I(X,\varnothing, Y)  \&  I(X,\varnothing,W) 
%\end{split}
%\end{equation}



\begin{Conjecture}[Pearl's Conjecture]
	In this paper, we follow Pearl's conjecture that the graphoid axiom system is complete and conjecture. ~\cite{pearl1}
\end{Conjecture}

     Also, we find that New Graphoid Axioms $\mathcal{A^+}$ is also complete and sound under Pearl's Conjecture. 
    
     To show that our conclusion is right, we first introduce the following lemma.
     
     \begin{Lemma}\label{bound}
     	The number of new constraints that can be inferred from one single Statistical Constraint is $6$ at most.
     \end{Lemma}
     
     \begin{proof}
     	Nathan to do
     \end{proof}
     
     
     Based on Lemma ~\ref{bound}, we then formally prove our conjecture. 
     
\begin{Theorem}~\label{com}
	New Graphoid Axioms $\mathcal{A^+}$ is sound and complete under Pearl's Conjecture.
\end{Theorem}

\begin{proof}
	Nathan TO DO
\end{proof}


\subsection{Efficient Consistency Checking algorithm with $\mathcal{A^+}$ }~\label{checking}

In this section, we further show an efficient checking algorithms with the new inference rule $\mathcal{A^+}$.

\oliver{I thought we were assuming 3 variables only?}

\begin{algorithm}[h]\label{check}
	\caption{Efficient Consistency Checking }\label{algorithm: bcc}
	\KwIn{A set of Independence Constraints $I$, A set of Dependence constraints $D$, Inference system $A$}
	\KwOut{Consistent or not (YES or NO)}
	%	$G \leftarrow \emptyset$ \;
	$S \leftarrow I$\;
	$E \leftarrow \emptyset $ \;  
	$Con \leftarrow 0$ \;
	%	$E \leftarrow \emptyset$ \;
	\For{each constriaints in $I$}
	{
		Add marginal constraints into $E$ \;
		Remove marginal constraints from $I$ \;
	}
	
	\For{each $a$ in $E$}
	{
		\For{each $b$ in $I$}
		{
			\If{$a$ matches $b$ by $A$}
			{
				Infer new constraints from $a$ and $b$ by $A$ \;
				Add new constraints into $S$ \;
				Add new marginal constraints into $E$ \;
			}
			remove $a$ \;
		}	
	}
	\If{$S \cap D^c = \emptyset$}
	{
		$Con \leftarrow 1$ \;
	}
	Return $Con$
\end{algorithm}

\subsection{Extension Algorithm}~\label{extension}
\na{To Oliver: refer to Oliver's work} 


\subsection{Summary} \label{sum}

\fi

==> consistency-new.tex <==
\section{Properties of {\Large \bf \SCs}} \label{cck}
%We further study two properties of Statistical Constraints, and one fundamental problem associated with Statistical Constraints.
Before applying \SCs to error detection, we need to investigate a number of basic properties of \SCs. In this section, we first present an inference system for \SCs, and then study two fundamental properties associated with \SCs: (1) \emph{Consistency}: whether a set of \SCs have conflicts; (2) \emph{Implication}: whether a set of \SCs imply (entail) another \SC. %We first present an inference system for statistical constraints in Section~\ref{subsec:infer}, and then propose our solutions to the consistency and redundancy problems in Section~\ref{subsec:consistency} and Section~\ref{subsec:implication}, respectively.


\subsection{A General Inference System for {\large \bf \SCs}} \label{subsec:infer}
An inference system consists of  a collection of inference rules, where each rule is in the form of 
\[\SC_1 ~~\&~~ \SC_2 \cdots ~~\&~~ \SC_n \quad \Longrightarrow \quad \SC_{new},\]
which states that if the left-hand side \SCs hold, then the right-hand side \SC must hold. Having an inference system is essential to solve the consistency problem. For example,  suppose we are given three constraints:
\[\Sigma = \{\SC_1:  A \indep B, ~~~~\SC_2:  A \indep C | B, ~~~~\SC_3: A \nindep C\}.\] 
Applying the rule (see Definition~\ref{def:new-inference}):
\[(A \indep B) \quad  \&  \quad  (A \indep C | B) \quad  \Longrightarrow \quad A \indep C,\]
shows that $\Sigma$ is inconsistent because $\SC_1$ and $\SC_2$ imply $\neg \SC_3$. 


For existing row-oriented constraints, FDs have a sound and complete inference system that is known as Armstrong’s Axioms~\cite{abiteboul1995foundations}. Wenfei et al. extend Armstrong’s Axioms to CFDs and prove that the new inference system is also sound and complete~\cite{bohannon2007conditional}. Xu et al. develop a set of sound (but not complete) inference rules for DCs~\cite{chu2013holistic}. A natural question is: can we develop a sound and complete inference system for \SCs? In the following, we first introduce some background knowledge about the well-known \emph{Graphoid Axioms}~\cite{pearl2}, and then present our inference system derived from the axioms. 



\vspace{.5em}

{\noindent \bf Graphoid Axioms.} %In the Statistics field, 
Geiger and Pearl~\cite{pearl2} showed that conditional independence statements satisfy the following  axioms.
%(inference rules).
%known as the \emph{Graphoid Axioms} $\mathcal{A}$. 

\begin{Definition}\label{def:graphoid-axioms}
Let $\set{X}$, $\set{Y}$, $\set{Z}$, and $\set{W}$ denote four disjoint sets of random variables. The \emph{graphoid Axioms} $\mathcal{A}$ are the following:

{\noindent \emph{Symmetry}}: 
\[\set{X} \indep \set{Y} \mid \set{Z}  \quad \Longleftrightarrow \quad  \set{Y} \indep \set{X} \mid \set{Z}\]

{\noindent \emph{Decomposition}}: 	
\[
\set{X} \indep \set{YW} \mid \set{Z}  \quad  \Longrightarrow \quad 
\begin{cases}
\set{X} \indep \set{Y} \mid \set{Z} \\
\set{X} \indep \set{W} \mid \set{Z}
\end{cases} 
\]

{\noindent \emph{Weak Union}}:
\[\set{X} \indep \set{YW} \mid \set{Z}  \quad \Longrightarrow  \quad \set{X} \indep \set{Y} \mid \set{ZW}\]

{\noindent \emph{Contraction}}:
\[\big (\set{X} \indep \set{Y} \mid \set{Z} \big ) ~~ \& ~~ \big (\set{X} \indep \set{W} \mid \set{YZ} \big ) \quad \Longrightarrow \quad  \set{X} \indep \set{YW} \mid \set{Z}\]

% {\noindent \emph{Intersection}}:
% \[\big (\set{X} \indep \set{Y} \mid \set{Z}\big )  ~~ \& ~~  \big (\set{X} \indep \set{W} \mid \set{Z}\big ) \quad \Longrightarrow \quad   \set{X} \indep \set{YW} \mid \set{Z}\]
\end{Definition}

\noindent Note that $\set{Z}$ can be the empty set.
%thus the above axioms also hold without $\set{Z}$. 
For example, for the symmetry axiom, we have $\set{X} \indep \set{Y}   \Longrightarrow \set{Y} \indep \set{X}.$



\vspace{.5em}

{\noindent \bf A General Inference System for \SCs.} Graphoid Axioms $\mathcal{A}$ are applicable to any conditional independence statement. Since this paper only considers those conditional independence statements with no more than three variables, we can simplify $\mathcal{A}$.
%and derive a new inference system $\mathcal{G}$. 

\begin{Definition}\label{def:new-inference}
Let $A$, $B$, $C$ denote three random variables. The inference system $\mathcal{G}$ for \SCs consists of the following %inference 
rules.

{\noindent \emph{Symmetry}}:
\[A \indep B \mid C  \quad \Longleftrightarrow \quad B \indep A \mid C \]
%\[A \indep B \mid C  \quad \Longleftrightarrow \quad B \indep A \mid C\]

{\noindent \emph{Contraction-weak-union-decomposition}}:
\[\big (A \indep B\big)  ~~ \& ~~ \big (A \indep C \mid B\big ) \quad \Longrightarrow \quad  
\begin{cases}
A \indep C \\
A \indep B \mid C
\end{cases}\]
\end{Definition}

We can prove that Definition~\ref{def:graphoid-axioms} and Definition~\ref{def:new-inference} are equivalent for \SCs involving at most three random variables. Therefore, we only need to consider the two inference rules in $\mathcal{G}$ rather than all the rules in $\mathcal{A}$. Lemma~\ref{lem:equivalence} formally proves their equivalence. 

\begin{Lemma}\label{lem:equivalence}
    For any set $\mathcal{I}$ of \SCs involving at most three random variables, and any single \SC $\gamma$, we have that
    (i) if $\mathcal{I} \vdash_{\mathcal{A}} \gamma$, then $\mathcal{I} \vdash_{\mathcal{G}} \gamma$;
    (2) if $\mathcal{I} \vdash_{\mathcal{G}} \gamma$, then $\mathcal{I} \vdash_{\mathcal{A}} \gamma$,
    where $\mathcal{I} \vdash_{\mathcal{A}} \gamma$ (resp. $\mathcal{I} \vdash_{\mathcal{G}} \gamma$) denotes that  $\mathcal{I}$ implies $\gamma$ using $\mathcal{A}$ (resp. $\mathcal{G}$).
\end{Lemma}

\begin{proof}
    All the proofs of this paper can be found in Appendix.
\end{proof}

%\oliver{maybe add extension to future work}

We next discuss the soundness and completeness of the new inference system $\mathcal{G}$. 

\vspace{.5em}

{\noindent \bf Soundness.} Graphoid Axioms $\mathcal{A}$ have been proved to be sound ~\cite{pearl2014probabilistic}. Since $\mathcal{G}$ and $\mathcal{A}$ are equivalent for \SCs (Lemma~\ref{lem:equivalence}), we conclude that $\mathcal{G}$ is also sound.

\vspace{.5em}

{\noindent \bf Completeness.} When Graphoid Axioms were first developed, they were conjectured to be a complete inference system ~\cite{pearl2014probabilistic}. In 1990s, Studeny proved that the conjecture ~\cite{studeny1990conditional} was {\em incorrect}. However, Studeny's proof assumes that each independence statement is allowed to contain an arbitrary number of random variables, thus it is still an open question whether the system $\mathcal{A}$ is complete under the assumption that each independence statement contains no more than three variables. For this reason, we conjecture that \emph{when each independence statement contains no more than three variables, Graphoid Axioms $\mathcal{A}$ are complete}. If the conjecture is true, Lemma~\ref{lem:equivalence} entails that $\mathcal{G}$ is complete.   %We defer to future work.  in this situation. Based on the conjecture, we can easily prove that $\mathcal{I}$ is complete using Lemma~\ref{lem:equivalence}. 

{\noindent \bf Remark.} To resolve the possibility of false positive detections by the $\mathcal{G}$, we further propose a \emph{sound} and \emph{complete} system \emph{$\mathcal{G}^{m}$} in Sec. \ref{cck_general} for any given \SCs.


%\vspace{.5em}

%{\noindent \bf Remark.}


%Please note that the above axioms also hold when $\set{Z}$ is empty, i.e., removing $\set{Z}$ from the condition of each conditional independence. For example, for the decomposition axiom, we have 
%\[\set{X} \indep \set{YW}   \Longrightarrow \set{X} \indep \set{Y} ~~ \& ~~ \set{X} \indep \set{W}.\]




%{\noindent \bf Remark.} The Graphoid Axioms was conjectured to be both sound and complete~[Pearl's paper??]. However, in 1990, Studeny proved that it is not complete, and the author further proved that there does not exist a finite set of axioms that are complete~\cite{studeny1990conditional}. However, in this paper, we assume that each \SC has no more than three variables. It is still an open question that when each condition dependence has no more than variables, whether the Graphoid Axioms is complete or not. In this paper, 


%only sound but not complete, it is widely used in practice (e.g., multivariate modeling and causality analysis). Thus, in this paper, we only 



%Geiger and Pearl~\cite{pearl2} has showed for the conditional independence and marginal independence can be governed by a set of axioms under certain assumptions. The axiom is called \textbf{Graphoid Axioms} $\mathcal{A}$ and it is complete and sound~\cite{pearl1}. 






\subsection{Consistency and Implication} \label{subsec:consistency}
Being able to check whether a given set $\Sigma$ of \SCs is consistent or not is important because if  $\Sigma$ is not consistent, %when applying it to error detection, 
a user will get contradictory error-detection results. In the following, we first formally define the consistency problem, and then present a consistency-checking framework. In order to apply the framework, the key is to solve the implication problem. Therefore, we define the implication problem and propose an efficient implication algorithm. 
%
Intuitively, if $\Sigma$ is consistent, it means that $\Sigma$ has no conflict. That is, there exists a joint distribution that satisfies $\Sigma$. Definition~\ref{def:consistency} presents a formal definition.

\begin{Definition}[Consistency]\label{def:consistency}
Given a set $\Sigma$ of \SCs, let $\set{V}$ denote the set of random variables that appear in $\Sigma$. The consistency problem is to determine whether there exists a joint distribution $P(\set{V})$ that satisfies every \SC in $\Sigma$. 
\end{Definition}


\begin{figure}[t]
   \centering 
   \includegraphics[width=0.9\linewidth]{fig/joint-new.pdf} 
   \vspace{-1em}
   \caption{An example of a joint distribution that satisfies $\Sigma = \{A \indep B,\; A \nindep B| C\}$}\label{fig:joint}\vspace{-1.5em}
\end{figure}

For example, consider $\Sigma = \{A \indep B,\; A \nindep B| C\}$. Since there are three random variables in $\Sigma$, we have $\set{V} = \{A, B, C\}$. As shown in Figure~\ref{fig:joint}, we can construct a joint distribution $P(A, B, C)$ that satisfies $\Sigma$, thus $\Sigma$ is consistent. If we are given $\Sigma' = \{A \indep B,\; A \nindep B\}$, it is impossible to construct a joint distribution that satisfies $\Sigma'$, thus $\Sigma'$ is inconsistent. 

\vspace{.5em}

{\noindent \bf Consistency-checking Framework.} Geiger and Pearl~\cite{pearl2} proposed a framework to solve the consistency problem. They first divide $\Sigma$ into two disjoint sets $\mathcal{I}$ and $\mathcal{D}$, where $\mathcal{I}$ (resp. $\mathcal{D}$) represents the set of independence (resp. dependence) statements in $\Sigma$. For each $\lambda \in \mathcal{D}$, it checks whether $\mathcal{I}$ implies $\lnot \lambda$. If the answer is no for all $\lambda$, then $\Sigma$ is consistent; otherwise, it is not consistent. The correctness of the framework was proved in~\cite{pearl2}. For example, consider $\Sigma = \{A \indep B,\; A \nindep B| C\}$. We have $\mathcal{I} = \{A \indep B\}$  and $\mathcal{D} = \{A \nindep B| C\}$. We can see that $\mathcal{D}$ does not imply  $\lnot \lambda = A \indep B| C$, thus $\Sigma$ is consistent.    


\vspace{.5em}

To apply the above framework,
%to solve the problem in Definition~\ref{def:consistency}, the key challenge is how to efficiently check whether $\mathcal{I}$ implies $\lnot \lambda$ or not.  In other words, 
we aim to determine whether an independence \SC $\gamma$ can be inferred from $\mathcal{I}$ using $\mathcal{G}$.  Definition~\ref{def:implication} formally defines the implication problem. 

\begin{Definition}[Implication]\label{def:implication}
Given a set $\mathcal{I}$ of independence \SCs, and another independence \SC $\gamma$, the implication problem is to determine whether $\gamma$ can be inferred from $\mathcal{I}$ using $\mathcal{G}$, i.e., check whether $\mathcal{I} \vdash_{\mathcal{G}} \gamma$ holds or not.
\end{Definition}

{\noindent \bf Implication Algorithm.} We propose an iterative algorithm. The algorithm starts with $\mathcal{I}^* = \mathcal{I}$, and then iteratively expands $\mathcal{I}^*$ with new \SCs. At each iteration, the algorithm checks which inference rule in $\mathcal{G}$ can be used to generate a new \SC, and then adds it to $\mathcal{I}^*$. The algorithm terminates when $\mathcal{I}^*$ cannot be further expanded. After that, the algorithm checks whether $\gamma \in \mathcal{I}^*$ holds. If so, then $\mathcal{I}$ implies  $\gamma$; otherwise, $\mathcal{I}$ does not imply $\gamma$.

\begin{example}~\label{exa:implication}
Given a set of independence \SCs $\mathcal{I} = \{A\indep B, A \indep C | B, B\indep C,  C \indep E | D\}$ over attributes $M=\{A, B, C, D, \\
E\}$. To compute $\mathcal{I}^*$, we initially set $\mathcal{I}^* = \mathcal{I}$, and then apply the implication algorithm.

\noindent {\underline{Step 1: Constructing Hash Table}}. $H=\{\{A,B\},\{B,C\}\}$ will be generated according to the marginal \SCs  in  $\mathcal{I}^*$, i.e., $A \indep B$ and $B \indep C $.

\noindent {\underline{Step 2: Employing Inference System $\mathcal{G}$}}. We check each conditional \SC in $\mathcal{I}^*$. For $\SC_1:A \indep C | B $, we first check whether $\{A,B\}$ or $\{B,C\}$ exists. Obviously, we have both of them in the $H$. Applying the \emph{contraction-weak-union-decomposition} inference rule in $\mathcal{G}$, we can obtain three new \SCs: $A\indep B|C$, $B \indep C |A$, and $A \indep C$. We add them into $\mathcal{I}^*$, and hash $A \indep C$ as $\{A,C\}$ and add it into $H$. 

\noindent {\underline{Step 3: Repeating}}. Repeat Step 1 and Step 2 till there are no more \SCs that can be inferred. In this example, we eventually arrive at $\mathcal{I}^* = \{A\indep B, A\indep C, B\indep C, A \indep B|C, A \indep C | B, B \indep C |A,  C \indep E | D\}$. 

\end{example}

To analyze the time complexity of the implication algorithm, we answer two  questions:\\
\indent \emph{Q1. What's the time complexity of generating a new \SC?} \\
\indent \emph{Q2. How many new \SCs can be generated in total?}

\vspace{0.25em}

\noindent For $Q1$, consider the two inference rules in Definition~\ref{def:new-inference}. The algorithm first checks whether the symmetry rule can be used to generate a new \SC or not. The time complexity of this process is $\mathcal{O}(|\mathcal{I}^*|)$. For the contraction-weak-union-decomposition rule, a naive way is to enumerate every pair of \SCs in $\mathcal{I}^*$ and then check whether the rule can be used or not. It needs $\mathcal{O}(|\mathcal{I}^*|^2)$ time. In fact, we can utilize a hash table to reduce the time complexity to $\mathcal{O}(|\mathcal{I}^*|)$. Specifically, we build a hash table for marginal \SCs (e.g., $A \indep B$), and then for each conditional \SC (e.g.,  $A \indep C | B$), we check whether $A \indep B$ or $C \indep B$ exists in the hash table. %This avoids $n^2$ comparisons. In total, our algorithm needs $\mathcal{O}(|\mathcal{I}^*|)$ time to generate a new \SC at each iteration.      

\vspace{0.25em}





\noindent For $Q2$, we seek to compute an upper bound for the number of newly generated \SCs. The key observation is that for any inference rule in $\mathcal{G}$, its right-hand side will not introduce any new variable that is not on the left-hand side. For example, consider the contraction-weak-union-decomposition rule. The left-hand side has three variables $\{A, B, C\}$, and the right-hand side has the same three variables, without introducing any new variable.      


% \na{TO JN: do we need to like say, this observation is the coverage problem like CFD and DC said. }

Based on this observation, we find that there is a relationship between $|\mathcal{I}|$  and $|\mathcal{I}^*|$. That is, $|\mathcal{I}^*| \leq 12 |\mathcal{I}|$. If we consider symmetry \SCs (e.g., $A \indep B$ and $B \indep A$) are the same, then $|\mathcal{I}^*| \leq 6 |\mathcal{I}|$.  We give the intuition below, and provide a formal proof in Lemma~\ref{lem:upper-bound}. 

We say $\SC_1$ \emph{covers} $\SC_2$ if the variable set of $\SC_1$ is a superset of the variable set of $\SC_2$. %For example, suppose $\SC_1: A \indep B$. The variable set of $\SC_1$ is $\{A, B\}$. Then, it covers two different \SCs:
%\[A \indep B, \;\; B \indep A.\]
%\na{I changed a little bit of the example here, is it right?}
%
For example, suppose $\SC_1: A \indep B | C$. Then, it covers 6 different \SCs:
\begin{align*}
A \indep B,\;\; A \indep C,\;\; B \indep C,\;\; A \indep B | C,\;\; A \indep C | B,\;\; B \indep C | A
\end{align*}
The above observation implies the \SCs in $\mathcal{I}$ can cover all the \SCs in $\mathcal{I}^*$. Since each $\SC \in \mathcal{I}$ can cover at most 6 different \SCs, then we have that $|\mathcal{I}^*| \leq 6 |\mathcal{I}|$. Lemma~\ref{lem:upper-bound} formally proves this result.


\begin{Lemma}\label{lem:upper-bound}
Given a set $\mathcal{I}$ of independence \SCs, let $\mathcal{I}^*$ denote the set of all the independence \SCs implied from $\mathcal{I}$. Then, we have $|\mathcal{I}^*| \leq 6 |\mathcal{I}|$.     
\end{Lemma}

%\begin{proof}
%Sketch. Applying the axioms introduced in Definition.~\ref{def:new-inference}, we can find that the inference system cannot generate any further more information beyond variables involved. It can be proved by contradiction. Furthermore, we apply the combination theory, where there are $2 \binom{3}{2}$ possible outcomes. \end{proof} . 



%Since the implication algorithm needs at most $\mathcal{O}(|\mathcal{I}|)$  is $\mathcal{O}(|\mathcal{I}|^2)$. Next, we 


\vspace{.5em}

{\noindent \bf Consistency-checking Algorithm.} We can develop a consistency-checking algorithm using the implication algorithm. See the pseudo-code in Algorithm~\ref{alg:check}. The algorithm first computes $\mathcal{I}^*$. Then, for each $\lambda \in \mathcal{D}$, it checks whether $\lnot\lambda \in \mathcal{I}^*$ holds or not. If no for all $\lambda$, then $\Sigma$ is consistent; otherwise, $\Sigma$ is inconsistent. 

%there exists $\lambda \in \mathcal{D}$ such that $\lnot\lambda \in \mathcal{I}^*$, it means that $\mathcal{I}$ implies $\lnot\lambda$. Since $\lambda \in \mathcal{D}$, then $\Sigma$ is inconsistent. If there does not exist $\lambda  \in \mathcal{D}$ such that $\lnot\lambda \in \mathcal{I}^*$, then $\Sigma$ is consistent. 
% \na{To JN: do we need the pseudo-code algorithm for this?}


\begin{algorithm}[t]
	\caption{Consistency-checking Algorithm}\label{alg:check}
	\KwIn{A set of \SCs: $\Sigma$}
	\KwOut{Consistent or not (YES or NO)}
	\vspace{0.5em}
	Divide $\Sigma$ into $\mathcal{I}$ and $\mathcal{D}$\;
	Use the implication algorithm to obtain $\mathcal{I}^*$\;
	\For{$\lambda \in \mathcal{D}$}
	{
	    \If{$\lnot \lambda \in \mathcal{I}^*$}
	    {
	        {\bf return} NO\; 
	    }
	}
	{\bf return} YES\;
\end{algorithm}

\begin{example}
Given a set of \SCs $\Sigma=\{A\indep B, A \indep C | B, A \nindep C, B\indep C,  C \nindep D,  C \indep E | D, E \nindep F \}$, we check the consistency of $\Sigma$ as follows: 

\noindent {\underline{Step 1: Dividing}}.  Divide $\Sigma$ into $\mathcal{I} = \{A\indep B, A \indep C | B, B\indep C,  C \indep E | D\}$ and $\mathcal{D} =\{A \nindep C, C \nindep D, E \nindep F\}$;

\noindent {\underline{Step 2: Computing $\mathcal{I}^*$}}. By employing the implication algorithm on $\mathcal{I}$, we are able to acquire  $\mathcal{I}^*$. Similar to Example.~\ref{exa:implication}, we can obtain $\mathcal{I}^* = \{A\indep B, A\indep C, B\indep C, A \indep B|C, A \indep C | B, B \indep C |A,  C \indep E | D\}$. 

\noindent {\underline{Step 3: Checking the Implication}}. Check that whether there exists $\lambda \in \mathcal{D}$ such that $\lnot\lambda \in \mathcal{I}^*$ holds. We see that $\lnot\lambda: A \indep C$ is in $\mathcal{I}^*$, thus $\Sigma$ is inconsistent. 
\end{example}


{\noindent \bf Time Complexity.} The implication algorithm needs $\mathcal{O}(|\mathcal{I}^*|)$ iterations, and each iteration needs $\mathcal{O}(|\mathcal{I}^*|)$ time. The total time complexity is $\mathcal{O}(|\mathcal{I}^*|^2) = \mathcal{O}((6|\mathcal{I}|)^2) = \mathcal{O}(|\mathcal{I}|^2)$. For the consistency-checking algorithm, the main bottleneck is spent in running the implication algorithm to compute $\mathcal{I}^*$ (see Line 2 in Algorithm~\ref{alg:check}), thus the total time complexity is $\mathcal{O}(|\mathcal{I}|^2)$.


\vspace{.5em}


{\noindent \bf Resolving Inconsistency.} Once an inconsistency is detected, we help the user to resolve the inconsistency.  Specifically, suppose the consistency-checking algorithm finds a conflict: $\mathcal{I}$ implies $A \indep B$ but $A \nindep B$ is in $\Sigma$. We ask the user to check which one is correct. If the former is correct, then $A \nindep B$ should not be in $\Sigma$, and we remove $A \nindep B$ from $\Sigma$. Otherwise, we show the derivation of $A \indep B$  from $\mathcal{I}$ and then ask the user to remove the incorrect \SCs involved in the derivation.   



\subsection{A Sound and Complete Algorithm for Consistency checking}\label{cck_general}

{\noindent \bf ~ Graph-induced Graphoid Axioms}. \cite{pearl2014probabilistic} showed that conditional independence statements based on graph-induced axioms satisfy the following rules, and it is proved that the systems $\mathcal{A}^m$ consisted of following rules is \emph{complete} and \emph{sound}   for graph-induced graphoids. 

\begin{Definition}\label{def:grapho-induced-axioms}
Let $\set{X}$, $\set{Y}$, $\set{Z}$, and $\set{W}$ denote four disjoint sets of random variables. The \emph{graphoid Axioms} $\mathcal{A}^{m}$ are the following:

    {\noindent \emph{Symmetry}}: 
\[\set{X} \indep \set{Y} \mid \set{Z}  \quad \Longleftrightarrow \quad  \set{Y} \indep \set{X} \mid \set{Z}\]

{\noindent \emph{Decomposition}}: 	
\[
\set{X} \indep \set{YW} \mid \set{Z}  \quad  \Longrightarrow \quad 
\begin{cases}
\set{X} \indep \set{Y} \mid \set{Z} \\
\set{X} \indep \set{W} \mid \set{Z}
\end{cases} 
\]

{\noindent \emph{Intersection}}:
\[\big (\set{X} \indep \set{W} \mid \set{YZ} \big ) ~~ \& ~~ \big (\set{X} \indep \set{Y} \mid \set{WZ} \big ) \quad \Longrightarrow \quad  \set{X} \indep \set{YW} \mid \set{Z}\]


{\noindent \emph{Strong Union}}:
\[\set{X} \indep \set{Y} \mid \set{Z}  \quad \Longrightarrow \quad  \set{X} \indep \set{Y} \mid \set{ZW}\]

{\noindent \emph{Transitivity}}: 	
\[
\set{X} \indep \set{Y} \mid \set{Z}  \quad  \Longrightarrow \quad \forall \gamma \notin \set{X} \cup \set{Y} \cup \set{Z}, ~\set{X} \indep \gamma \mid \set{Z}~ or ~ \set{Y} \indep \gamma \mid \set{Z}
\]

\end{Definition}


Naturally, we also have $X \indep Y  \Longrightarrow \neg X\nindep Y$. By Definition ~\ref{def:grapho-induced-axioms}, we can consider \emph{Transitivity} as applying to dependence statements, and have a new axiom. 

\vspace{1em}
\begin{Lemma}
{\noindent \emph{Dependence Transitivity}}:
\[\exists \gamma \notin \set{X} \cup \set{Y} \cup \set{Z}, ~ \big (\set{X} \nindep \set{\gamma} \mid \set{Z} \big ) ~~ \& ~~ \big (\set{\gamma} \nindep \set{Y} \mid \set{Z} \big ) ~ \Longrightarrow ~ \set{X} \nindep \set{Y} \mid \set{Z}  \]

\end{Lemma}




% \begin{Definition}
%     The inference system $\mathcal{G}^{m}$ of induced graph consists of five axioms in Definition ~\ref{def:grapho-induced-axioms} and \emph{Dependence Transitivity}
% \end{Definition}

The (conditional) independence and dependence are governed by six  properties proposed in Definition \ref{def:grapho-induced-axioms}. Simply applying the algorithm to resolve the inconsistency among given independence and dependence statements arises exponential computational costs. In the following, we propose a new class of dependence statements to refine axioms, and also brings a $O(n \times m^2)$ algorithm to resolve the inconsistency where $n$ is the numer of attributes of the given dataset, and $m$ is the number of given \SCs. 

One key observation while handling multiple \SCs is that some of the information entailed by one group of \SCs can be completely covered by another group of \SCs. Intuitively, the idea is to replace some of \SCs with more powerful but straight forward \SCs in terms of implication. 

\begin{Definition}[Refinement]
Let $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ denote three disjoint sets of random variables. $\set{X}$, $\set{Y}$, $\set{Z}$ are not necessarily proper supersets of $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ respectively. Refinement means $X \indep Y | Z$ refines $X^{'} \indep Y^{'}~|~Z^{'}$, which can be written as $X \indep Y ~|~Z \geq X^{'} \indep Y^{'}~|~Z{'}$. Note that $X \indep Y ~|~Z > X^{'} \indep Y^{'}~|~Z{'}$ if and only if $X \indep Y ~|~Z \geq X^{'} \indep Y^{'}~|~Z{'}$ but $X^{'} \indep Y^{'}~|~Z{'} \geq X \indep Y ~|~Z$ doesn't hold.
\end{Definition}

\begin{Lemma}
 Let $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ denote three disjoint sets of random variables. $\set{X}$, $\set{Y}$, $\set{Z}$ are not necessarily proper supersets of $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ respectively. If  $X \indep Y ~|~Z \geq X^{'} \indep Y^{'}~|~Z{'}$, then  $X \indep Y ~|~Z \longrightarrow X^{'} \indep Y^{'}~|~Z{'}$. 
\end{Lemma}




\begin{Definition}\label{def:cande}
Let $\set{X}$, $\set{Y}$, $\set{Z}$, and $\set{W}$ denote four disjoint sets of random variables. The \emph{inference system} $\mathcal{G}^{m}$ for induced graph are the following:

{\noindent \emph{Fast Intersection}}:
\[\big (\set{X} \indep \set{Y} \mid \set{ZW} \big ) ~~ \& ~~ \big (\set{X} \indep \set{W} \mid \set{ZY} \big ) ~\Longleftrightarrow~ (\set{X} \indep \set{Y} \mid \set{Z}) ~~ \& ~~ (\set{X} \indep \set{W} \mid \set{Z}) \]

% \vspace{0.5em}
% Replace Independence \SCs: $~\set{X} \indep \set{Y} \mid \set{ZW}, \set{X} \indep \set{ZW} \mid \set{Y}$ by $\set{X} \indep \set{Y} \mid \set{Z}, \set{X} \indep \set{Z} \mid \set{W}$ 
% \vspace{0.5em}

{\noindent \emph{Dependence Transitivity}}:
\[\big (\set{X} \nindep \set{\gamma} \mid \set{Z} \big ) ~~ \& ~~ \big (\set{\gamma^{'}} \nindep \set{\gamma} \mid \set{Z} \big ) \quad \Longrightarrow \quad \set{X} \nindep \set{\gamma^{'}} \mid \set{Z}\]
\end{Definition}

\begin{Lemma}[Dependence \SCs Upper Bound]\label{dep:upper}
    Given a databset $D$ with $n$ attributes and $m$ dependence \SCs, by applying the \emph{Dependence Transitivity}, there will be at most $m\times n$ independence \SCs finally.
\end{Lemma}

Importantly, based on the refinement, we can use the \emph{Fast Intersection} Rule to deduce the given pairs when applying the axioms. By this way, the number of independence \SCs will not increase all the time. Meanwhile, leveraging dependence transitivity will bring more dependence \SCs, the largest number of inferred dependence \SCs can be bounded as shown in Lemma.\ref{dep:upper}. 

\begin{Definition}[Consistency]\label{def:consistency_graph}
For any given \SCs, if their \emph{Compressing} and \emph{Expanding} output a pair \SC: ~~$\set{X} \nindep \set{Y} \mid \set{Z}$ and $\set{X}^{'} \indep \set{Y}^{'} \mid \set{Z}^{'}$ such that $X \indep Y ~|~Z \geq X^{'} \indep Y^{'}~|~Z{'}$, the given \SCs are \textbf{inconsistent} otherwise given \SCs are \textbf{consistent} here $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ are three disjoint sets of random variables, and  $\set{X}$, $\set{Y}$, $\set{Z}$ are not necessarily proper supersets of $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ respectively.
\end{Definition}


Combing Definition.\ref{def:cande} and Definition.\ref{def:consistency_graph}, we get the Consistency Checking algorithm based on graph-induced inference system. Algorithm.\ref{alg:check_graph} elaborates the detailed pseudo-code. 

\vspace{.5em}

\noindent \textbf{Complexity Analysis.} For a given dataset $D$ with $n$ attributes, and $m$ \SCs. The consistency checking algorithm takes three steps. The first step is compressing independence \SCs if $\set{X}\indep \set{Y} \mid \set{Z}$ will be placed by $\set{X}\indep \set{Y} \mid \set{Z}^{'}$ where ${Z}^{'}$ contain fewer variables than ${Z}$. Each independence \SC can be replaced by \emph{at most} $n$ times. Hence, the number of compressing steps is $n \times m$ and the complexity is $O(mn)$. Similarly, in expanding step, for each dependence \SC will add \emph{at most} $n$ new \SCs. Obviously, the computational cost is $O(mn)$. Finally, we could possibly have at most $m$ independence \SCs to be checked against $m \times n$ dependence \SCs. Therefore, the complexity of the consistency checking algorithm is $O(m^2 \times n)$.


\begin{Lemma}[Soundness]
The \emph{Consistency Checking} based on $\mathcal{G}^{m}$ for induced graph is Sound.
\end{Lemma}

\begin{proof}
    Sketch. To prove the soundness of the consistency checking algorithm, we need to prove the soundness of \emph{Fast-intersection}, \emph{Dependence Transitivity} and \emph{Refinement Consistency Checking}. By applying \emph{Decomposition, Intersection, and Strong Union}, it is easy to show the soundness of Fast Intersection. 
    
    The soundness of compressing and expanding step. The
\end{proof}

\begin{Lemma}[Completeness]
The \emph{Consistency Checking} based on $\mathcal{G}^{m}$ for induced graph is Complete.
\end{Lemma}

\begin{proof}
    Sketch. 
\end{proof}



\begin{example}

\end{example}


\begin{algorithm}[t]
\caption{Consistency-checking Algorithm}\label{alg:check_graph}
	\KwIn{A set of \SCs: $\Sigma$}
	\KwOut{Consistent or not (YES or NO)}
	\vspace{0.5em}
	Divide $\Sigma$ into $\mathcal{I}$ and $\mathcal{D}$\;
	Compressing $\mathcal{I}$ to obtain $\mathcal{I}^{'}$ by Fast Intersection \;
	Expanding $\mathcal{D}$ to obtain $\mathcal{D}^{'}$ by Dependence Transitivity\;
	\For{$\lambda \in \mathcal{D}^{'}$}
	{
	    \If{there $\exists~\omega$ in $I^{'}$ such that $\lnot \lambda \geq  I $}
	   {
	        {\bf return} NO\; 
	    }
	}
	{\bf return} YES\;
\end{algorithm}






% Employing the refinement, we can rewrite the independence and dependence statements, and moreover, we can compress the (conditional) independence.


% \begin{Lemma}
%  Let $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ denote three disjoint sets of random variables. $\set{X}$, $\set{Y}$, $\set{Z}$ are not necessarily proper supersets of $\set{X}^{'}$, $\set{Y}^{'}$, and $\set{Z}^{'}$ respectively. If  $X \indep Y ~|~Z \geq X^{'} \indep Y^{'}~|~Z{'}$, then $X \indep Y ~|~Z$  is derivable from  $X^{'} \indep Y^{'}~|~Z{'}$, which can be written as $X \indep Y ~|~Z \longrightarrow X^{'} \indep Y^{'}~|~Z{'}$. 
% \end{Lemma}


% \begin{Proof}
% If $X \indep Y ~|~Z \geq X^{'} \indep Y^{'}~|~Z{'}$, then we can rewrite the claim as 
% \end{Proof}





\iffalse 
    













\subsection{Implication Problem} \label{subsec:implication}



\subsection{Consistency and Implication}


\subsection{Consistency Checking Problem}

\iffalse
\begin{Definition}[Consistency]
	A set of Statistical Constraints $\SC$ is \defterm{consistent} if and only if there exists a probability distribution $\prob$ that satisfies all (in)dependence statements in $\SC$. We use $\SC \sim \mathbb{P}$ to denote this. \oliver{a bit unusual notation, maybe check Pearl's or other papers. update: Pearl uses subscript notation Ch. 3.1., so maybe this is okay.} 
	%If there is no probability distribution $\mathbb{P}$ satisfies the statistical constraints $\Sigma$, we say that the set $\Sigma$ is not consistent, or the statistical constraints has the consistency violation. 
\end{Definition}
\fi


\subsection{Efficient Consistency checking}

In this section, we present an algorithm for checking the internal consistency of a set of constraints~\cite{cck}. The most general version of the consistency problem is known to be \oliver{undecidable?}. Our algorithm works in the case where statistical constraints are limited to 3 variables. While this is a strong assumption, it covers a range of natural (in)dependence constraints, sufficient for us to evaluate the efficacy of our approach for data cleaning. Under future work we discuss a number of ways in which the limitation to 3 variables can be overcome. 
Based on previous inference system, we construct a new system ~\ref{inference} to solve the consistency checking problem introduced in ~\ref{cck}. 
 %And we further extend to support all statistical constraints(Sec.~\ref{extension}). 
 
 \oliver{I'm confused about two things. 1) If we assume 3 variables only, do we need any axioms? 2) I would think Geiger and Pearl look at implication only, not consistency. They usually look at independence statements only which are always consistent.}
 
 \na{Yes, we still need the axioms for the inference. Since we omit one and compress another two axioms.}


%We further investigate the fundamental problem: Consistency Checking problem (Sec.~\ref{}), and propose a new inference system and algorithm to support Statistical Constraints introduced in this paper(Sec.~\ref{inference}, Sec.~\ref{checking}), and we further extend to support all statistical constraints(Sec.~\ref{extension}). 
%In this section, we propose the problem on consistency checking. We first give the problem definition of consistency checking. Later, we provide the solution to this problem. We show that our algorithm can bound the time complexity to $O(n^2)$. Furthermore, we provide a method to repair the statistical constraints under certain budget. 


%\subsection{Consistency and Consistency Checking}

% The consistency and implication are two fundamental properties in Statistical Constraints, and are proposed in ~\cite{pearl2,Banjo,pearl1}. The consistency measures the agreement between constraints, that is whether there exists any contradiction between constraints. The implication between statistical constraints is whether the given statistical constraints can entail other statistical constraints. 



A key observations here is that, if we are given the set of random variables, $U=\{x_1,x_2,x_3,...\}$, the maximum number of constraints over $U$ is bounded. 

\begin{Lemma}[Consistent Constraints Bound]
	Given a set of constraints $\Sigma$ following the input in this paper, the maximum number of $|\Sigma|$  is  $\frac{n(n-1)(n-2)}{2}$.
\end{Lemma}

\na {TO JN: Do we need to have a motivation example here? To highlight the significance of this problem, just use the example in the slides? }

\quad Consistency problem of independence problem is first proposed by Dan Geiger and Judea Pearl~\cite{pearl2} in 1992. The formal definition of the consistency given the set of statistical constraints is below.

\begin{Problem}[Consistency Checking]
	Given a set of statistical constraints $S$ over set of variables $X$, whether $S$ is consistent or not.
\end{Problem}

Obviously, to solve this problem, we need to find whether there are some contradictory between statistical constraints. A observation here is that simply check the constraints between the independence set $I$ and the dependence set $D$ is not applicable since the statistical constraint have the capacity to entail other statistical constraints. Therefore, we need an inference system to infer all constraints that can be entailed by the given constraints. 



\subsection{A new Inference System for SCs} \label{inference}

% The implication between statistical constraints is whether the given statistical constraints can entail other statistical constraints.
~\cite{ pearl2} has showed for the conditional independence and marginal independence can be governed by a set of axioms under certain assumptions. The axiom is called \textbf{Graphoid Axioms} $\mathcal{A}$ and it is complete and sound~\cite{pearl1}.  

However, in this paper, our statistical constraints is a special type of the independence and dependence. Under the same assumption in ~\cite{pearl1}, we introduce our new axioms and prove it is complete and sound. 
\begin{Definition}[Graphoid Axioms $\mathcal{A}$]
	Let $X$, $Y$ and $Z$ be three random variables, and $W$ be the further variable. The following conditions hold for the independence relationship 
\end{Definition}	
	
	Symmetry: 
\begin{equation}
 			 I(X,Z,Y) \longleftrightarrow I(Y,Z,X)
\end{equation}
	
	Decomposition: 
\begin{equation}
      I(X,Z,Y\cup W) \longrightarrow I(X,Z,Y)  \quad \& \quad  I(X,Z,W) 
\end{equation}

	Weak Union: 
\begin{equation}
    I(X,Z,Y\cup W) \longrightarrow I(X,Z\cup W,Y)
\end{equation}

  Contraction: 
\begin{equation}
	I(X,Z,Y) \&  I(X,Z\cup W,Y)  \longrightarrow I(X,Z,Y\cup W)
\end{equation}

	Intersection:
\begin{equation}
	I(X,Z,Y)  \quad \& \quad  I(X,Z,W) \longrightarrow   I(X,Z,Y\cup W) 
\end{equation}

The $\mathcal{A}$ here is applicable for all independence relationship. However, considered our statistical constraints(no more than three variables for one constraint), it is not that useful since some of  for our statistical constraints is not applicable to  them.


The below we introduce our new Graphoid Axioms $\mathcal{A^+}$.

\begin{Definition}[New Graphoid Axioms $\mathcal{A^+}$]
	Let $X$, $Y$ and $Z$ be three random variables, and $W$ be the further variable. The following conditions hold for the independence relationship 
\end{Definition}	

Symmetry: 
\begin{equation}\label{sym}
	I(X,Z,Y) \longleftrightarrow I(Y,Z,X)
\end{equation}

Contraction-union-decomposition: 
\begin{equation}\label{con}
\begin{split}
	I(X,\varnothing,Y) \&  I(X,Y,W) \longleftrightarrow & I(X,\varnothing,Y\cup W) \\ \longrightarrow & I(X,\varnothing, Y)  \&  I(X,\varnothing,W) \\&   I(X,Y,W)  \&  I(X,W,Y) 
\end{split}
\end{equation}

%Intersection-union-decomposition: 
%\begin{equation}\label{in}
%\begin{split}
%I(X,Y,W) \&  I(X,Y,W) \longleftrightarrow & I(X,\varnothing,Y\cup W) \\ \longrightarrow & I(X,\varnothing, Y)  \&  I(X,\varnothing,W) \\&  I(X,\varnothing,Y) \&  I(X,Y,W)
%\end{split}
%\end{equation}
%
%If we combine the equation \ref{con} and equation \ref{in}, we can have a new axiom to replace the two. 
%
%\begin{equation}\label{in}
%\begin{split}
%I(X,Y,W) \&  I(X,Y,W) & \longleftrightarrow  I(X,\varnothing,Y\cup W) \\&   \longleftrightarrow  I(X,\varnothing,Y) \&  I(X,Y,W) \\ &  \longrightarrow I(X,\varnothing, Y)  \&  I(X,\varnothing,W) 
%\end{split}
%\end{equation}



\begin{Conjecture}[Pearl's Conjecture]
	In this paper, we follow Pearl's conjecture that the graphoid axiom system is complete and conjecture. ~\cite{pearl1}
\end{Conjecture}

     Also, we find that New Graphoid Axioms $\mathcal{A^+}$ is also complete and sound under Pearl's Conjecture. 
    
     To show that our conclusion is right, we first introduce the following lemma.
     
     \begin{Lemma}\label{bound}
     	The number of new constraints that can be inferred from one single Statistical Constraint is $6$ at most.
     \end{Lemma}
     
     \begin{proof}
     	Nathan to do
     \end{proof}
     
     
     Based on Lemma ~\ref{bound}, we then formally prove our conjecture. 
     
\begin{Theorem}~\label{com}
	New Graphoid Axioms $\mathcal{A^+}$ is sound and complete under Pearl's Conjecture.
\end{Theorem}

\begin{proof}
	Nathan TO DO
\end{proof}


\subsection{Efficient Consistency Checking algorithm with $\mathcal{A^+}$ }~\label{checking}

In this section, we further show an efficient checking algorithms with the new inference rule $\mathcal{A^+}$.

\oliver{I thought we were assuming 3 variables only?}

\begin{algorithm}[h]\label{check}
	\caption{Efficient Consistency Checking }\label{algorithm: bcc}
	\KwIn{A set of Independence Constraints $I$, A set of Dependence constraints $D$, Inference system $A$}
	\KwOut{Consistent or not (YES or NO)}
	%	$G \leftarrow \emptyset$ \;
	$S \leftarrow I$\;
	$E \leftarrow \emptyset $ \;  
	$Con \leftarrow 0$ \;
	%	$E \leftarrow \emptyset$ \;
	\For{each constriaints in $I$}
	{
		Add marginal constraints into $E$ \;
		Remove marginal constraints from $I$ \;
	}
	
	\For{each $a$ in $E$}
	{
		\For{each $b$ in $I$}
		{
			\If{$a$ matches $b$ by $A$}
			{
				Infer new constraints from $a$ and $b$ by $A$ \;
				Add new constraints into $S$ \;
				Add new marginal constraints into $E$ \;
			}
			remove $a$ \;
		}	
	}
	\If{$S \cap D^c = \emptyset$}
	{
		$Con \leftarrow 1$ \;
	}
	Return $Con$
\end{algorithm}

\subsection{Extension Algorithm}~\label{extension}
\na{To Oliver: refer to Oliver's work} 


\subsection{Summary} \label{sum}

\fi

==> consistency-old.tex <==
\section{Properties of Statistical Constraints}

In this section, we studies the fundamental properties of Statistical Constraints: Consistency and Implication (Sec.~\ref{cck}). Based on previous inference system, we construct a new system ~\ref{inference} to solve the consistency checking problem introduced in ~\ref{cck}. And we further extend to support all statistical constraints(Sec.~\ref{extension}). We summarize this section in ~\ref{sum}


%We further investigate the fundamental problem: Consistency Checking problem (Sec.~\ref{}), and propose a new inference system and algorithm to support Statistical Constraints introduced in this paper(Sec.~\ref{inference}, Sec.~\ref{checking}), and we further extend to support all statistical constraints(Sec.~\ref{extension}). 
%In this section, we propose the problem on consistency checking. We first give the problem definition of consistency checking. Later, we provide the solution to this problem. We show that our algorithm can bound the time complexity to $O(n^2)$. Furthermore, we provide a method to repair the statistical constraints under certain budget. 


\subsection{Consistency and Consistency Checking}\label{cck}
The consistency and implication are two fundamental properties in Statistical Constraints, and are proposed in ~\cite{pearl2,Banjo,pearl1}. The consistency measures the agreement between constraints, that is whether there exists any contradiction between constraints. The implication between statistical constraints is whether the given statistical constraints can entail other statistical constraints. 

\begin{Definition}[Consistency]
	We define the Consistency of a set of Statistical Constraints $\Sigma$ as there exists a probability distribution $\mathbb{P}$ that satisfies all statistical constraints in $S$. We use $\Sigma \sim \mathbb{P}$ to denote this. If there is no probability distribution $\mathbb{P}$ satisfies the statistical constraints $\Sigma$, we say that the set $\Sigma$ is not consistent, or the statistical constraints has the consistency violation. 
\end{Definition}

A key observations here is that, if we are given the set of random variables, $U=\{x_1,x_2,x_3,...\}$, the maximum number of constraints over $U$ is bounded. 

\begin{Lemma}[Consistent Constraints Bound]
	Given a set of constraints $\Sigma$ following the input in this paper, the maximum number of $|\Sigma|$  is  $\frac{n(n-1)(n-2)}{2}$.
\end{Lemma}

\na {TO JN: Do we need to have a motivation example here? To highlight the significance of this problem, just use the example in the slides? }

\quad Consistency problem of independence problem is first proposed by Dan Geiger and Judea Pearl~\cite{pearl2} in 1992. The formal definition of the consistency given the set of statistical constraints is below.

\begin{Problem}[Consistency Checking]
	Given a set of statistical constraints $S$ over set of variables $X$, whether $S$ is consistent or not.
\end{Problem}

Obviously, to solve this problem, we need to find whether there are some contradictory between statistical constraints. A observation here is that simply check the constraints between the independence set $I$ and the dependence set $D$ is not applicable since the statistical constraint have the capacity to entail other statistical constraints. Therefore, we need an inference system to infer all constraints that can be entailed by the given constraints. 



\subsection{A new Inference System for SCs} \label{inference}

% The implication between statistical constraints is whether the given statistical constraints can entail other statistical constraints.
~\cite{ pearl2} has showed for the conditional independence and marginal independence can be governed by a set of axioms under certain assumptions. The axiom is called \textbf{Graphoid Axioms} $\mathcal{A}$ and it is complete and sound~\cite{pearl1}.  

However, in this paper, our statistical constraints is a special type of the independence and dependence. Under the same assumption in ~\cite{pearl1}, we introduce our new axioms and prove it is complete and sound. 
\begin{Definition}[Graphoid Axioms $\mathcal{A}$]
	Let $X$, $Y$ and $Z$ be three random variables, and $W$ be the further variable. The following conditions hold for the independence relationship 
\end{Definition}	
	
	Symmetry: 
\begin{equation}
 			 I(X,Z,Y) \longleftrightarrow I(Y,Z,X)
\end{equation}
	
	Decomposition: 
\begin{equation}
      I(X,Z,Y\cup W) \longrightarrow I(X,Z,Y)  \quad \& \quad  I(X,Z,W) 
\end{equation}

	Weak Union: 
\begin{equation}
    I(X,Z,Y\cup W) \longrightarrow I(X,Z\cup W,Y)
\end{equation}

  Contraction: 
\begin{equation}
	I(X,Z,Y) \&  I(X,Z\cup W,Y)  \longrightarrow I(X,Z,Y\cup W)
\end{equation}

	Intersection:
\begin{equation}
	I(X,Z,Y)  \quad \& \quad  I(X,Z,W) \longrightarrow   I(X,Z,Y\cup W) 
\end{equation}

The $\mathcal{A}$ here is applicable for all independence relationship. However, considered our statistical constraints(no more than three variables for one constraint), it is not that useful since some of  for our statistical constraints is not applicable to  them.


The below we introduce our new Graphoid Axioms $\mathcal{A^+}$.

\begin{Definition}[New Graphoid Axioms $\mathcal{A^+}$]
	Let $X$, $Y$ and $Z$ be three random variables, and $W$ be the further variable. The following conditions hold for the independence relationship 
\end{Definition}	

Symmetry: 
\begin{equation}\label{sym}
	I(X,Z,Y) \longleftrightarrow I(Y,Z,X)
\end{equation}

Contraction-union-decomposition: 
\begin{equation}\label{con}
\begin{split}
	I(X,\varnothing,Y) \&  I(X,Y,W) \longleftrightarrow & I(X,\varnothing,Y\cup W) \\ \longrightarrow & I(X,\varnothing, Y)  \&  I(X,\varnothing,W) \\&   I(X,Y,W)  \&  I(X,W,Y) 
\end{split}
\end{equation}

%Intersection-union-decomposition: 
%\begin{equation}\label{in}
%\begin{split}
%I(X,Y,W) \&  I(X,Y,W) \longleftrightarrow & I(X,\varnothing,Y\cup W) \\ \longrightarrow & I(X,\varnothing, Y)  \&  I(X,\varnothing,W) \\&  I(X,\varnothing,Y) \&  I(X,Y,W)
%\end{split}
%\end{equation}
%
%If we combine the equation \ref{con} and equation \ref{in}, we can have a new axiom to replace the two. 
%
%\begin{equation}\label{in}
%\begin{split}
%I(X,Y,W) \&  I(X,Y,W) & \longleftrightarrow  I(X,\varnothing,Y\cup W) \\&   \longleftrightarrow  I(X,\varnothing,Y) \&  I(X,Y,W) \\ &  \longrightarrow I(X,\varnothing, Y)  \&  I(X,\varnothing,W) 
%\end{split}
%\end{equation}



\begin{Conjecture}[Pearl's Conjecture]
	In this paper, we follow Pearl's conjecture that the graphoid axiom system is complete and conjecture. ~\cite{pearl1}
\end{Conjecture}

     Also, we find that New Graphoid Axioms $\mathcal{A^+}$ is also complete and sound under Pearl's Conjecture. 
    
     To show that our conclusion is right, we first introduce the following lemma.
     
     \begin{Lemma}\label{bound}
     	The number of new constraints that can be inferred from one single Statistical Constraint is $9$ at most.
     \end{Lemma}
     
     \begin{proof}
     	Nathan to do
     \end{proof}
     
     
     Based on Lemma ~\ref{bound}, we then formally prove our conjecture. 
     
\begin{Theorem}~\label{com}
	New Graphoid Axioms $\mathcal{A^+}$ is sound and complete under Pearl's Conjecture.
\end{Theorem}

\begin{proof}
	Nathan TO DO
\end{proof}


\subsection{Efficient Consistency Checking algorithm with $\mathcal{A^+}$ }~\label{checking}

\begin{algorithm}[h]\label{check}
	\caption{Consistency Checking }\label{algorithm: bcc}
	\KwIn{A set of Independence Constraints $I$, A set of Dependence constraints $D$, Inference system $A$}
	\KwOut{Consistent or not (YES or NO)}
	%	$G \leftarrow \emptyset$ \;
	$S \leftarrow I$\;
	$E \leftarrow \emptyset $ \;  
	$Con \leftarrow 0$ \;
	%	$E \leftarrow \emptyset$ \;
	\For{each constriaints in $I$}
	{
		Add marginal constraints into $E$ \;
		Remove marginal constraints from $I$ \;
	}
	
	\For{each $a$ in $E$}
	{
		\For{each $b$ in $I$}
		{
			\If{$a$ matches $b$ by $A$}
			{
				Infer new constraints from $a$ and $b$ by $A$ \;
				Add new constraints into $S$ \;
				Add new marginal constraints into $E$ \;
				remove $b$ \;
			}
			remove $a$ \;
		}	
	}
	\If{$S \cap D^c = \emptyset$}
	{
		$Con \leftarrow 1$ \;
	}
	Return $Con$
\end{algorithm}

\subsection{Extension Algorithm}~\label{extension}
\na{To Oliver: Oliver's work}
\subsection{Summary} \label{sum}




==> consistency_vldb.tex <==
\section{Properties of {\Large \bf \SCs}} \label{cck}
%We further study two properties of Statistical Constraints, and one fundamental problem associated with Statistical Constraints.
Before applying \SCs to error detection, we need to investigate a number of basic properties of \SCs. In this section, we first present an inference system for \SCs, and then study two fundamental properties associated with \SCs: (1) \emph{Consistency}: whether a set of \SCs have conflicts; (2) \emph{Implication}: whether a set of \SCs imply (entail) another \SC. %We first present an inference system for statistical constraints in Section~\ref{subsec:infer}, and then propose our solutions to the consistency and redundancy problems in Section~\ref{subsec:consistency} and Section~\ref{subsec:implication}, respectively.


\subsection{An Inference System for {\large \bf \SCs}} \label{subsec:infer}
An inference system consists of  a collection of inference rules, where each rule is in the form of 
\[\SC_1 ~~\&~~ \SC_2 \cdots ~~\&~~ \SC_n \quad \Longrightarrow \quad \SC_{new},\]
which states that if the left-hand side \SCs hold, then the right-hand side \SC must hold. Having an inference system is essential to solve the consistency problem. For example,  suppose we are given three constraints:
\[\Sigma = \{\SC_1:  A \indep B, ~~~~\SC_2:  A \indep C | B, ~~~~\SC_3: A \nindep C\}.\] 
Applying the rule (see Definition~\ref{def:new-inference}):
\[(A \indep B) \quad  \&  \quad  (A \indep C | B) \quad  \Longrightarrow \quad A \indep C,\]
shows that $\Sigma$ is inconsistent because $\SC_1$ and $\SC_2$ imply $\neg \SC_3$. 


For existing row-oriented constraints, FDs have a sound and complete inference system that is known as Armstrong’s Axioms~\cite{abiteboul1995foundations}. Wenfei et al. extend Armstrong’s Axioms to CFDs and prove that the new inference system is also sound and complete~\cite{bohannon2007conditional}. Xu et al. develop a set of sound (but not complete) inference rules for DCs~\cite{chu2013holistic}. A natural question is: can we develop a sound and complete inference system for \SCs? In the following, we first introduce some background knowledge about the well-known \emph{Graphoid Axioms}~\cite{pearl2}, and then present our inference system derived from the axioms. 



\vspace{.5em}

{\noindent \bf Graphoid Axioms.} %In the Statistics field, 
Geiger and Pearl~\cite{pearl2} showed that conditional independence statements satisfy the following  axioms.
%(inference rules).
%known as the \emph{Graphoid Axioms} $\mathcal{A}$. 

\begin{Definition}\label{def:graphoid-axioms}
Let $\set{X}$, $\set{Y}$, $\set{Z}$, and $\set{W}$ denote four disjoint sets of random variables. The \emph{graphoid Axioms} $\mathcal{A}$ are the following:

{\noindent \emph{Symmetry}}: 
\[\set{X} \indep \set{Y} \mid \set{Z}  \quad \Longleftrightarrow \quad  \set{Y} \indep \set{X} \mid \set{Z}\]

{\noindent \emph{Decomposition}}: 	
\[
\set{X} \indep \set{YW} \mid \set{Z}  \quad  \Longrightarrow \quad 
\begin{cases}
\set{X} \indep \set{Y} \mid \set{Z} \\
\set{X} \indep \set{W} \mid \set{Z}
\end{cases} 
\]

{\noindent \emph{Weak Union}}:
\[\set{X} \indep \set{YW} \mid \set{Z}  \quad \Longrightarrow  \quad \set{X} \indep \set{Y} \mid \set{ZW}\]

{\noindent \emph{Contraction}}:
\[\big (\set{X} \indep \set{Y} \mid \set{Z} \big ) ~~ \& ~~ \big (\set{X} \indep \set{W} \mid \set{YZ} \big ) \quad \Longrightarrow \quad  \set{X} \indep \set{YW} \mid \set{Z}\]

% {\noindent \emph{Intersection}}:
% \[\big (\set{X} \indep \set{Y} \mid \set{Z}\big )  ~~ \& ~~  \big (\set{X} \indep \set{W} \mid \set{Z}\big ) \quad \Longrightarrow \quad   \set{X} \indep \set{YW} \mid \set{Z}\]
\end{Definition}

\noindent Note that $\set{Z}$ can be the empty set.
%thus the above axioms also hold without $\set{Z}$. 
For example, for the symmetry axiom, we have $\set{X} \indep \set{Y}   \Longrightarrow \set{Y} \indep \set{X}.$



\vspace{.5em}

{\noindent \bf An Inference System for \SCs.} Graphoid Axioms $\mathcal{A}$ are applicable to any conditional independence statement. Since this paper only considers those conditional independence statements with no more than three variables, we can simplify $\mathcal{A}$.
%and derive a new inference system $\mathcal{G}$. 

\begin{Definition}\label{def:new-inference}
Let $A$, $B$, $C$ denote three random variables. The inference system $\mathcal{G}$ for \SCs consists of the following %inference 
rules.

{\noindent \emph{Symmetry}}:
\[A \indep B \mid C  \quad \Longleftrightarrow \quad B \indep A \mid C \]
%\[A \indep B \mid C  \quad \Longleftrightarrow \quad B \indep A \mid C\]

{\noindent \emph{Contraction-weak-union-decomposition}}:
\[\big (A \indep B\big)  ~~ \& ~~ \big (A \indep C \mid B\big ) \quad \Longrightarrow \quad  
\begin{cases}
A \indep C \\
A \indep B \mid C
\end{cases}\]
\end{Definition}

We can prove that Definition~\ref{def:graphoid-axioms} and Definition~\ref{def:new-inference} are equivalent for \SCs involving at most three random variables. Therefore, we only need to consider the two inference rules in $\mathcal{G}$ rather than all the rules in $\mathcal{A}$. Lemma~\ref{lem:equivalence} formally proves their equivalence. 

\begin{Lemma}\label{lem:equivalence}
    For any set $\mathcal{I}$ of \SCs involving at most three random variables, and any single \SC $\gamma$, we have that
    (i) if $\mathcal{I} \vdash_{\mathcal{A}} \gamma$, then $\mathcal{I} \vdash_{\mathcal{G}} \gamma$;
    (2) if $\mathcal{I} \vdash_{\mathcal{G}} \gamma$, then $\mathcal{I} \vdash_{\mathcal{A}} \gamma$,
    where $\mathcal{I} \vdash_{\mathcal{A}} \gamma$ (resp. $\mathcal{I} \vdash_{\mathcal{G}} \gamma$) denotes that  $\mathcal{I}$ implies $\gamma$ using $\mathcal{A}$ (resp. $\mathcal{G}$).
\end{Lemma}

\begin{proof}
    All the proofs of this paper can be found in Appendix.
\end{proof}

%\oliver{maybe add extension to future work}

We next discuss the soundness and completeness of the new inference system $\mathcal{G}$. 

\vspace{.5em}

{\noindent \bf Soundness.} Graphoid Axioms $\mathcal{A}$ have been proved to be sound ~\cite{pearl2014probabilistic}. Since $\mathcal{G}$ and $\mathcal{A}$ are equivalent for \SCs (Lemma~\ref{lem:equivalence}), we conclude that $\mathcal{G}$ is also sound.

\vspace{.5em}

{\noindent \bf Completeness.} When Graphoid Axioms were first developed, they were conjectured to be a complete inference system ~\cite{pearl2014probabilistic}. In 1990s, Studeny proved that the conjecture ~\cite{studeny1990conditional} was {\em incorrect}. However, Studeny's proof assumes that each independence statement is allowed to contain an arbitrary number of random variables, thus it is still an open question whether the system $\mathcal{A}$ is complete under the assumption that each independence statement contains no more than three variables. For this reason, we conjecture that \emph{when each independence statement contains no more than three variables, Graphoid Axioms $\mathcal{A}$ are complete}. If the conjecture is true, Lemma~\ref{lem:equivalence} entails that $\mathcal{G}$ is complete.   %We defer to future work.  in this situation. Based on the conjecture, we can easily prove that $\mathcal{I}$ is complete using Lemma~\ref{lem:equivalence}. 

%\vspace{.5em}

%{\noindent \bf Remark.}


%Please note that the above axioms also hold when $\set{Z}$ is empty, i.e., removing $\set{Z}$ from the condition of each conditional independence. For example, for the decomposition axiom, we have 
%\[\set{X} \indep \set{YW}   \Longrightarrow \set{X} \indep \set{Y} ~~ \& ~~ \set{X} \indep \set{W}.\]




%{\noindent \bf Remark.} The Graphoid Axioms was conjectured to be both sound and complete~[Pearl's paper??]. However, in 1990, Studeny proved that it is not complete, and the author further proved that there does not exist a finite set of axioms that are complete~\cite{studeny1990conditional}. However, in this paper, we assume that each \SC has no more than three variables. It is still an open question that when each condition dependence has no more than variables, whether the Graphoid Axioms is complete or not. In this paper, 


%only sound but not complete, it is widely used in practice (e.g., multivariate modeling and causality analysis). Thus, in this paper, we only 



%Geiger and Pearl~\cite{pearl2} has showed for the conditional independence and marginal independence can be governed by a set of axioms under certain assumptions. The axiom is called \textbf{Graphoid Axioms} $\mathcal{A}$ and it is complete and sound~\cite{pearl1}. 






\subsection{Consistency and Implication} \label{subsec:consistency}
Being able to check whether a given set $\Sigma$ of \SCs is consistent or not is important because if  $\Sigma$ is not consistent, %when applying it to error detection, 
a user will get contradictory error-detection results. In the following, we first formally define the consistency problem, and then present a consistency-checking framework. In order to apply the framework, the key is to solve the implication problem. Therefore, we define the implication problem and propose an efficient implication algorithm. 
%
Intuitively, if $\Sigma$ is consistent, it means that $\Sigma$ has no conflict. That is, there exists a joint distribution that satisfies $\Sigma$. Definition~\ref{def:consistency} presents a formal definition.

\begin{Definition}[Consistency]\label{def:consistency}
Given a set $\Sigma$ of \SCs, let $\set{V}$ denote the set of random variables that appear in $\Sigma$. The consistency problem is to determine whether there exists a joint distribution $P(\set{V})$ that satisfies every \SC in $\Sigma$. 
\end{Definition}


\begin{figure}[t]
   \centering 
   \includegraphics[width=0.9\linewidth]{fig/joint-new.pdf} 
   \vspace{-1em}
   \caption{An example of a joint distribution that satisfies $\Sigma = \{A \indep B,\; A \nindep B| C\}$}\label{fig:joint}\vspace{-1.5em}
\end{figure}

For example, consider $\Sigma = \{A \indep B,\; A \nindep B| C\}$. Since there are three random variables in $\Sigma$, we have $\set{V} = \{A, B, C\}$. As shown in Figure~\ref{fig:joint}, we can construct a joint distribution $P(A, B, C)$ that satisfies $\Sigma$, thus $\Sigma$ is consistent. If we are given $\Sigma' = \{A \indep B,\; A \nindep B\}$, it is impossible to construct a joint distribution that satisfies $\Sigma'$, thus $\Sigma'$ is inconsistent. 

\vspace{.5em}

{\noindent \bf Consistency-checking Framework.} Geiger and Pearl~\cite{pearl2} proposed a framework to solve the consistency problem. They first divide $\Sigma$ into two disjoint sets $\mathcal{I}$ and $\mathcal{D}$, where $\mathcal{I}$ (resp. $\mathcal{D}$) represents the set of independence (resp. dependence) statements in $\Sigma$. For each $\lambda \in \mathcal{D}$, it checks whether $\mathcal{I}$ implies $\lnot \lambda$. If the answer is no for all $\lambda$, then $\Sigma$ is consistent; otherwise, it is not consistent. The correctness of the framework was proved in~\cite{pearl2}. For example, consider $\Sigma = \{A \indep B,\; A \nindep B| C\}$. We have $\mathcal{I} = \{A \indep B\}$  and $\mathcal{D} = \{A \nindep B| C\}$. We can see that $\mathcal{D}$ does not imply  $\lnot \lambda = A \indep B| C$, thus $\Sigma$ is consistent.    


\vspace{.5em}

To apply the above framework,
%to solve the problem in Definition~\ref{def:consistency}, the key challenge is how to efficiently check whether $\mathcal{I}$ implies $\lnot \lambda$ or not.  In other words, 
we aim to determine whether an independence \SC $\gamma$ can be inferred from $\mathcal{I}$ using $\mathcal{G}$.  Definition~\ref{def:implication} formally defines the implication problem. 

\begin{Definition}[Implication]\label{def:implication}
Given a set $\mathcal{I}$ of independence \SCs, and another independence \SC $\gamma$, the implication problem is to determine whether $\gamma$ can be inferred from $\mathcal{I}$ using $\mathcal{G}$, i.e., check whether $\mathcal{I} \vdash_{\mathcal{G}} \gamma$ holds or not.
\end{Definition}

{\noindent \bf Implication Algorithm.} We propose an iterative algorithm. The algorithm starts with $\mathcal{I}^* = \mathcal{I}$, and then iteratively expands $\mathcal{I}^*$ with new \SCs. At each iteration, the algorithm checks which inference rule in $\mathcal{G}$ can be used to generate a new \SC, and then adds it to $\mathcal{I}^*$. The algorithm terminates when $\mathcal{I}^*$ cannot be further expanded. After that, the algorithm checks whether $\gamma \in \mathcal{I}^*$ holds. If so, then $\mathcal{I}$ implies  $\gamma$; otherwise, $\mathcal{I}$ does not imply $\gamma$.

\begin{example}~\label{exa:implication}
Given a set of independence \SCs $\mathcal{I} = \{A\indep B, A \indep C | B, B\indep C,  C \indep E | D\}$ over attributes $M=\{A, B, C, D, \\
E\}$. To compute $\mathcal{I}^*$, we initially set $\mathcal{I}^* = \mathcal{I}$, and then apply the implication algorithm.

\noindent {\underline{Step 1: Constructing Hash Table}}. $H=\{\{A,B\},\{B,C\}\}$ will be generated according to the marginal \SCs  in  $\mathcal{I}^*$, i.e., $A \indep B$ and $B \indep C $.

\noindent {\underline{Step 2: Employing Inference System $\mathcal{G}$}}. We check each conditional \SC in $\mathcal{I}^*$. For $\SC_1:A \indep C | B $, we first check whether $\{A,B\}$ or $\{B,C\}$ exists. Obviously, we have both of them in the $H$. Applying the \emph{contraction-weak-union-decomposition} inference rule in $\mathcal{G}$, we can obtain three new \SCs: $A\indep B|C$, $B \indep C |A$, and $A \indep C$. We add them into $\mathcal{I}^*$, and hash $A \indep C$ as $\{A,C\}$ and add it into $H$. 

\noindent {\underline{Step 3: Repeating}}. Repeat Step 1 and Step 2 till there are no more \SCs that can be inferred. In this example, we eventually arrive at $\mathcal{I}^* = \{A\indep B, A\indep C, B\indep C, A \indep B|C, A \indep C | B, B \indep C |A,  C \indep E | D\}$. 

\end{example}

To analyze the time complexity of the implication algorithm, we answer two  questions:\\
\indent \emph{Q1. What's the time complexity of generating a new \SC?} \\
\indent \emph{Q2. How many new \SCs can be generated in total?}

\vspace{0.25em}

\noindent For $Q1$, consider the two inference rules in Definition~\ref{def:new-inference}. The algorithm first checks whether the symmetry rule can be used to generate a new \SC or not. The time complexity of this process is $\mathcal{O}(|\mathcal{I}^*|)$. For the contraction-weak-union-decomposition rule, a naive way is to enumerate every pair of \SCs in $\mathcal{I}^*$ and then check whether the rule can be used or not. It needs $\mathcal{O}(|\mathcal{I}^*|^2)$ time. In fact, we can utilize a hash table to reduce the time complexity to $\mathcal{O}(|\mathcal{I}^*|)$. Specifically, we build a hash table for marginal \SCs (e.g., $A \indep B$), and then for each conditional \SC (e.g.,  $A \indep C | B$), we check whether $A \indep B$ or $C \indep B$ exists in the hash table. %This avoids $n^2$ comparisons. In total, our algorithm needs $\mathcal{O}(|\mathcal{I}^*|)$ time to generate a new \SC at each iteration.      

\vspace{0.25em}





\noindent For $Q2$, we seek to compute an upper bound for the number of newly generated \SCs. The key observation is that for any inference rule in $\mathcal{G}$, its right-hand side will not introduce any new variable that is not on the left-hand side. For example, consider the contraction-weak-union-decomposition rule. The left-hand side has three variables $\{A, B, C\}$, and the right-hand side has the same three variables, without introducing any new variable.      


% \na{TO JN: do we need to like say, this observation is the coverage problem like CFD and DC said. }

Based on this observation, we find that there is a relationship between $|\mathcal{I}|$  and $|\mathcal{I}^*|$. That is, $|\mathcal{I}^*| \leq 12 |\mathcal{I}|$. If we consider symmetry \SCs (e.g., $A \indep B$ and $B \indep A$) are the same, then $|\mathcal{I}^*| \leq 6 |\mathcal{I}|$.  We give the intuition below, and provide a formal proof in Lemma~\ref{lem:upper-bound}. 

We say $\SC_1$ \emph{covers} $\SC_2$ if the variable set of $\SC_1$ is a superset of the variable set of $\SC_2$. %For example, suppose $\SC_1: A \indep B$. The variable set of $\SC_1$ is $\{A, B\}$. Then, it covers two different \SCs:
%\[A \indep B, \;\; B \indep A.\]
%\na{I changed a little bit of the example here, is it right?}
%
For example, suppose $\SC_1: A \indep B | C$. Then, it covers 6 different \SCs:
\begin{align*}
A \indep B,\;\; A \indep C,\;\; B \indep C,\;\; A \indep B | C,\;\; A \indep C | B,\;\; B \indep C | A
\end{align*}
The above observation implies the \SCs in $\mathcal{I}$ can cover all the \SCs in $\mathcal{I}^*$. Since each $\SC \in \mathcal{I}$ can cover at most 6 different \SCs, then we have that $|\mathcal{I}^*| \leq 6 |\mathcal{I}|$. Lemma~\ref{lem:upper-bound} formally proves this result.


\begin{Lemma}\label{lem:upper-bound}
Given a set $\mathcal{I}$ of independence \SCs, let $\mathcal{I}^*$ denote the set of all the independence \SCs implied from $\mathcal{I}$. Then, we have $|\mathcal{I}^*| \leq 6 |\mathcal{I}|$.     
\end{Lemma}

%\begin{proof}
%Sketch. Applying the axioms introduced in Definition.~\ref{def:new-inference}, we can find that the inference system cannot generate any further more information beyond variables involved. It can be proved by contradiction. Furthermore, we apply the combination theory, where there are $2 \binom{3}{2}$ possible outcomes. \end{proof} . 



%Since the implication algorithm needs at most $\mathcal{O}(|\mathcal{I}|)$  is $\mathcal{O}(|\mathcal{I}|^2)$. Next, we 


\vspace{.5em}

{\noindent \bf Consistency-checking Algorithm.} We can develop a consistency-checking algorithm using the implication algorithm. See the pseudo-code in Algorithm~\ref{alg:check}. The algorithm first computes $\mathcal{I}^*$. Then, for each $\lambda \in \mathcal{D}$, it checks whether $\lnot\lambda \in \mathcal{I}^*$ holds or not. If no for all $\lambda$, then $\Sigma$ is consistent; otherwise, $\Sigma$ is inconsistent. 

%there exists $\lambda \in \mathcal{D}$ such that $\lnot\lambda \in \mathcal{I}^*$, it means that $\mathcal{I}$ implies $\lnot\lambda$. Since $\lambda \in \mathcal{D}$, then $\Sigma$ is inconsistent. If there does not exist $\lambda  \in \mathcal{D}$ such that $\lnot\lambda \in \mathcal{I}^*$, then $\Sigma$ is consistent. 
% \na{To JN: do we need the pseudo-code algorithm for this?}


\begin{algorithm}[t]
	\caption{Consistency-checking Algorithm}\label{alg:check}
	\KwIn{A set of \SCs: $\Sigma$}
	\KwOut{Consistent or not (YES or NO)}
	\vspace{0.5em}
	Divide $\Sigma$ into $\mathcal{I}$ and $\mathcal{D}$\;
	Use the implication algorithm to obtain $\mathcal{I}^*$\;
	\For{$\lambda \in \mathcal{D}$}
	{
	    \If{$\lnot \lambda \in \mathcal{I}^*$}
	    {
	        {\bf return} NO\; 
	    }
	}
	{\bf return} YES\;
\end{algorithm}

\begin{example}
Given a set of \SCs $\Sigma=\{A\indep B, A \indep C | B, A \nindep C, B\indep C,  C \nindep D,  C \indep E | D, E \nindep F \}$, we check the consistency of $\Sigma$ as follows: 

\noindent {\underline{Step 1: Dividing}}.  Divide $\Sigma$ into $\mathcal{I} = \{A\indep B, A \indep C | B, B\indep C,  C \indep E | D\}$ and $\mathcal{D} =\{A \nindep C, C \nindep D, E \nindep F\}$;

\noindent {\underline{Step 2: Computing $\mathcal{I}^*$}}. By employing the implication algorithm on $\mathcal{I}$, we are able to acquire  $\mathcal{I}^*$. Similar to Example.~\ref{exa:implication}, we can obtain $\mathcal{I}^* = \{A\indep B, A\indep C, B\indep C, A \indep B|C, A \indep C | B, B \indep C |A,  C \indep E | D\}$. 

\noindent {\underline{Step 3: Checking the Implication}}. Check that whether there exists $\lambda \in \mathcal{D}$ such that $\lnot\lambda \in \mathcal{I}^*$ holds. We see that $\lnot\lambda: A \indep C$ is in $\mathcal{I}^*$, thus $\Sigma$ is inconsistent. 
\end{example}


{\noindent \bf Time Complexity.} The implication algorithm needs $\mathcal{O}(|\mathcal{I}^*|)$ iterations, and each iteration needs $\mathcal{O}(|\mathcal{I}^*|)$ time. The total time complexity is $\mathcal{O}(|\mathcal{I}^*|^2) = \mathcal{O}((6|\mathcal{I}|)^2) = \mathcal{O}(|\mathcal{I}|^2)$. For the consistency-checking algorithm, the main bottleneck is spent in running the implication algorithm to compute $\mathcal{I}^*$ (see Line 2 in Algorithm~\ref{alg:check}), thus the total time complexity is $\mathcal{O}(|\mathcal{I}|^2)$.


\vspace{.5em}


{\noindent \bf Resolving Inconsistency.} Once an inconsistency is detected, we help the user to resolve the inconsistency.  Specifically, suppose the consistency-checking algorithm finds a conflict: $\mathcal{I}$ implies $A \indep B$ but $A \nindep B$ is in $\Sigma$. We ask the user to check which one is correct. If the former is correct, then $A \nindep B$ should not be in $\Sigma$, and we remove $A \nindep B$ from $\Sigma$. Otherwise, we show the derivation of $A \indep B$  from $\mathcal{I}$ and then ask the user to remove the incorrect \SCs involved in the derivation.   















\iffalse 
    













\subsection{Implication Problem} \label{subsec:implication}



\subsection{Consistency and Implication}


\subsection{Consistency Checking Problem}

\iffalse
\begin{Definition}[Consistency]
	A set of Statistical Constraints $\SC$ is \defterm{consistent} if and only if there exists a probability distribution $\prob$ that satisfies all (in)dependence statements in $\SC$. We use $\SC \sim \mathbb{P}$ to denote this. \oliver{a bit unusual notation, maybe check Pearl's or other papers. update: Pearl uses subscript notation Ch. 3.1., so maybe this is okay.} 
	%If there is no probability distribution $\mathbb{P}$ satisfies the statistical constraints $\Sigma$, we say that the set $\Sigma$ is not consistent, or the statistical constraints has the consistency violation. 
\end{Definition}
\fi


\subsection{Efficient Consistency checking}

In this section, we present an algorithm for checking the internal consistency of a set of constraints~\cite{cck}. The most general version of the consistency problem is known to be \oliver{undecidable?}. Our algorithm works in the case where statistical constraints are limited to 3 variables. While this is a strong assumption, it covers a range of natural (in)dependence constraints, sufficient for us to evaluate the efficacy of our approach for data cleaning. Under future work we discuss a number of ways in which the limitation to 3 variables can be overcome. 
Based on previous inference system, we construct a new system ~\ref{inference} to solve the consistency checking problem introduced in ~\ref{cck}. 
 %And we further extend to support all statistical constraints(Sec.~\ref{extension}). 
 
 \oliver{I'm confused about two things. 1) If we assume 3 variables only, do we need any axioms? 2) I would think Geiger and Pearl look at implication only, not consistency. They usually look at independence statements only which are always consistent.}
 
 \na{Yes, we still need the axioms for the inference. Since we omit one and compress another two axioms.}


%We further investigate the fundamental problem: Consistency Checking problem (Sec.~\ref{}), and propose a new inference system and algorithm to support Statistical Constraints introduced in this paper(Sec.~\ref{inference}, Sec.~\ref{checking}), and we further extend to support all statistical constraints(Sec.~\ref{extension}). 
%In this section, we propose the problem on consistency checking. We first give the problem definition of consistency checking. Later, we provide the solution to this problem. We show that our algorithm can bound the time complexity to $O(n^2)$. Furthermore, we provide a method to repair the statistical constraints under certain budget. 


%\subsection{Consistency and Consistency Checking}

% The consistency and implication are two fundamental properties in Statistical Constraints, and are proposed in ~\cite{pearl2,Banjo,pearl1}. The consistency measures the agreement between constraints, that is whether there exists any contradiction between constraints. The implication between statistical constraints is whether the given statistical constraints can entail other statistical constraints. 



A key observations here is that, if we are given the set of random variables, $U=\{x_1,x_2,x_3,...\}$, the maximum number of constraints over $U$ is bounded. 

\begin{Lemma}[Consistent Constraints Bound]
	Given a set of constraints $\Sigma$ following the input in this paper, the maximum number of $|\Sigma|$  is  $\frac{n(n-1)(n-2)}{2}$.
\end{Lemma}

\na {TO JN: Do we need to have a motivation example here? To highlight the significance of this problem, just use the example in the slides? }

\quad Consistency problem of independence problem is first proposed by Dan Geiger and Judea Pearl~\cite{pearl2} in 1992. The formal definition of the consistency given the set of statistical constraints is below.

\begin{Problem}[Consistency Checking]
	Given a set of statistical constraints $S$ over set of variables $X$, whether $S$ is consistent or not.
\end{Problem}

Obviously, to solve this problem, we need to find whether there are some contradictory between statistical constraints. A observation here is that simply check the constraints between the independence set $I$ and the dependence set $D$ is not applicable since the statistical constraint have the capacity to entail other statistical constraints. Therefore, we need an inference system to infer all constraints that can be entailed by the given constraints. 



\subsection{A new Inference System for SCs} \label{inference}

% The implication between statistical constraints is whether the given statistical constraints can entail other statistical constraints.
~\cite{ pearl2} has showed for the conditional independence and marginal independence can be governed by a set of axioms under certain assumptions. The axiom is called \textbf{Graphoid Axioms} $\mathcal{A}$ and it is complete and sound~\cite{pearl1}.  

However, in this paper, our statistical constraints is a special type of the independence and dependence. Under the same assumption in ~\cite{pearl1}, we introduce our new axioms and prove it is complete and sound. 
\begin{Definition}[Graphoid Axioms $\mathcal{A}$]
	Let $X$, $Y$ and $Z$ be three random variables, and $W$ be the further variable. The following conditions hold for the independence relationship 
\end{Definition}	
	
	Symmetry: 
\begin{equation}
 			 I(X,Z,Y) \longleftrightarrow I(Y,Z,X)
\end{equation}
	
	Decomposition: 
\begin{equation}
      I(X,Z,Y\cup W) \longrightarrow I(X,Z,Y)  \quad \& \quad  I(X,Z,W) 
\end{equation}

	Weak Union: 
\begin{equation}
    I(X,Z,Y\cup W) \longrightarrow I(X,Z\cup W,Y)
\end{equation}

  Contraction: 
\begin{equation}
	I(X,Z,Y) \&  I(X,Z\cup W,Y)  \longrightarrow I(X,Z,Y\cup W)
\end{equation}

	Intersection:
\begin{equation}
	I(X,Z,Y)  \quad \& \quad  I(X,Z,W) \longrightarrow   I(X,Z,Y\cup W) 
\end{equation}

The $\mathcal{A}$ here is applicable for all independence relationship. However, considered our statistical constraints(no more than three variables for one constraint), it is not that useful since some of  for our statistical constraints is not applicable to  them.


The below we introduce our new Graphoid Axioms $\mathcal{A^+}$.

\begin{Definition}[New Graphoid Axioms $\mathcal{A^+}$]
	Let $X$, $Y$ and $Z$ be three random variables, and $W$ be the further variable. The following conditions hold for the independence relationship 
\end{Definition}	

Symmetry: 
\begin{equation}\label{sym}
	I(X,Z,Y) \longleftrightarrow I(Y,Z,X)
\end{equation}

Contraction-union-decomposition: 
\begin{equation}\label{con}
\begin{split}
	I(X,\varnothing,Y) \&  I(X,Y,W) \longleftrightarrow & I(X,\varnothing,Y\cup W) \\ \longrightarrow & I(X,\varnothing, Y)  \&  I(X,\varnothing,W) \\&   I(X,Y,W)  \&  I(X,W,Y) 
\end{split}
\end{equation}

%Intersection-union-decomposition: 
%\begin{equation}\label{in}
%\begin{split}
%I(X,Y,W) \&  I(X,Y,W) \longleftrightarrow & I(X,\varnothing,Y\cup W) \\ \longrightarrow & I(X,\varnothing, Y)  \&  I(X,\varnothing,W) \\&  I(X,\varnothing,Y) \&  I(X,Y,W)
%\end{split}
%\end{equation}
%
%If we combine the equation \ref{con} and equation \ref{in}, we can have a new axiom to replace the two. 
%
%\begin{equation}\label{in}
%\begin{split}
%I(X,Y,W) \&  I(X,Y,W) & \longleftrightarrow  I(X,\varnothing,Y\cup W) \\&   \longleftrightarrow  I(X,\varnothing,Y) \&  I(X,Y,W) \\ &  \longrightarrow I(X,\varnothing, Y)  \&  I(X,\varnothing,W) 
%\end{split}
%\end{equation}



\begin{Conjecture}[Pearl's Conjecture]
	In this paper, we follow Pearl's conjecture that the graphoid axiom system is complete and conjecture. ~\cite{pearl1}
\end{Conjecture}

     Also, we find that New Graphoid Axioms $\mathcal{A^+}$ is also complete and sound under Pearl's Conjecture. 
    
     To show that our conclusion is right, we first introduce the following lemma.
     
     \begin{Lemma}\label{bound}
     	The number of new constraints that can be inferred from one single Statistical Constraint is $6$ at most.
     \end{Lemma}
     
     \begin{proof}
     	Nathan to do
     \end{proof}
     
     
     Based on Lemma ~\ref{bound}, we then formally prove our conjecture. 
     
\begin{Theorem}~\label{com}
	New Graphoid Axioms $\mathcal{A^+}$ is sound and complete under Pearl's Conjecture.
\end{Theorem}

\begin{proof}
	Nathan TO DO
\end{proof}


\subsection{Efficient Consistency Checking algorithm with $\mathcal{A^+}$ }~\label{checking}

In this section, we further show an efficient checking algorithms with the new inference rule $\mathcal{A^+}$.

\oliver{I thought we were assuming 3 variables only?}

\begin{algorithm}[h]\label{check}
	\caption{Efficient Consistency Checking }\label{algorithm: bcc}
	\KwIn{A set of Independence Constraints $I$, A set of Dependence constraints $D$, Inference system $A$}
	\KwOut{Consistent or not (YES or NO)}
	%	$G \leftarrow \emptyset$ \;
	$S \leftarrow I$\;
	$E \leftarrow \emptyset $ \;  
	$Con \leftarrow 0$ \;
	%	$E \leftarrow \emptyset$ \;
	\For{each constriaints in $I$}
	{
		Add marginal constraints into $E$ \;
		Remove marginal constraints from $I$ \;
	}
	
	\For{each $a$ in $E$}
	{
		\For{each $b$ in $I$}
		{
			\If{$a$ matches $b$ by $A$}
			{
				Infer new constraints from $a$ and $b$ by $A$ \;
				Add new constraints into $S$ \;
				Add new marginal constraints into $E$ \;
			}
			remove $a$ \;
		}	
	}
	\If{$S \cap D^c = \emptyset$}
	{
		$Con \leftarrow 1$ \;
	}
	Return $Con$
\end{algorithm}

\subsection{Extension Algorithm}~\label{extension}
\na{To Oliver: refer to Oliver's work} 


\subsection{Summary} \label{sum}

\fi

==> experiments-old.tex <==
\section{Experiments}\label{sec:exp}

% \begin{figure}[t]
%   \centering 
%   \includegraphics[scale=0.45]{fig/exp/scs_check/efficiency.eps} 
%   \vspace{-2em}
%   \caption{Time for Consistency Checking of \SCs (``0.5 Times'' means that the ) \label{fig:scs_check}\vspace{-2em}
% \end{figure}


\begin{table*}[h]\label{tab:con_summary}
 \centering
 \caption{Constraints Used by Different Error Detection Methods } 
 %\setlength\tabcolsep{3.5pt}
   \begin{tabular}{|c|c|c|}
   \hline
       \textbf{Attributes} & \textbf{CODED} & \textbf{Denial  Constraints} \\ \hline
   \hline
    Home Value(H), Black Index(B) & $H \indep B$ &  N/A\\ \hline
    N\_oxide(N), Distance(D) & $N \nindep D$ & \specialcell{}{For any two records, if N value of one is larger, \\ its D value shall be smaller than another one}\\ \hline
%     For any two records, if the N of one is larger, \\
%   \hline
  N, B, Tax rate (T) & $N \indep B ~|~T$ & N/A \\ \hline
  T, B, Crime(C) & $T \nindep B~ |~C$ & \specialcell{}{When $C = c$, For any two records, if T value of \\ one is larger, its B value shall be smaller than another one}\\ \hline
   \end{tabular}%
\end{table*}%

\begin{figure}[t]
   \centering 
   \includegraphics[scale=0.36]{fig/exp/scs_check/efficiency_new.eps} 
   \vspace{-1em}
   \caption{Time for Consistency Checking of \SCs 
%   \oliver{should that be divided by 10?}\na{it will be congested}
   }\label{fig:scs_check}\vspace{-1em}
\end{figure}


\begin{figure}[t]
  \centering 
  \includegraphics[scale=0.5]{fig/exp/cat/var_k_cat.eps} 
  \vspace{-1em}
  \caption{Effectiveness of Error Detection Methods for  of Categorical dataset}\label{fig:score_cat}\vspace{-1em}
\end{figure}


\begin{figure}[t]
   \centering 
   \includegraphics[scale=0.23]{fig/exp/Scalability/Scalability.eps} 
   \vspace{-1em}
   \caption{Scalability of Fast CODED \SCs 
%   \oliver{is one quantity fixed in the other plot? e.g. K = ? for number of records?}\na{Yes, we gonna wirte these parts in the efficiency section}
   }\label{fig:scalability}\vspace{-1em}
\end{figure}



\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.39]{fig/exp/error_impact/error_impact_indep.eps} 
   \vspace{-2em}
   \caption{Different Error Impact on Independence \SCs}\label{fig:imp_indep}\vspace{-2em}
\end{figure*}



\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.39]{fig/exp/error_impact/error_impact_dep.eps} 
   \vspace{-2em}
   \caption{Different Error Impacts on Dependence \SCs.}\label{fig:imp_dep}
\end{figure*}



\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.6]{fig/exp/sync_files/var_k_dep.eps} 
   \caption{Effectiveness of Error Detection Methods for Dependence \SCs}\label{fig:dep_var_k}\vspace{-2em} \label{fig:dep_bar_chart}
\end{figure*}


\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.6]{fig/exp/sync_files/var_k_indep.eps} 
   \caption{Effectiveness of Error Detection Methods for Independence \SCs}\label{fig:indep_var_k}\vspace{-2em}\label{fig:indep_bar_chart}
\end{figure*}



\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.69]{fig/exp/sync_files/dep_var_k.eps} 
   \vspace{-1em}
   \caption{Effectiveness of Error Detection Methods for Dependence \SCs}\label{fig:dep_score}\vspace{-1em}
\end{figure*}


\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.69]{fig/exp/sync_files/indep_var_k.eps} 
   \vspace{-1em}
   \caption{Effectiveness of Error Detection Methods for Independence \SCs}\label{fig:indep_score}\vspace{-1em}
\end{figure*}


\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.69]{fig/exp/sync_files/dep_var_k_condition.eps} 
   \vspace{-1em}
   \caption{Effectiveness of Error Detection Methods for Conditional Dependence \SCs}\label{fig:dep_score_condition}\vspace{-1em}
\end{figure*}

\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.69]{fig/exp/sync_files/indep_var_k_condition.eps} 
   \vspace{-1em}
   \caption{Effectiveness of Error Detection Methods for Conditional Independence \SCs}\label{fig:dep_score_condition}\vspace{-1em}
\end{figure*}



\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.45]{fig/exp/real_world/real-world.eps}
   \vspace{-2em}
   \caption{Detecting Real-world Error in \emph{Sensor}\oliver{why the big difference in recall vs. precision? And what is precision?: Answer: we draw $K$ from a fixed number of error record, e.g. 400}}\label{fig:sensor}\vspace{-2em}
\end{figure*}


In this section, we evaluate the effectiveness and efficiency of our methods on real-life datasets with both synthetic errors and real-world errors. Specifically, we examined (1) the computational efficiency of the consistency-checking methods, (2) the effectiveness of our method compared to the state-of-the-art approaches on detecting synthetic and real-life errors, and (3) the scalability of our error-detection method.

%By these experiments, we examined  our algorithms, and discovered limitations  %of our methods for further improvement. 

\subsection{Experiment Setup}
\noindent \textbf{Datasets.} We used four real-life datasets with both simulated and real errors.

(1) {\tt BOSTON\footnote{\scriptsize https://www.cs.toronto.edu/~delve/data/boston/bostonDetail.html}.} The Boston dataset was taken from the Boston Standard Metropolitan Statistical Area (SMSA) in 1970. This dataset was first used in~\cite{Harvard} to study the relationship between clean air quality and household's willing to pay. There are 506 instances, and each instance has 14 attributes like Distance to CBD area (DT), Nitric Oxides Concentration (NR), and Crime Rate (CR).

(2) {\tt CAR\footnote{https://archive.ics.uci.edu/ml/datasets/Car+Evaluation.}.} Car Evaluation dataset is from UCI Machine Learning repository. This dataset contains seven attributes like buying price, maintainence price and safety level. 

(3) {\tt SENSOR\footnote{http://db.csail.mit.edu/labdata/labdata.html}.} The Sensor dataset collected the sensor reports from Intel Lab. The dataset has more than 2 million records, containing the humidity and temperature reports from 54 different sensors. %There are more than 2 million records in the dataset. This dataset~[???] has been widely used in data error detection, data repairing, and data curation.

(4) {\tt HOCKEY\footnote{https://github.com/liuyejia/Model\_Trees\_Full\_Dataset}}. The Hockey dataset collected the records of each NHL game from 1998-2010. It has more than ten attributes which variously describe player attributes and player performance statistics for a season. 
%the critical information of the game, player performance, and etc.

\vspace{.25em}


\noindent \textbf{Simulated Errors.} In Section~\ref{sec:intro}, we introduced two types of errors: \emph{sorting error} and \emph{imputation error} (see Figure~\ref{fig:car-error}). We simulated them on the Boston dataset.   


To simulate the \emph{sorting} error on column $A = \{a_1, a_2, \cdots, a_n\}$, we first select a sub-sequence of $A$, then sort them in an ascending order, denoted by $A' = \{a'_i, \cdots, a'_j\}$ ($a'_i \leq a'_{i+1} \leq \cdots \leq a'_j$). Finally, we put the sorted values back to the original column, i.e., $\error{A} = \{a_1, \cdots, a_{i-1}, a'_i, \cdots, a'_{j}, a_{j+1}, \cdots, a_n\}$. We say that $\error{A}$ has sorting error with the error rate of $\frac{j-i+1}{n}$. Note that the sorting error can either make two columns more dependent or more independent: Consider another column $B$. If the original data is randomly shuffled, then $\error{A}$ and $B$ will become more independent; if the original data is sorted by $B$, then $\error{A}$ and $B$ will be more dependent. We use the former for dependence, the latter for independence \SCs.

To simulate the imputation error on column $A = \{a_1, a_2, \cdots, a_n\}$, we assume that $A$ has a set of $m$ missing values (i.e., error rate = $\frac{m}{n}$), and the missing values are replaced by the mean value of column $A$. Let $\error{A}$ denote the new column. Like the sorting error, the imputation error can either make two columns more dependent or more independent. Consider another column $B$. If the missing values are randomly selected, $\error{A}$ and $B$ will become more independent; if the missing values are selected based on a range condition on $B$ (e.g., the temperature readings are missing between 10 AM and 11 AM), $\error{A}$ and $B$ will become more dependent. We use the former (latter) for dependence (independence) \SCs. 
\oliver{would be nice to have an example here}\na{TO JN: Shall we have an example here?}

In addition, we explored the impact of combination of the two error types given that in practice, the combination of errors is not rare. We call it \emph{combination error}, which consists of 80\% sorting error and 20\% imputation error.  



%occurs when a data scientist sorted data points by one column to see the tendency but forgot to reverse the process. 
%The result is that one column is sorted but others remain random or same. We consider two sorting situations: (1) Single sorting: the data scientist just sorted one column and didn't revert it back; (2) she sorted the entire dataset by columb $b$, and then she further took a look at the order of column $a$; 

%which can not be matched with other column values. 
%Missing values  are ubiquitous. Usually data analysts choose one standard imputation method to fill in the missing value. However, these imputation methods sometimes introduce errors that violate statistical constraints. We consider an imputation method that fills in missing values with a constant, like the mean, maximum or minimum value. In our experimental evaluations, we choose the mean value for the imputation. 
%in the data consistent with the given dataset. T
%This error type is called ~\emph{Imputation} error. We examined the Sorting error and Imputation error. 

%In addition, we also explored the impact of combination of the two errors given that in reality, the combination of errors is not rare. 
%and bring more tough challenges. 

\vspace{.25em}

\noindent \textbf{Real-life Errors.} For the \emph{sensor dataset}, we adopted the methods that~\cite{mayfield2010eracer} and~\cite{jeffery2006declarative} used to obtain the ground truth errors. First of all, we aggregate the mean value of sensor reports by hours. Reported mean temperatures larger than 60 degrees or lower than 15 degrees can be assumed to be erroneous.  We throw away these values, and use  mean value imputation to fill them in. Furthermore, we mark outliers by keeping a time window of neighboring sensors: in this time window, the reports from sensors should not deviate by more than a factor of 3 from the region's mean value. %By these steps, we define the ground truth errors for the sensor dataset. 

For the ~\emph{hockey dataset}, the dataset creators performed imputations to support machine learning analysis. The imputations are found by comparing their dataset with the original data from hockey data websites. 
%There are many missing/empty entries in the original dataset, therefore we can easily get these ground truth. 

\vspace{.25em}

\noindent \textbf{Error-Detection Approaches.} We compared the effectiveness of error-detection across three approaches: CODED, Denial Constraints(DC)~\cite{chu2013discovering}, and DBoost~\cite{mariet2016outlier}. For the CODED hypothesis testing, we used $\chi^2$ for categorical data, and Kendall's $\tau$ for numerical data. We implemented the error-drill-down framework, and adopted the $K$ strategy for dependent \SCs and the $K^c$ strategy for independent \SCs. We also implemented DC based on ~\cite{chu2013discovering}. We construct the denial constraints as shown in Table~\ref{tab:con_summary} and count the DC violations of each tuple. Sorting these tuples by the count of violations, and return $K$ records. For the DBoost, to make sure we can obtain a key value, and the model can work, we set the mixture n$\_$subpops threshold to be $3, 0.001$, and statistical epsilon to be $0$. 

\vspace{.25em}

\noindent \textbf{Quality Measurement.} We used \emph{Precision@K}, \emph{Precision}, and \emph{Recall} to measure the quality of error-detection approaches. \emph{Precision} is the ratio of the number of correctly detected records to the number of total returned records,  \emph{Recall} is the ratio of the number of correctly detected records to the number of total erroneous records. \emph{Precision@K} is the precision among the \emph{k} returned records. 

 

\subsection{Experimental Results}
% \oliver{order of figures doesn't match discussion - is that deliberate?}
% \na{It can be fixed later easily.}
\noindent \textbf{\underline{{Exp-1: Efficiency of Consistency Checking.}}}
We examined the efficiency of the consistency-checking algorithm. Note that the consistency checking is {\em not} related to data. Therefore, randomly generating \SCs is appropriate to test the scalability of our %efficient 
consistency-checking algorithm. We randomly generated $|\mathcal{I}|$ independence \SCs and $|\mathcal{D}|$ dependence \SCs from $|\mathcal{D}|/2$ variables. We measured the runtime of consistency checking by varying $|\mathcal{I}|$ and $|\mathcal{D}|$, respectively. The results are shown in Figure~\ref{fig:scs_check}. Each figure has three lines, which represent different ratios of $|\mathcal{I}|$ to $|\mathcal{D}|$.


We make two interesting observations. First, our consistency-checking algorithm scales well by varying either $|\mathcal{I}|$ or $|\mathcal{D}|$. Even with 500 independence (dependence) \SCs, the algorithm can terminate within 0.5 ms. Second, the efficiency is more related to $|\mathcal{I}|$ than $|\mathcal{D}|$. This is because the consistency-checking algorithm proposed comprises two parts: implication and checking, where the implication algorithm needs $\mathcal{O}(|\mathcal{I}^2|)$ time, which typically dominates the whole process.


%The $x$-axis is the number of total constraints or variables, and the $y$-axis is the running time in 100 msec.

%\noindent \textbf{Random rules generation.} To study the efficiency of the consistency checking algorithms, we randomly generate rules for testing. It is worth attention that the consistency checking is {\em not} related to the data. Therefore, randomly generating rules is applicable for testing the scalability of efficient consistency checking approach. The efficiency of the consistency checking algorithm is determined by the \# of constraints, and the ratio between independent \SCs and dependent \SCs. Also, according to Lemma ~[,,,], the \# of attributes may increase computational cost. Therefore, we evaluated the following three different situations.


%\noindent \underline{\emph{Varying the \# of independent and dependent \SCs.}} Algorithmically, the \# of \SCs will dominate the time in computation. The consistency checking algorithm proposed comprises two parts: implication and checking. Different \# of independent \SCs and dependent \SCs can help reveal which type of \SCs and even which part of the algorithm needs more time computationally. 

%\noindent \underline{\emph{Varying the \# of attributes.}} Since the \# of attributes bounds the possible \SCs, it is also necessary to study the influence of \# of attributes. 

%\noindent \underline{\emph{Varying the ratio of independent \SCs and dependent \SCs.}}  We compared the ratio of independent \SCs and dependent \SCs. We want to examined the majoring influence while resolving the inconsistency.

%As shown in Fig.~\ref{fig:scs_check}, more \SCs lead to more processing time.  Interestingly,  the \# of independent ~\SCs has only a slight impact on run time (Fig.~\ref{fig:scs_check}a. In contrast, varying the \# of {\em dependent} \SCs has a dramatic impact, as does varying the number of attributes (Fig.~\ref{fig:scs_check}b and c). 
%Combine the two above, it can be inferred, the increase \# of \SCs and attributes, particularly the \# of independent \SCs will cost more computation time. 
%One principal reason is that the implication algorithm, which needs at most $|\mathcal{I}^*|$ where the $|\mathcal{I}^*|$ is the number of independent ~\SCs. Intuitively, the number of independent \SCs will afect the final result. 
 
\vspace{.25em}


\noindent \textbf{\underline{Exp-2: Impact of Errors.}}
To illustrate the impacts of data errors on independence and dependence relationships among variables, we varied the rates of sorting error, imputation error, and combination error, %respectively, 
and tested how the $\tau$ value changed accordingly. The results are shown in Figure~\ref{fig:imp_indep} and Figure~\ref{fig:imp_dep}.

Figure~\ref{fig:imp_indep} shows the results w.r.t. an independence \SC. Generally, all the errors tend to raise the tau value, indicating a violation of the independence \SC. The sorting error brings consistent side effects on the tau value (Figure~\ref{fig:imp_indep}(a)). Imputation error has a strong negative impact at lower error rates, then the tau value reverses (Figure~\ref{fig:imp_indep}(b)). This can be explained as follows. Starting with independent data, imputing a constant value induces correlations among the two columns, as many data points are assigned the same value for both. Once many data points have been imputed with a constant value, the correlation decreases until one column contains the same constant everywhere, implying zero correlation between them. 

Figure~\ref{fig:imp_dep} shows the results for a dependence \SC. We can see that as more errors were generated, the $\tau$ value decreased, i.e., the columns became more independent. With the error rate at 0.8, the $\tau$ value approached zero, indicating an independence relationship.   


Figures~\ref{fig:imp_indep}(a) and (b) show that with small error rates, the $\tau$ value remained small (e.g., within [0,0.3]). In this situation, although no violation will be detected, CODED can still achieve high error-detection performance with the help of the proposed error-drill-down framework, which we examine in the next experiment. 
%(see the results in the next experiment).

%ccor examined the impact of different type of errors, including the sorting error and missing value imputation. We mainly studied two types of errors: \emph{sorting} and ~\emph{poor missing value imputation}. We want to evaluate the impact of two errors and the whether default hypothesis test methods are sensitive to these errors.

%We evaluated the impact of different error types on the tau value, our default statistic for assessing statistical constraints on a dataset. 
% Tau value, the key statistics in the hypothesis testing~[???]. Tau value is able to show the correlation of the data. Therefore, with the increase of error rate, we evaluated the how influential the error impact could be in two different types of \SCs. 
%Noted that~\emph{not independent} indicates two situations: ~\emph{positive correlated} and ~\emph{negative correlated}. We also evaluated the error impact on both two situations. 


%Generally, all the errors tend to raise the tau value, indicating a violation of the statistical independence constraint. The sorting error brings consistent side effects on the tau value in among different ~\SCs (Fig.~\ref{fig:imp_indep} (a)) \oliver{what is rooms/black index?}. Imputation error has a strong negative impact at lower error rates, then the tau value reverses (Fig.~\ref{fig:imp_indep} (b)). This can be explained as follows. Starting with independent data, imputing a constant value induces correlations among the two columns, as many data points are assigned the same value for both. Once many data points have been imputed a constant value, the correlation decreases until both columns contain the same constant everywhere, implying zero correlation between them. 

%\noindent \textbf{Error types.} \emph{Sorting} error occurs when a data scientist sorted data points by one column to see the tendency but forgot to reverse the process. 
%manipulated the sorting operation on one column but didn't reverse the process. 
%The result is that one column is sorted but others remain random or same. We consider two sorting situations: (1) Single sorting: the data scientist just sorted one column and didn't revert it back; (2) she sorted the entire dataset by columb $b$, and then she further took a look at the order of column $a$; 

%which can not be matched with other column values. 
%Missing values  are ubiquitous. Usually data analysts choose one standard imputation method to fill in the missing value. However, these imputation methods sometimes introduce errors that violate statistical constraints. We consider an imputation method that fills in missing values with a constant, like the mean, maximum or minimum value. In our experimental evaluations, we choose the mean value for the imputation. 
%in the data consistent with the given dataset. T
%This error type is called ~\emph{Imputation} error. We examined the Sorting error and Imputation error. 

%In addition, we also explored the impact of combination of the two errors given that in reality, the combination of errors is not rare. 
%and bring more tough challenges. 




% negative impact which, however, is not as strong as the Sorting error. More obviously, in Fig.~\ref{fig:imp_indep} (b), the impact brings by Imputation is uneven in independent \SCs group. \oliver{b) looks weaker than a) at first. then it reverses. Needs more discussion.}

% Surprised thought this can be explained in this way: Take the ultimate situation as an example, we get all tied tuples which means all the tau value is equal to 0. The Imputation error works in that way since the imputed error are the same value, like the mean value, one random value or maximum value. Therefore, the same value finally will make the tau value to be 0. Starting from nearly perfect independent, and with the increase of  error rate, the tauv value would turn to be 0 again. Hence it is reasonable to conjecture such error will make the value to be less independent, however, be more independent eventually. 

%Another subtle explanation is that there is no positive independent or negative independent. Errors could make the dataset less independent: more positive correlated or negative correlated. Cancellation of errors will alleviate the impact brought. \oliver{needs review}

%For the combination errors, since the ratio of sorting error to Imputation error is 4:1, the sorting error effect dominates the Imputation effects.
% it is possibly that impact induced by missing value and errors dominated the error impact over the dataset. That explains why though the impact of Imputation error is not constant, the sorting error shields the shadow on the dataset. 


%In summary, the sorting error and Imputation error can induce correlations that violate independence constraints, and the tau statistic detects the violation.

% We examined the effectiveness of CODED compared to two baselines: DC-clean and DBoost. 

\vspace{.25em}

\noindent \textbf{\underline{Exp-3: Evaluation of Error-Detection Approaches.}} We compared CODED with existing error-detection methods on the Boston dataset for three types of errors. For dependence \SCs, we compared with Denial Constraint (DC) and DBoost; for independence \SCs, since DC cannot express independence relationships, we compared only with DBoost. We considered all four common templates of \SCs: (1) $A \indep B$; (2)$A \nindep B$; (3) $A \indep B~ | ~C$ ; (4) $A \nindep B ~|~ C$, where $A$, $B$, and $C$ are three columns. Furthermore, the dependent and independent relationship among columns are from~\cite{Harvard}. 
% \oliver{nice}
% and a dependency model trained by ready probabilistic models. ,%\oliver{would be nice to make this more visual like a table}

%\na{To JN: do we need a table describing the meaning of selected columns?}

\noindent \underline{$A \indep B$ and $A \nindep B$.} We picked the \emph{Black Index} and \emph{N Oxide} from the Boston dataset since they are independent, we also picked \emph{Distance} and \emph{N Oxide} from Boston dataset as they are dependent.  \oliver{why only Boston?}\na{You think it is necessary to have more datasets in this section? We already have four datasets, one for simulate errors, one for categorical, and two for real-world. } We picked the \emph{Distance} and \emph{N Oxide} from the Boston dataset since they are dependent. Based on the observation, the error level can be grouped into three levels: \emph{minor error} where the ratio of errors varies from $1\%$ to $20\%$, \emph{moderate error} where the ratio of errors varies from $20\%$ to $45\%$, and \emph{major error}where the ratio of errors is usually larger than $50\%$. Results are shown in figure.~\ref{fig:dep_bar_chart} and figure.~\ref{fig:indep_bar_chart}.  Mostly, for all three methods, the precision increases as the error level increased. It is easy to understand, since when there is the large portion of errors, the dependence or independence relationship will be changed more dramatically, and it is easier for CODED and other methods to detect them. When there are minor errors, all three methods fail to detect them above precision$=0.5$ averagely. This implies when there are minor errors, the relationship defined by \SCs will not be changed so much. This means, the influence of entailed by these errors didn't dominate the original one. It is reasonable that all three methods didn't perform well under this setting. With the increase of errors, the precision of all three methods increases as well. For the error type, three methods perform better under sorting error and combination error, however, they are not that good in detecting error when the error is imputation error. This phenomena is more obvious when it come to CODED with conditional independent \SCs. In fig.~\ref{fig:indep_bar_chart} (b), we can find that all methods didn't perform well compared to other settings. \na{Do we need to explain why figure 9 (b) all methods doesn't perform well? It is like a dramatically down}. One reason is that influence aroused by imputation error was not always 

As recall describes the ratio of error detected in context of total errors. Given we set $K=50$, so the recall will naturally decrease with the increase with errors. That is the reason why recall keep going down when there are more simulated errors inserted. 

CODED outperforms both DC and DBoost in three different error levels, different error types and different \SCs. \na{Do we need to explain why other methods didn't perform well?}

Meanwhile, we also evaluate the effectiveness (f-score) varying the $K$ value to see how f-score changes under different $K$ values. Results are shown in fig.~\ref{fig:dep_score} and fig.~\ref{fig:indep_score}. With the increase of $K$, f-score results of all three methods increases as well for three different error types. The f-score results of CODED may reach $0.85$ when combination errors are inserted which is much larger than that of DBoost and DC, which are $0.42$ and $0.16$ separately. Generally CODED outperforms other two methods in all settings. This demonstrates that CODED is better to capture the errors in such setting. Notably, CODED employs $NK$ strategy to independence \SCs, which is averagely better than employing $K$ strategy to dependence \SCs. \na{Shall we discuss a little bit why NK is better than K?}One reason is that the errors are systematically generated, which will have equal influence over the entire dataset. This is more observed when coming to independence \SCs. Removing $N-K$ records according to the chosen hypothesis testing method, the rest $K$ records are more suspicious to be erroneous. 

However, CODED is not so stable as another two methods. CODED performs better when the errors are sorting error and combination error, where the average f-score is $0.6$ and highest f-score is around $0.8$. That will be decreased to average one $0.5$ and highest one $0.6$. The same reason also applies here. CODED is more powerful to detect the errors when the relationship implied by original \SCs are changed. If the influence of errors over the \SCs is minor, the power to detect the error will correspondingly decrease. As observed in exp-2, the influence of imputation error will not 

\noindent \underline{$A \indep B ~|~C$ and $A \nindep B ~|~C$.} We also examined the effectiveness of CODED compared to state-of-art methods under conditional independent and conditional dependent setting in moderate error level.  Results are very similar to the independence \SCs and dependence \SCs. Though tendency is similar, the level is a little bit lower compared to marginal ones. The best f-score of CODED, DBoost and DC are $0.72$, $0.49$, and $0.26$ separately. 

\noindent\textbf{\underline{Exp-5: Effectiveness on categorical dataset.}}We also examined the effectiveness on categorical dataset, where we use the CAR dataset. \emph{Selling price} and \emph{Maintenance price} are dependent, \emph{safety} and \emph{doors} are independent. We evaluated the performance of CODED and DBoost when inserting moderate level errors. Results are shown in fig.~\ref{fig:score_cat}. Since most of categorical data are oridinal, the sorting operation is not common in analyzing these data. As the result, we focus on the imputation errors in this experiment. \na{Change the statement before, default method for categorical dataset is $\chi^2$ test}. Both CODED and DBoost performs well in detecting the imputation error. The average f-score of CODED and DBoost are $0.45$ and $0.24$ respectively. Similar to the phenomena in exp-4, COEDE and DBoost both perform better under Independence \SCs setting.  

\noindent \textbf{\underline{Exp-6: Scalability.}} We evaluated the efficiency of top-$K$ strategy methods in a fast implementation described in Sec.~\ref{sec:drill-down}. Given that the worst-case time complexity of the FAST-CODED algorithm is $\mathcal{O}(k n \log n)$, intuitively the k-value and \# records will determine the actual time cost. We examined the performance of Fast-CODED varying $k$ and \# of records. Results are shown in Fig.~\ref{fig:scalability}. 

When conducting the experiment varying $K$, we set \# of records to be 10 thousand. It can be found that the execution time grows at a linear peace w.r.t. to the increase of K in fig.~\ref{fig:scalability}(a). As analyzed in Sec.~\ref{sec:drill-down}, the time complexity of $K$ strategy method is $\mathcal{O}(n \log n)$ for initialization, and is $\mathcal{O}(kn\log n)$ to pick up $K$ records. Under the normal setting of online analytics where $K=50$, CODED executes the query within 3 seconds. In the extreme setting that $K=200$, COEDE takes less than 8 seconds, which is pretty fast. The results is consistent with the complexity analysis. This demonstrates the scalability of FAST-CODED varying $K$. 

We further explore the scalability of Fast-CODED with different data size. It is obvious, based on the analysis above, the time cost is dominated by the size of datasize. Since we expected to use CODED to support the human-in-loop analysis in large-scale, we examined the efficiency when $K=50$ under different data size setting. In fig.~\ref{fig:scalability} (b), we can find that the increase of time follows the linear increase w.r.t. the increase of data size. Fast CODED takes less than 1 min (60 seconds) to process when there are 0.6 million records. And Fast CODED takes around 2 min where there are 1 million records. Therefore, FAST-CODED is possible to support human-in-loop analytic when employed for large-scale data. 

% \subsection{Scalability of Error Detection Method}



%impact of errors of different error types, including the sorting error and missing value.We evaluate the impact of errors injected varying different constraints. 


\noindent \textbf{\underline{Exp-7: Effectiveness on Real-world Dataset.}} In Exp-7, we examined the effectiveness of Real-world dataset on real-world dataset. 

\noindent\textbf{Sensor Dataset.} Since the location of sensors will determined by the surrounding temperature, neighboring sensors tend to report similar temperatures, which means these reported results shall be the dependent. Reversely, for those sensors that are far from each other are supposed to report different temperatures, which means these reports are independent. We chose sensors close to each other and construct the \SCs based on this.  Results are shown in fig.~\ref{fig:sensor}. It is noted that the precision is at least larger than $0.8$. CODED is able to detect errors at a 100\% percent ratio. More importantly, Sensor dataset contains more than one type of errors. From this experiment, we can conclude that CODED has the potential to detect combination of errors, which is more complex than that of single type. We leave the study of employing CODED to multiple types errors as the future work.

\noindent\textbf{Hockey Dataset.} \na{There are some problems with the Hockey dataset. We shall discuss whether we need to add it or not.}

\noindent \textbf{\underline{Summary}}



==> experiments__Jiannan_Wang_s_conflicted_copy_2018-04-29_.tex <==
\section{Experiments}\label{sec:exp}

% \begin{figure}[t]
%   \centering 
%   \includegraphics[scale=0.45]{fig/exp/scs_check/efficiency.eps} 
%   \vspace{-2em}
%   \caption{Time for Consistency Checking of \SCs (``0.5 Times'' means that the ) \label{fig:scs_check}\vspace{-2em}
% \end{figure}


\begin{table*}[h]\label{tab:con-summary}
 \centering
 \caption{Constraints Used by Different Error Detection Methods \jn{What about the constraints used by the Car dataset?}} 
 %\setlength\tabcolsep{3.5pt}
   \begin{tabular}{|c|c|c|}
   \hline
       \textbf{Attributes} & \textbf{CODED} & \textbf{Denial  Constraints} \\ \hline
   \hline
    Home Value(H), Black Index(B) & $H \indep B$ &  N/A\\ \hline
    N\_oxide(N), Distance(D) & $N \nindep D$ & \specialcell{}{For any two records, if N value of one is larger, \\ its D value shall be smaller than another one}\\ \hline
%     For any two records, if the N of one is larger, \\
%   \hline
  N, B, Tax rate (T) & $N \indep B ~|~T$ & N/A \\ \hline
  T, B, Crime(C) & $T \nindep B~ |~C$ & \specialcell{}{When $C = c$, For any two records, if T value of \\ one is larger, its B value shall be smaller than another one}\\ \hline
   \end{tabular}%
 \label{tbl:constraints}
\end{table*}%

\begin{figure}[t]
   \centering 
   \includegraphics[scale=0.36]{fig/exp/scs_check/efficiency_new.eps} 
   \vspace{-1em}
   \caption{Time for Consistency Checking of \SCs 
%   \oliver{should that be divided by 10?}\na{it will be congested}
   }\label{fig:scs_check}\vspace{-1em}
\end{figure}


\begin{figure}[t]
  \centering 
  \includegraphics[scale=0.5]{fig/exp/cat/var_k_cat.eps} 
  \vspace{-1em}
  \caption{Effectiveness of Error Detection Methods for  of Categorical dataset}\label{fig:score_cat}\vspace{-1em}
\end{figure}


\begin{figure}[t]
   \centering 
   \includegraphics[scale=0.23]{fig/exp/Scalability/Scalability.eps} 
   \vspace{-1em}
   \caption{Scalability of Fast CODED \SCs 
%   \oliver{is one quantity fixed in the other plot? e.g. K = ? for number of records?}\na{Yes, we gonna wirte these parts in the efficiency section}
   }\label{fig:scalability}\vspace{-1em}
\end{figure}



\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.39]{fig/exp/error_impact/error_impact_indep.eps} 
   \vspace{-2em}
   \caption{Different Error Impact on Independence \SCs}\label{fig:imp_indep}\vspace{-2em}
\end{figure*}



\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.39]{fig/exp/error_impact/error_impact_dep.eps} 
   \vspace{-2em}
   \caption{Different Error Impacts on Dependence \SCs.}\label{fig:imp_dep}
\end{figure*}



\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.6]{fig/exp/sync_files/var_k_dep.eps} 
   \caption{Effectiveness of Error Detection Methods for Dependence \SCs}\label{fig:dep_var_k}\vspace{-2em} \label{fig:dep_bar_chart}
\end{figure*}


\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.6]{fig/exp/sync_files/var_k_indep.eps} 
   \caption{Effectiveness of Error Detection Methods for Independence \SCs}\label{fig:indep_var_k}\vspace{-2em}\label{fig:indep_bar_chart}
\end{figure*}



\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.69]{fig/exp/sync_files/dep_var_k.eps} 
   \vspace{-1em}
   \caption{Effectiveness of Error Detection Methods for Dependence \SCs}\label{fig:dep_score}\vspace{-1em}
\end{figure*}


\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.69]{fig/exp/sync_files/indep_var_k.eps} 
   \vspace{-1em}
   \caption{Effectiveness of Error Detection Methods for Independence \SCs}\label{fig:indep_score}\vspace{-1em}
\end{figure*}


\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.69]{fig/exp/sync_files/dep_var_k_condition.eps} 
   \vspace{-1em}
   \caption{Effectiveness of Error Detection Methods for Conditional Dependence \SCs}\label{fig:dep_score_condition}\vspace{-1em}
\end{figure*}

\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.69]{fig/exp/sync_files/indep_var_k_condition.eps} 
   \vspace{-1em}
   \caption{Effectiveness of Error Detection Methods for Conditional Independence \SCs}\label{fig:dep_score_condition}\vspace{-1em}
\end{figure*}



\begin{figure*}[t]
   \centering 
   \includegraphics[scale=0.45]{fig/exp/real_world/real-world.eps}
   \vspace{-2em}
   \caption{Detecting Real-world Error in \emph{Sensor}\oliver{why the big difference in recall vs. precision? And what is precision?: Answer: we draw $K$ from a fixed number of error record, e.g. 400}}\label{fig:sensor}\vspace{-2em}
\end{figure*}


In this section, we evaluate the effectiveness and efficiency of our methods on real-life datasets with both synthetic errors and real errors. Specifically, we examined (1) the computational efficiency of the consistency-checking methods, (2) the effectiveness of our method compared to the state-of-the-art approaches on detecting synthetic and real-life errors, and (3) the scalability of our error-detection method.

%By these experiments, we examined  our algorithms, and discovered limitations  %of our methods for further improvement. 

\subsection{Experiment Setup}
\noindent \textbf{Datasets.} We used four real-life datasets to evaluate our approaches.

(1) {\tt BOSTON\footnote{\scriptsize https://www.cs.toronto.edu/~delve/data/boston/bostonDetail.html}.} The Boston dataset was taken from the Boston Standard Metropolitan Statistical Area (SMSA) in 1970. This dataset was first used in~\cite{Harvard} to study the relationship between clean air quality and household's willing to pay. There are 506 instances, and each instance has 14 attributes. We used *** attributes: Distance to CBD area (DT), Nitric Oxides Concentration (NR), and Crime Rate (CR). \jn{List all the attributes used in the experiment (see Table~\ref{tbl:constraints}). Also, please use the same abbreviations as Table~\ref{tbl:constraints}.}

(2) {\tt CAR\footnote{\scriptsize  https://archive.ics.uci.edu/ml/datasets/Car+Evaluation.}.} The Car Evaluation dataset is from UCI Machine Learning repository. This dataset contains seven attributes. We used *** attributes: buying price, maintainence price and safety level. \jn{List all the attributes used in the experiment.}

(3) {\tt SENSOR\footnote{http://db.csail.mit.edu/labdata/labdata.html}.} The Sensor dataset collected the sensor reports from the Berkeley/Intel Lab. The dataset has more than 2 million records, containing the humidity and temperature reports from 54 different sensors. %There are more than 2 million records in the dataset. This dataset~[???] has been widely used in data error detection, data repairing, and data curation.

(4) {\tt HOCKEY\footnote{https://github.com/liuyejia/Model\_Trees\_Full\_Dataset}}. The Hockey dataset collected the records of each NHL game from 1998-2010. It has more than ten attributes which variously describe player attributes and player performance statistics for a season. 
%the critical information of the game, player performance, and etc.

\vspace{.25em}


\noindent \textbf{Simulated Errors.} In Section~\ref{sec:intro}, we introduced two types of errors: \emph{sorting error} and \emph{imputation error} (see Figure~\ref{fig:car-error}). We simulated them on the Boston dataset. \jn{How about the Car dataset?}   


To simulate the \emph{sorting} error on column $A = \{a_1, a_2, \cdots, a_n\}$, we first select a sub-sequence of $A$, then sort them in an ascending order, denoted by $A' = \{a'_i, \cdots, a'_j\}$ ($a'_i \leq a'_{i+1} \leq \cdots \leq a'_j$). After that, we put the sorted values back to the original column, i.e., $\error{A} = \{a_1, \cdots, a_{i-1}, a'_i, \cdots, a'_{j}, a_{j+1}, \cdots, a_n\}$. We say that $\error{A}$ has sorting error with the error rate of $\frac{j-i+1}{n}$. 
Note that the sorting error may either make two columns $A$ and $B$ more independent or less independent. If the original data is randomly shuffled, then $\error{A}$ and $B$ tend to be more independent; if the original data is sorted by $B$, then $\error{A}$ and $B$ tend to be less independent. We used the former for dependence \SCs, the latter for independence \SCs. 


To simulate the imputation error on column $A = \{a_1, a_2, \cdots, a_n\}$, we assume that $A$ has a set of $m$ missing values (i.e., error rate = $\frac{m}{n}$), and the missing values are replaced by the mean value of column $A$. Let $\error{A}$ denote the new column. Like the sorting error, the imputation error may either make two columns more independent or less independent. If the missing values are randomly selected, $\error{A}$ and $B$ tend to become more independent; if the missing values are selected based on a range condition on $B$, $\error{A}$ and $B$ tend to become less independent. We used the former (latter) for dependence (independence) \SCs. 
\oliver{would be nice to have an example here}\na{TO JN: Shall we have an example here?} \jn{Yes. Create a figure, and in the figure, use a synthetic dataset with two columns A and B to illustrate the above four senarios.}

In addition, we explored the impact of combination of the two error types given that in practice, the combination of errors is not rare. We call it \emph{combination error}, which consists of 80\% sorting error and 20\% imputation error.  



%occurs when a data scientist sorted data points by one column to see the tendency but forgot to reverse the process. 
%The result is that one column is sorted but others remain random or same. We consider two sorting situations: (1) Single sorting: the data scientist just sorted one column and didn't revert it back; (2) she sorted the entire dataset by columb $b$, and then she further took a look at the order of column $a$; 

%which can not be matched with other column values. 
%Missing values  are ubiquitous. Usually data analysts choose one standard imputation method to fill in the missing value. However, these imputation methods sometimes introduce errors that violate statistical constraints. We consider an imputation method that fills in missing values with a constant, like the mean, maximum or minimum value. In our experimental evaluations, we choose the mean value for the imputation. 
%in the data consistent with the given dataset. T
%This error type is called ~\emph{Imputation} error. We examined the Sorting error and Imputation error. 

%In addition, we also explored the impact of combination of the two errors given that in reality, the combination of errors is not rare. 
%and bring more tough challenges. 

\vspace{.25em}

\noindent \textbf{Real-life Errors.} For the Sensor dataset, we first aggregated the mean value of sensor reports by hours.  Reported mean temperatures higher than 60 degrees or lower than 15 degrees were assumed to be erroneous~\cite{mayfield2010eracer}. We throwed away these values, and used mean value imputation to fill them in. We treated this processed dataset as the input dataset, and aimed to detect missing values and outliers on it. The missing values were the ones that were throwed away (as mentioned above). For the outliers, we adopted the method in~\cite{jeffery2006declarative} to define the ground truth. The method kept a time window of neighboring sensors: in this time window, the reports from sensors should not deviate by more than a factor of 3 from the region's mean value.


%We adopted the methods that~\cite{mayfield2010eracer} and~\cite{jeffery2006declarative} used to obtain the ground truth. First of all, we aggregated the mean value of sensor reports by hours. Reported mean temperatures larger than 60 degrees or lower than 15 degrees can be assumed to be erroneous.  We throw away these values, and use  mean value imputation to fill them in. Furthermore, we mark outliers by keeping a time window of neighboring sensors: in this time window, the reports from sensors should not deviate by more than a factor of 3 from the region's mean value. %By these steps, we define the ground truth errors for the sensor dataset. 

For the Hockey dataset, the dataset creators performed imputations to support machine learning analysis. The imputations are found by comparing their dataset with the original data from hockey data websites. A surprising finding is that those imputed values bias the machine-learning model. We aim to detect those imputed values. 

%There are many missing/empty entries in the original dataset, therefore we can easily get these ground truth. 

\vspace{.25em}

\noindent \textbf{Error-Detection Approaches.} We compared CODED with two state-of-the-art error detection approaches, Denial Constraints(DC)~\cite{chu2013discovering} and DBoost~\cite{mariet2016outlier}. Table~\ref{tbl:constraints} summarized the constraints used by CODED and DC.  For the CODED hypothesis testing, we used the $\chi^2$ test for categorical data, and the $\tau$ test for numerical data. We implemented the error-drill-down framework, and adopted the $K$ strategy for dependence \SCs and the $K^c$ strategy for independence \SCs. DC is a constraint based error detection approach. We counted the DC violations of each record, and returned the top-$k$ records that involve the most number of violations. DBoost is an outlier detection approach. We downloaded its code from the github~\footnote{\scriptsize}\jn{Add the link}. We set the mixture n$\_$subpops threshold to be $3, 0.001$ \jn{why does n$\_$subpops have two numbers?}, and the statistical epsilon to be $0$. 

%Table~\ref{tbl:constraints} summarized the constraints used by CODED and DC on different datasets.     




\vspace{.25em}

\noindent \textbf{Quality Measurement.} We used \emph{Precision@K}, \emph{Precision}, and \emph{Recall} to measure the quality of error-detection approaches. \emph{Precision} is the ratio of the number of correctly detected records to the number of total returned records,  \emph{Recall} is the ratio of the number of correctly detected records to the number of total erroneous records. \emph{Precision@K} is the precision among the \emph{k} returned records. 

 

\subsection{Experimental Results}
% \oliver{order of figures doesn't match discussion - is that deliberate?}
% \na{It can be fixed later easily.}
\noindent \textbf{\underline{{Exp-1: Efficiency of Consistency Checking.}}}
We examined the efficiency of the consistency-checking algorithm. Note that the consistency checking is {\em not} related to data. Therefore, randomly generating \SCs is appropriate to test the scalability of our %efficient 
consistency-checking algorithm. We randomly generated $|\mathcal{I}|$ independence \SCs and $|\mathcal{D}|$ dependence \SCs from $|\mathcal{D}|/2$ variables. We measured the runtime of consistency checking by varying $|\mathcal{I}|$ and $|\mathcal{D}|$, respectively. The results are shown in Figure~\ref{fig:scs_check}. Each figure has three lines, which represent different ratios of $|\mathcal{I}|$ to $|\mathcal{D}|$.


We make two interesting observations. First, our consistency-checking algorithm scales well by varying either $|\mathcal{I}|$ or $|\mathcal{D}|$. Even with 500 independence (dependence) \SCs, the algorithm can terminate within 0.5 ms. Second, the efficiency is more related to $|\mathcal{I}|$ than $|\mathcal{D}|$. This is because the consistency-checking algorithm proposed comprises two parts: implication and checking, where the implication algorithm needs $\mathcal{O}(|\mathcal{I}^2|)$ time, which typically dominates the whole process.


%The $x$-axis is the number of total constraints or variables, and the $y$-axis is the running time in 100 msec.

%\noindent \textbf{Random rules generation.} To study the efficiency of the consistency checking algorithms, we randomly generate rules for testing. It is worth attention that the consistency checking is {\em not} related to the data. Therefore, randomly generating rules is applicable for testing the scalability of efficient consistency checking approach. The efficiency of the consistency checking algorithm is determined by the \# of constraints, and the ratio between independent \SCs and dependent \SCs. Also, according to Lemma ~[,,,], the \# of attributes may increase computational cost. Therefore, we evaluated the following three different situations.


%\noindent \underline{\emph{Varying the \# of independent and dependent \SCs.}} Algorithmically, the \# of \SCs will dominate the time in computation. The consistency checking algorithm proposed comprises two parts: implication and checking. Different \# of independent \SCs and dependent \SCs can help reveal which type of \SCs and even which part of the algorithm needs more time computationally. 

%\noindent \underline{\emph{Varying the \# of attributes.}} Since the \# of attributes bounds the possible \SCs, it is also necessary to study the influence of \# of attributes. 

%\noindent \underline{\emph{Varying the ratio of independent \SCs and dependent \SCs.}}  We compared the ratio of independent \SCs and dependent \SCs. We want to examined the majoring influence while resolving the inconsistency.

%As shown in Fig.~\ref{fig:scs_check}, more \SCs lead to more processing time.  Interestingly,  the \# of independent ~\SCs has only a slight impact on run time (Fig.~\ref{fig:scs_check}a. In contrast, varying the \# of {\em dependent} \SCs has a dramatic impact, as does varying the number of attributes (Fig.~\ref{fig:scs_check}b and c). 
%Combine the two above, it can be inferred, the increase \# of \SCs and attributes, particularly the \# of independent \SCs will cost more computation time. 
%One principal reason is that the implication algorithm, which needs at most $|\mathcal{I}^*|$ where the $|\mathcal{I}^*|$ is the number of independent ~\SCs. Intuitively, the number of independent \SCs will afect the final result. 
 
\vspace{.25em}


\noindent \textbf{\underline{Exp-2: Impact of Errors.}}
To illustrate the impacts of data errors on independence and dependence relationships among variables, we varied the rates of sorting error, imputation error, and combination error, %respectively, 
and tested how the $\tau$ value changed accordingly. The results are shown in Figure~\ref{fig:imp_indep} and Figure~\ref{fig:imp_dep}.

Figure~\ref{fig:imp_indep} shows the results w.r.t. an independence \SC. Generally, all the errors tend to raise the tau value, indicating a violation of the independence \SC. The sorting error brings consistent side effects on the tau value (Figure~\ref{fig:imp_indep}(a)). Imputation error has a strong negative impact at lower error rates, then the tau value reverses (Figure~\ref{fig:imp_indep}(b)). This can be explained as follows. Starting with independent data, imputing a constant value induces correlations among the two columns. Once many data points have been imputed with a constant value, the correlation decreases until one column contains the same constant everywhere, implying zero correlation between them. 

Figure~\ref{fig:imp_dep} shows the results for a dependence \SC. We can see that as more errors were generated, the $\tau$ value decreased, i.e., the columns became more independent. With the error rate at 0.8, the $\tau$ value approached zero, indicating an independence relationship.   


%Figures~\ref{fig:imp_indep}(a) and (b) show that with small error rates, the $\tau$ value remained small (e.g., within [0,0.3]). While this may not violate an \SC, CODED can still detect errors accurately using the proposed error-drill-down framework. We will examine this result in the next experiment. 

%(see the results in the next experiment).

%ccor examined the impact of different type of errors, including the sorting error and missing value imputation. We mainly studied two types of errors: \emph{sorting} and ~\emph{poor missing value imputation}. We want to evaluate the impact of two errors and the whether default hypothesis test methods are sensitive to these errors.

%We evaluated the impact of different error types on the tau value, our default statistic for assessing statistical constraints on a dataset. 
% Tau value, the key statistics in the hypothesis testing~[???]. Tau value is able to show the correlation of the data. Therefore, with the increase of error rate, we evaluated the how influential the error impact could be in two different types of \SCs. 
%Noted that~\emph{not independent} indicates two situations: ~\emph{positive correlated} and ~\emph{negative correlated}. We also evaluated the error impact on both two situations. 


%Generally, all the errors tend to raise the tau value, indicating a violation of the statistical independence constraint. The sorting error brings consistent side effects on the tau value in among different ~\SCs (Fig.~\ref{fig:imp_indep} (a)) \oliver{what is rooms/black index?}. Imputation error has a strong negative impact at lower error rates, then the tau value reverses (Fig.~\ref{fig:imp_indep} (b)). This can be explained as follows. Starting with independent data, imputing a constant value induces correlations among the two columns, as many data points are assigned the same value for both. Once many data points have been imputed a constant value, the correlation decreases until both columns contain the same constant everywhere, implying zero correlation between them. 

%\noindent \textbf{Error types.} \emph{Sorting} error occurs when a data scientist sorted data points by one column to see the tendency but forgot to reverse the process. 
%manipulated the sorting operation on one column but didn't reverse the process. 
%The result is that one column is sorted but others remain random or same. We consider two sorting situations: (1) Single sorting: the data scientist just sorted one column and didn't revert it back; (2) she sorted the entire dataset by columb $b$, and then she further took a look at the order of column $a$; 

%which can not be matched with other column values. 
%Missing values  are ubiquitous. Usually data analysts choose one standard imputation method to fill in the missing value. However, these imputation methods sometimes introduce errors that violate statistical constraints. We consider an imputation method that fills in missing values with a constant, like the mean, maximum or minimum value. In our experimental evaluations, we choose the mean value for the imputation. 
%in the data consistent with the given dataset. T
%This error type is called ~\emph{Imputation} error. We examined the Sorting error and Imputation error. 

%In addition, we also explored the impact of combination of the two errors given that in reality, the combination of errors is not rare. 
%and bring more tough challenges. 




% negative impact which, however, is not as strong as the Sorting error. More obviously, in Fig.~\ref{fig:imp_indep} (b), the impact brings by Imputation is uneven in independent \SCs group. \oliver{b) looks weaker than a) at first. then it reverses. Needs more discussion.}

% Surprised thought this can be explained in this way: Take the ultimate situation as an example, we get all tied tuples which means all the tau value is equal to 0. The Imputation error works in that way since the imputed error are the same value, like the mean value, one random value or maximum value. Therefore, the same value finally will make the tau value to be 0. Starting from nearly perfect independent, and with the increase of  error rate, the tauv value would turn to be 0 again. Hence it is reasonable to conjecture such error will make the value to be less independent, however, be more independent eventually. 

%Another subtle explanation is that there is no positive independent or negative independent. Errors could make the dataset less independent: more positive correlated or negative correlated. Cancellation of errors will alleviate the impact brought. \oliver{needs review}

%For the combination errors, since the ratio of sorting error to Imputation error is 4:1, the sorting error effect dominates the Imputation effects.
% it is possibly that impact induced by missing value and errors dominated the error impact over the dataset. That explains why though the impact of Imputation error is not constant, the sorting error shields the shadow on the dataset. 


%In summary, the sorting error and Imputation error can induce correlations that violate independence constraints, and the tau statistic detects the violation.

% We examined the effectiveness of CODED compared to two baselines: DC-clean and DBoost. 

\vspace{.25em}

\noindent \textbf{\underline{Exp-3: Evaluation of Error-Detection Approaches.}} We compared CODED with existing error-detection methods on the Boston dataset for three types of errors. For dependence \SCs, we compared with Denial Constraint (DC) and DBoost; for independence \SCs, since DC cannot express independence relationships, we compared only with DBoost. We considered all four common templates of \SCs: (1) $A \indep B$; (2)$A \nindep B$; (3) $A \indep B~ | ~C$ ; (4) $A \nindep B ~|~ C$. Furthermore, the dependence and independence relationships among columns are from~\cite{Harvard}. 


% \oliver{nice}
% and a dependency model trained by ready probabilistic models. ,%\oliver{would be nice to make this more visual like a table}

%\na{To JN: do we need a table describing the meaning of selected columns?}

\noindent \underline{$A \indep B$ and $A \nindep B$.} We picked the \emph{Black Index} and \emph{N Oxide} from the Boston dataset since they are independent, we also picked \emph{Distance} and \emph{N Oxide} from Boston dataset as they are dependent.  \oliver{why only Boston?}\na{You think it is necessary to have more datasets in this section? We already have four datasets, one for simulate errors, one for categorical, and two for real-world. } We picked the \emph{Distance} and \emph{N Oxide} from the Boston dataset since they are dependent. Based on the observation, the error level can be grouped into three levels: \emph{minor error} where the ratio of errors varies from $1\%$ to $20\%$, \emph{moderate error} where the ratio of errors varies from $20\%$ to $45\%$, and \emph{major error}where the ratio of errors is usually larger than $50\%$. Results are shown in figure.~\ref{fig:dep_bar_chart} and figure.~\ref{fig:indep_bar_chart}.  Mostly, for all three methods, the precision increases as the error level increased. It is easy to understand, since when there is the large portion of errors, the dependence or independence relationship will be changed more dramatically, and it is easier for CODED and other methods to detect them. When there are minor errors, all three methods fail to detect them above precision$=0.5$ averagely. This implies when there are minor errors, the relationship defined by \SCs will not be changed so much. This means, the influence of entailed by these errors didn't dominate the original one. It is reasonable that all three methods didn't perform well under this setting. With the increase of errors, the precision of all three methods increases as well. For the error type, three methods perform better under sorting error and combination error, however, they are not that good in detecting error when the error is imputation error. This phenomena is more obvious when it come to CODED with conditional independent \SCs. In fig.~\ref{fig:indep_bar_chart} (b), we can find that all methods didn't perform well compared to other settings. \na{Do we need to explain why figure 9 (b) all methods doesn't perform well? It is like a dramatically down}. One reason is that influence aroused by imputation error was not always 

As recall describes the ratio of error detected in context of total errors. Given we set $K=50$, so the recall will naturally decrease with the increase with errors. That is the reason why recall keep going down when there are more simulated errors inserted. 

CODED outperforms both DC and DBoost in three different error levels, different error types and different \SCs. \na{Do we need to explain why other methods didn't perform well?}

Meanwhile, we also evaluate the effectiveness (f-score) varying the $K$ value to see how f-score changes under different $K$ values. Results are shown in fig.~\ref{fig:dep_score} and fig.~\ref{fig:indep_score}. With the increase of $K$, f-score results of all three methods increases as well for three different error types. The f-score results of CODED may reach $0.85$ when combination errors are inserted which is much larger than that of DBoost and DC, which are $0.42$ and $0.16$ separately. Generally CODED outperforms other two methods in all settings. This demonstrates that CODED is better to capture the errors in such setting. Notably, CODED employs $NK$ strategy to independence \SCs, which is averagely better than employing $K$ strategy to dependence \SCs. \na{Shall we discuss a little bit why NK is better than K?}One reason is that the errors are systematically generated, which will have equal influence over the entire dataset. This is more observed when coming to independence \SCs. Removing $N-K$ records according to the chosen hypothesis testing method, the rest $K$ records are more suspicious to be erroneous. 

However, CODED is not so stable as another two methods. CODED performs better when the errors are sorting error and combination error, where the average f-score is $0.6$ and highest f-score is around $0.8$. That will be decreased to average one $0.5$ and highest one $0.6$. The same reason also applies here. CODED is more powerful to detect the errors when the relationship implied by original \SCs are changed. If the influence of errors over the \SCs is minor, the power to detect the error will correspondingly decrease. As observed in exp-2, the influence of imputation error will not 

\noindent \underline{$A \indep B ~|~C$ and $A \nindep B ~|~C$.} We also examined the effectiveness of CODED compared to state-of-art methods under conditional independent and conditional dependent setting in moderate error level.  Results are very similar to the independence \SCs and dependence \SCs. Though tendency is similar, the level is a little bit lower compared to marginal ones. The best f-score of CODED, DBoost and DC are $0.72$, $0.49$, and $0.26$ separately. 

\noindent\textbf{\underline{Exp-5: Effectiveness on categorical dataset.}}We also examined the effectiveness on categorical dataset, where we use the CAR dataset. \emph{Selling price} and \emph{Maintenance price} are dependent, \emph{safety} and \emph{doors} are independent. We evaluated the performance of CODED and DBoost when inserting moderate level errors. Results are shown in fig.~\ref{fig:score_cat}. Since most of categorical data are oridinal, the sorting operation is not common in analyzing these data. As the result, we focus on the imputation errors in this experiment. \na{Change the statement before, default method for categorical dataset is $\chi^2$ test}. Both CODED and DBoost performs well in detecting the imputation error. The average f-score of CODED and DBoost are $0.45$ and $0.24$ respectively. Similar to the phenomena in exp-4, COEDE and DBoost both perform better under Independence \SCs setting.  

\noindent \textbf{\underline{Exp-6: Scalability.}} We evaluated the efficiency of top-$K$ strategy methods in a fast implementation described in Sec.~\ref{sec:drill-down}. Given that the worst-case time complexity of the FAST-CODED algorithm is $\mathcal{O}(k n \log n)$, intuitively the k-value and \# records will determine the actual time cost. We examined the performance of Fast-CODED varying $k$ and \# of records. Results are shown in Fig.~\ref{fig:scalability}. 

When conducting the experiment varying $K$, we set \# of records to be 10 thousand. It can be found that the execution time grows at a linear peace w.r.t. to the increase of K in fig.~\ref{fig:scalability}(a). As analyzed in Sec.~\ref{sec:drill-down}, the time complexity of $K$ strategy method is $\mathcal{O}(n \log n)$ for initialization, and is $\mathcal{O}(kn\log n)$ to pick up $K$ records. Under the normal setting of online analytics where $K=50$, CODED executes the query within 3 seconds. In the extreme setting that $K=200$, COEDE takes less than 8 seconds, which is pretty fast. The results is consistent with the complexity analysis. This demonstrates the scalability of FAST-CODED varying $K$. 

We further explore the scalability of Fast-CODED with different data size. It is obvious, based on the analysis above, the time cost is dominated by the size of datasize. Since we expected to use CODED to support the human-in-loop analysis in large-scale, we examined the efficiency when $K=50$ under different data size setting. In fig.~\ref{fig:scalability} (b), we can find that the increase of time follows the linear increase w.r.t. the increase of data size. Fast CODED takes less than 1 min (60 seconds) to process when there are 0.6 million records. And Fast CODED takes around 2 min where there are 1 million records. Therefore, FAST-CODED is possible to support human-in-loop analytic when employed for large-scale data. 

% \subsection{Scalability of Error Detection Method}



%impact of errors of different error types, including the sorting error and missing value.We evaluate the impact of errors injected varying different constraints. 


\noindent \textbf{\underline{Exp-7: Effectiveness on Real-world Dataset.}} In Exp-7, we examined the effectiveness of Real-world dataset on real-world dataset. 

\noindent\textbf{Sensor Dataset.} Since the location of sensors will determined by the surrounding temperature, neighboring sensors tend to report similar temperatures, which means these reported results shall be the dependent. Reversely, for those sensors that are far from each other are supposed to report different temperatures, which means these reports are independent. We chose sensors close to each other and construct the \SCs based on this.  Results are shown in fig.~\ref{fig:sensor}. It is noted that the precision is at least larger than $0.8$. CODED is able to detect errors at a 100\% percent ratio. More importantly, Sensor dataset contains more than one type of errors. From this experiment, we can conclude that CODED has the potential to detect combination of errors, which is more complex than that of single type. We leave the study of employing CODED to multiple types errors as the future work.

\noindent\textbf{Hockey Dataset.} \na{There are some problems with the Hockey dataset. We shall discuss whether we need to add it or not.}

\noindent \textbf{\underline{Summary}}



==> old-versions/detection-long.tex <==
\section{Detecting SCs violations}~\label{sec:detection}
% \na{One Example with Running example to show how do we use SCs to detect violations.}
% \na{To Oliver, We may need to compare with Pearson Tests}
% In this section, we show how do we use the Independence Test methods with Statistical Constrains to detect the violations among Columns. We first formally introduce the independence testing methods (Sec. ~\ref{intro}), and then we show how to apply independence testing to detect violations of statistical constraints (Sec. ~\ref{detect}). 

Evaluating whether a dataset satisfies an independence constraint is a classic application of statistical hypothesis testing. Hypothesis testing is an extensively developed area of statistics that is well covered in a number of sources \cite[Ch.10]{bib:wasserman}. To make the paper self-contained, we will briefly review the basic ideas. A \defterm{hypothesis test} $\test$ is a procedure that takes as input a dataset $\dset$ and outputs either 0 (``the hypothesis is rejected") or 1 (``the hypothesis is not rejected"). In classic scientific methodology, a deterministic hypothesis is rejected if it is inconsistent with the data. 
%To adapt this idea to the setting with probabilistic predictions,  a
A statistical hypothesis is rejected when, the probability of the data entailed by the hypothesis is below a user-specified threshold. In principle, a hypothesis test can be any type of procedure. In practice, for analytic and computational tractability, most tests are based on test statistics. A \defterm{test statistic} $\statistic{\dset}$ returns a real number for a given data set. Intuitively, the statistic is an aggregate function that summarizes the degree to which the dataset violates the hypothesis. The test therefore rejects the hypothesis if the statistic is sufficiently high: $\test(\dset)=0 \iff \statistic{\dset} > c$, where the \defterm{critical value} $c$ is a threshold parameter of the test. For a given independence  hypothesis $\set{\Xvariable} \indep \set{\Yvariable} | \set{\Zvariable}$, a test $\test$ for the hypothesis commits a false negative (type I error) on a dataset $\dset$ if $\set{\Xvariable} \indep \set{\Yvariable} | \set{\Zvariable}$ is true and $\statistic{\dset} > c$. We wish to bound a false negative error below a user-defined \defterm{significance level} $\significance$ such that $  P(\statistic{\dset} > c_{\significance}|\set{\Xvariable} \indep \set{\Yvariable} | \set{\Zvariable})<\significance$, where critical value $c_{\significance}$ is chosen to achieve the desired significance level $\significance$. 

% \begin{equation} \label{eq:significance}
%     P(\statistic{\dset} > c_{\significance}|\set{\Xvariable} \indep \set{\Yvariable} | \set{\Zvariable})<\significance
% \end{equation} 

A significance level test outputs one bit of information, whether the independence hypothesis should be rejected given the data or not. While this is the purpose of a test, we can provide more information to a user by specifying the {\em degree} to which the data disconfirm an independence hypothesis. An easily interpretable way to convey this information is the probability that, assuming the independence hypothesis were true, the deviation $d$ from independence measured by the null hypothesis would be as great as actually observed, or greater. This quantity is called the \defterm{$p$-value}: $ p({\dset}) = P(t \geq \statistic{\dset}|\set{\Xvariable} \indep \set{\Yvariable} | \set{\Zvariable})$.

% \begin{equation} \label{eq:p-value}
%     p({\dset}) = P(t \geq \statistic{\dset}|\set{\Xvariable} \indep \set{\Yvariable} | \set{\Zvariable})
% \end{equation} 

The $p$-value can also be viewed as the lowest false negative error bound $\significance$ such that if the user were to specify $\significance$, the test would reject the independence hypothesis. For example, if the $p$-value is $3\%$, this means that the test would reject the independence hypothesis for any significance level $\significance \geq 3\%$. Therefore the computation of the test result can be reduced to the computation of $p$-values: Given a $p$-value for a dataset, reject the independence hypothesis if and only if $p(\dset) \leq \significance$. For example, if the user specifies a significance level of $5\%$, and the $p$-value for a dataset is $3\%$, we can reject the independence hypothesis. 



{\em Computing $p$-values.} 
To find a $p$-value, we need to determine the conditional distribution of the test statistic, given that the independence hypothesis is true. Ideally this distribution follows one of the standard uni-variate distributions (e.g. a Gaussian or $\chi^2$ distribution) for which libraries exist. For independence tests, such test statistics are usually not available. However, it is possible to prove for many test statistics that they {\em asymptotically} follow a standard distribution, meaning that as the dataset grows larger and larger, the conditional distribution of Equation~\eqref{eq:p-value} is increasingly well approximated by a library distribution. This approximation is usually sufficiently close to be used even on medium-size samples. 
Which test statistics are suitable for independence hypotheses depends on the data type. In the following we evaluate how well standard test statistics and their approximating distributions perform for the task of data error detection.

%for a threshold $c$ called the critical value:

% To define this formally, let $\region_{T}: \{\dset:\test(\dset)=0\}$ be the datasets for which the test rejects the hypothesis. We omit the subscript $\test$ when context makes clear which test is referred to. For a given independence  hypothesis $\set{\Xvariable} \indep \set{\Yvariable} | \set{\Zvariable}$, a test $\test$ for the hypothesis commits a false negative (type I error) on a dataset $\dset$ if $\set{\Xvariable} \indep \set{\Yvariable} | \set{\Zvariable}$ is true and $\dset \in \region_{T}$. We wish to bound this error below the \defterm{significance level} $\significance$ such that $$P(\dset \in \region_{T}|\set{\Xvariable} \indep \set{\Yvariable} | \set{\Zvariable}) \leq \significance.$$ 
% %Defining a test procedure with this guarantee poses substantial mathematical and computational difficulties. 
% A standard approach is to define a \defterm{test statistic} $\statistic{\dset}$ that returns a real number for a given data set. Intuitively, the statistic is an aggregate function that summarizes the degree to which the dataset violates the hypothesis. The test therefore rejects the hypothesis if the statistic is sufficiently high, for a threshold $c$ called the critical value: $\test(\dset)=0 \iff \statistic{\dset} > c$. The critical value $c_{\significance}$ is chosen to achieve the desired significance level $\significance$:





\subsection{Independence Testing Methods}~\label{intro}

We describe independence tests only for unconditional independence $set{\Xvariable} \indep \set{\Yvariable}$. In the case where the conditioning variable set $\set{\Zvariable}$ is discrete, the unconditional test is applied for each setting $\set{\Zvariable} = \set{z}$. \oliver{nathan: is this right?} 

\subsubsection{Discrete Variables} Given an assignment $\set{\Xvariable} = \set{\xvalue}$, each datapoint satisfies the assignment or not. The \textbf{observed count} is the number $N_{\dset}(\set{\Xvariable} = \set{\xvalue})$ of datapoints that satisfy it. Thus the observed counts for complete assignments are denoted by $N_{\dset}(\set{\Xvariable} = \set{\xvalue},\set{\Yvariable} = \set{\yvalue})$. If the sets $\set{\Xvariable}$ and $\set{\Yvariable}$ were completely independent, the observed counts would equal the product of the marginal counts; these are called the \textbf{expected counts}: $E_{\dset}(\set{\Xvariable} = \set{\xvalue},\set{\Yvariable} = \set{\yvalue}) \equiv N_{\dset}(\set{\Xvariable} = \set{\xvalue}) \times N_{\dset}(\set{\Yvariable} = \set{\yvalue}).$

Test statistics for independence among discrete variables measure the difference between expected and observed counts. The \textbf{G-statistic} computes the log-difference over all possible assignments, where each log-difference is weighted by how often the observed count: $G(\dset) \equiv 2 \sum_{\set{\xvalue},\set{\yvalue}} N_{\dset}(\set{\Xvariable} = \set{\xvalue},\set{\Yvariable} = \set{\yvalue}) \times \ln(\frac{N_{\dset}(\set{\Xvariable} = \set{\xvalue},\set{\Yvariable} = \set{\yvalue})}{E_{\dset}(\set{\Xvariable} = \set{\xvalue},\set{\Yvariable}= \set{\yvalue})})$。

The chi-square statistic $\cstat$ sums the squared differences, weighted inversely to the expected counts:

$\cstat(\dset) \equiv  \sum_{\set{\xvalue},\set{\yvalue}} \frac{[N_{\dset}(\set{\Xvariable} = \set{\xvalue},\set{\Yvariable} = \set{\yvalue}) - E_{\dset}(\set{\Xvariable} = \set{\xvalue},\set{\Yvariable}= \set{\yvalue})]^2}{E_{\dset}(\set{\Xvariable} = \set{\xvalue},\set{\Yvariable}= \set{\yvalue})}$

Pearson introduced the chi-square statistic in 1900, as a practical approximation to the G-test, because computing logarithms was challenging then. The distribution of both the G and the chi-square statistic can be approximated by the $\chi^2$ distribution, whose probability density function for positive $t$ is given by $\chi_{k}^2(t) = \frac{1}{2^{k/2}\Gamma(k/2)} t^{k/2-1}e^{-x/2}.$

Here $k$ is a distribution parameter known as the degrees of freedom. In an independence test, we have $k = (r_{X}-1) \times (r_{Y}-1) $ where $r_X$ resp. $r_Y$ is the number of possible values for $X$ resp. $Y$. We can therefore compute the p-value for an observed G-statistic $G(\dset)$ as $p({\dset}) = \int_{G(\dset)}^{+\infty} \chi_{k}^2(t) dt$

where $k$ is set as described; similarly for an observed chi-square statistic $Q(\dset)$. The chi-square statistic is named after the $\chi^2$ distribution but should not be confused with it. In fact, the G-statistic is more closely approximated by the $\chi^2$ distribution than the chi-square statistic is, and so modern textbooks recommend using the G rather than the chi-square test. 

\subsubsection{Continuous Variables} 

We discuss independence tests for two continuous variables $\Xvariable$ and $\Yvariable$. 
For continuous variables, each exact value occurs typically only once in the data, so there are  no discrete counts to compare. Instead, independence tests consider the degree to which $\Xvariable$ and $\Yvariable$ vary together: whether an increase in $\Xvariable$ tends to correspond to an increase or decrease in $\Yvariable$. A number of different formulas have been developed for capturing this idea. Perhaps the best known is Pearson's correlation coefficient $\rho$. The correlation coefficient measures the degree to which $\Xvariable$ and $\Yvariable$ are linearly related. The disadvantage of the $\rho$ statistic is that it is reliable only under certain assumptions, including that the relationship between $\Xvariable$ and $\Yvariable$ is approximately linear. In fact, it is possible to have $\Yvariable$ be a deterministic (but nonlinear) function of $\Xvariable$ with 0 Pearson correlation. Since in the error detection problem, we have very little a priori knowledge of the exact form of the statistical dependence between $\Xvariable$ and $\Yvariable$, we examine statistical tests that make minimal assumptions about the nature of the dependence. In statistics, such tests are called {\em non-parametric}, since they do not assume that the dependence can be characterized by a fixed set of parameters known a priori before data observation. 

A well-established set of non-parametric tests for dependence are known as \defterm{rank correlations}. Rank correlations are based on a straightforward intuition, which makes them easy to interpret for a user: Each variable defines an ordering over data points, and if the variables are associated, the $\Xvariable$-ordering should carry information about the $\Yvariable$-ordering. In our car running example, if the most expensive car is also the most fuel-efficient, the second-most expensive car is the second-most fuel-efficient, ..., and the cheapest car is the least fuel-efficient, then there is a positive relationship between price and fuel efficiency. A rank correlation test therefore considers only how similar the $\Xvariable$-ranking is to the $\Yvariable$-ranking, and the not magnitude of the differences between different data points. The problem of detecting a probabilistic association is therefore reduced to deciding the similarity of two rankings. A number of similarity metrics for rankings have been proposed; these can be unified in a general formula known as the general correlation coefficient. Two of the most popular instances of the general correlation coefficient are Kendall's $\tau$ and Spearman's rank correlation metrics. Spearman rank correlation computes the Pearson correlation between the $\Xvariable$-ranks and the $\Yvariable$-ranks (rather than the Pearson correlation between the $\Xvariable$-values and the $\Yvariable$-values). This still assumes the existence of a linear relationship among ranks, whereas Kendall's $\tau$ is truly non-parametric without any assumptions about the functional form of the association among ranks. We therefore employ $\tau$ in our experiments. \oliver{1) do we need to show the general correlation coefficient. 2) anythign about other rank correlation coefficients like Mann-Whitney or Wilcoxon? Wilcoxon is used a lot in machine learning.} The definition of $\tau$ is as follows. 

Consider $n$ datapoints with two features $\dset= (\xvalue_1,\yvalue_1)\ldots,(\xvalue_n,\yvalue_n)$. Consider two datapoints $(\xvalue_i,\yvalue_i)$ and $(\xvalue_j,\yvalue_j)$ with $i \neq j$. There are three possibilities.

\begin{enumerate}
    \item $\xvalue_i > \xvalue_j$ and $\yvalue_i > \yvalue_j$, or $\xvalue_i < \xvalue_j$ and $\yvalue_i < \yvalue_j$. In this case the two variables agree on the ordering of $i$ and $j$ and the pair $(i,j)$ is \defterm{concordant}. 
    The number of concordant pairs is denoted as $n_c(\dset)$.
    \item $\xvalue_i > \xvalue_j$ and $\yvalue_i < \yvalue_j$, or $\xvalue_i < \xvalue_j$ and $\yvalue_i > \yvalue_j$. In this case the two variables disagree on the ordering of $i$ and $j$ and the pair $(i,j)$ is \defterm{discordant}. 
    The number of discordant pairs is denoted as $n_d(\dset)$.
    \item $\xvalue_i = \xvalue_j$ (the pair is tied in $X$) or $\yvalue_i = \yvalue_j$ (the pair is tied in $Y$). The number of pairs tied in $\Xvariable$ resp. $\Yvariable$ is denoted by $n_X(\dset)$ resp. $n_Y(\dset)$.
\end{enumerate}

The intuition behind the $\tau$ statistic is that it represents the difference in the proportion of concordant pairs and the proportion of discordant pairs. So it is a function of $n_{c} - n_{d}$, divided by an appropriate normalization constant that depends on the distribution of ties. The $\tau$ statistic is then computed as $\tau(\dset) \equiv \frac{n_c(\dset) - n_d(\dset)}{\sqrt{v(\dset)}}$, where $v(\dset)=\left(\binom{n}{2}-n_{X}(\dset)\right) \left(\binom{n}{2}-n_Y(\dset)\right)$.
% Let $t_{i}^{\Xvariable}$ be the number of ties in the $i$-th group of ties for $\Xvariable$, and similarly  $t_{j}^{\Yvariable}$ for the $j$-th tie group of $\Yvariable$. 

% Notice that the total number of pairs is given by

% \[
% \binom{n}{2} = n_c + n_d + n_X + n_Y + n_{XY}
% \]

% where $n_c$ is the number of concordant pairs, $n_d$ the number of discordant pairs, $n_X$ $(n_Y)$ the number of pairs tied only in $X$ ($Y$), and $n_{XY}$ the number of pairs tied in both. 


% $v(\dset)=\left(\binom{n}{2}-\sum_i \binom{t_i^{\Xvariable}}{2}\right) \left(\binom{n}{2}-\sum_j \binom{t_j^{\Yvariable}}{2}\right) $
% \[
% \tau(\dset) \equiv \frac{n_c - n_d}{\sqrt{(n_c + n_d + n_X) (n_c + n_d + n_Y)}}.
% \]

Notice that the denominator depends only on each variable separately, so the association between $\Xvariable$ and $\Yvariable$ is represented solely by the $n_c(\dset) - n_d(\dset)$ difference.
The distribution of $\tau$ under the independence hypothesis is difficult to determine analytically. To compute $p$-values, one can compute a rescaled version of the $\tau$ statistic as $z(\dset) \equiv \frac{n_c(\dset) - n_d(\dset)}{\sqrt{v'(\dset)}}$,
where $v'$ is a  function of $n_X$ and $n_Y$ carefully scaled to ensure that $z$  has a standard normal distribution $N(0,1)$ with mean 0 and variance 1. 
\oliver{find a real source for Kendall tau test}
For a given dataset, a $p$-value can therefore be computed as $p({\dset}) = \int_{|z(\dset)|}^{+\infty} \frac{\exp(-t^2/2)}{\sqrt{2\pi}} dt.

\iffalse
\subsection{Example: Detecting Violations with Statistical Constraints}~\label{detect}

  

==> scs-old.tex <==
\section{Statistical Constraints}

\quad In this section, we fist present a running example which will be used in following sections(Section \ref{example}). We formally define the constraints with mathematical expressions (Section \ref{scd}) and use the running example to illustrate(Sec \ref{illustration}).

\subsection{Running Example}\label{example}
In this paper, we used the dataset \emph{sensor} collected the readings from 54 sensors deployed in the Intel Lab (Now RISE Lab) for 38 consecutive days. The schema is as follows:

\noindent \texttt{\emph{\textbf{sensor}}(date, time, epoch,	moteid,	temperature, humidity, light, voltage)}

\oliver{Oliver: some semantics would be  helpful, perhaps an ER diagram. e.g. I don't know what a `"moteid`" is . Also a small example table. See eracer page.}

To extract Statistical Constraints from \emph{sensor}, we also leveraged the location information of the sensors, the schema of the location file is as follows:

%\noindent \texttt{\emph{\textbf{location}}(xcoordinates, y_coordinates, moteid)}


\noindent \texttt{\emph{\textbf{location}}(moteid1, moteid2, distance)}

In the following paper, we run some queries in order to extract Statistical Constraints from \emph{sensor}.



\subsection{Background Definitions}\label{scd}

\oliver{I suggest we define random variables so they closely follow columns. Given our title. Also we can be more succinct here. I'm starting to rewrite}



A \defterm{variable} $\Xvariable$ is an attribute or feature that can be assigned a value $\xvalue$ from a fixed domain; we write $\Xvariable = \xvalue$ to denote an assignment of a value to a variable. We use boldface vector notation for finite sets of objects. So for example $\set{\Xvariable} = \set{\xvalue} \equiv (\Xvariable_1 = \xvalue_1,\Xvariable_2 = \xvalue_2, \ldots, \Xvariable_n = \xvalue_n)$ denotes the \defterm{joint assignment} of variable $\Xvariable_i$ is assigned value $\xvalue_i$, for each $i=1,\ldots,n$. In relational terms, a variable corresponds to a non-primary key attribute or column, and joint assignments to tuples. \oliver{should we have translation table here so they don't miss this point?}

A \defterm{random variable} requires a distribution $P(\Xvariable = \xvalue)$ that assigns a probability to each domain value in the domain of $\Xvariable$. A \defterm{joint distribution} $P(\set{\Xvariable} = \set{\xvalue})$ assigns a probability to a vector of values, one for each variable in the list $\set{\Xvariable}$. In the following, we often abbreviate the probability assignment $P(\set{\Xvariable} = \set{\xvalue}) \equiv P(\set{\xvalue})$ when the relevant set of variables is clear from context.


Given a joint distribution for a set of variables $\set{\Xvariable}$, the \defterm{marginal distribution} over a subset $\set{\Yvariable}$ is defined by $$P(\set{\Yvariable}=\set{\yvalue}) \equiv \sum_{\set{\zvalue}} P(\set{\Yvariable}=\set{\yvalue},\set{\Zvariable}=\set{\zvalue}).$$ Here $\set{\Zvariable} = \set{\Xvariable}- \set{\Yvariable}$ contains the set of variables outside of $\set{\Yvariable}$, and the comma notation $\set{\Yvariable}=\set{\yvalue},\set{\Zvariable}=\set{\zvalue}$ denotes the conjunction of two joint assignments. Here and elsewhere in this paper, the summation applies to variables with discrete domains, and should be replaced by integrals for variables with continuous domains. The \defterm{conditional probability} of an assignment $\set{\Xvariable} = \set{\xvalue}$ given another assignment $P(\set{\Yvariable}=\set{\yvalue}$ is defined as 

$$P(\set{\Xvariable} = \set{\xvalue}|\set{\Yvariable}=\set{\yvalue}) \equiv P(\set{\Xvariable} = \set{\xvalue},\set{\Yvariable}=\set{\yvalue})/P(\set{\Yvariable}=\set{\yvalue}).$$

A key notion of this paper is the concept of {\em conditional independence among sets of variables.} Intuitively, a set of variables $\set{\Xvariable}$ is independent of another set $\set{\Yvariable}$ given a third conditioning set $\set{\Zvariable}$ if knowing the values of the variables in $\set{\Yvariable}$ adds no information about the values of the variables in $\set{\Xvariable}$, beyond what can be inferred from the values in the set $\set{\Zvariable}$. Formally, for three disjoint sets $\set{\Xvariable}, \set{\Yvariable}, \set{\Zvariable}$  we define 

\begin{eqnarray*}
\set{\Xvariable} \indep \set{\Yvariable} | \set{\Zvariable} & \equiv & \\ P(\set{\Xvariable}=\xvalue,\set{\Yvariable}=\yvalue|\set{\Zvariable} = \zvalue) & = \\ P(\set{\Xvariable}=\xvalue|\set{\Zvariable}=\zvalue) \times P(\set{\Yvariable}=\yvalue|\set{\Zvariable} = \zvalue) & \mbox{for all } \xvalue, \yvalue, \zvalue
\end{eqnarray*}

This definition assumes that $P(\set{\Zvariable} = \set{\zvalue} > 0$ for all possible values $\set{\zvalue}$. 
\oliver{should we define independence in terms of conditional probabilities?}
\oliver{should we discuss context-sensitive independence here?}
The negation of a conditional independence is a conditional dependence, written $\set{\Xvariable} \nindep \set{\Yvariable} | \set{\Zvariable}$. Thus conditional dependence holds if for {\em some} values $\set{\xvalue},\set{\yvalue},\set{\zvalue}$, we have $P(\set{\Yvariable} = \set{\yvalue}|\set{\Zvariable} = \zvalue)>0$ and $P(\set{\Xvariable}=\xvalue|\set{\Yvariable}=\yvalue,\set{\Zvariable} = \zvalue) \neq P(\set{\Xvariable}=\xvalue|\set{\Zvariable} = \zvalue)$.

% Fix a set of random variables $\set{\node} = \{\node_{1},\ldots,\node_{n}\}$. 


\quad Consider $\Omega=\{\omega_1, \omega_2,\omega_3,...\}$ as the set of all possible outcome events. We consider each random variable as a mapping $X: \Omega \to \mathbb{R}$  that assigns a real number $X(\omega)$ to each outcome $\omega$. 

\begin{Definition}[probability distribution]
	A function $\mathbb{P}$ that assigns a real number to $\mathbb{P}(A)$ to each event $A$ is a \textbf{probability distribution} or a \textbf{probability measure} where $A \in \Omega$. $\mathbb{P}(A)$ is the probability of $A$.
\end{Definition}

The probability distribution satisfies the three axioms: (1) 
$\mathbb{P}(A)\geq 0$ for every $A$; (2) $\mathbb{P}(\Omega)=1$; (3) If $A_1, A_2, ...$ are disjoint, then, $P(\bigcup_{\infty}^{i=1})=\sum_{i=1}^{\infty}\mathbb{P}(A_i)$.  Since the random variable is the mapping function, we can also write the probability distribution as $\mathbb{P}(X)$.  And its \textbf{probability function} is $p_X{(x)}=\mathbb{P}(X=x)$.
\vspace{1em}

Let $p(x)$ and $p(y)$ be probability  function of the $X$ and $Y$ from the attributes set $U=\ {}$respectively, and $p(x,y)$ as the joint probability function of$(X,Y)$. We assume $Z$ as a further variable. In the following part, we are to introduce independent constraints, dependent constraints and statistical constraints. 

%Statistical constraints $S$ is composed of two set: the Dependence set $D$ and the Independence $I$, that is $S=D\cup I$. 
\subsection{Independence and Dependence Constraints}

Our main idea in this paper is to detect data quality problems by finding contradictions with domain knowledge supplied by the user in the form of dependence and independence constraints. Such statistical constraints have several advantages. 1) {\em Interpretability.} They are easily interpreted by the user as relevance or irrelevance between attributes. Although the probabilistic semantics of a statistical constraint refers to quantitative probability distribution, specifying an (in)dependence constraint does not require the user to specify or consider numeric values. The large field of graphical models is based on the insight that (in)dependence constraints can be represented in terms of purely qualitative graphical relations among variables. 2) {\em Detectability.} The field of statistical hypothesis testing has developed many methods, built up over a century, for deciding whether a given data set violates an independence constraint. These methods provide parameters for controlling false positive and false negative error rates. 3) {\em Expressive power.} Deterministic constraints such as functional dependencies are powerful but also limited in the relationships among attributes that they allow a user to express. In contrast, many important facts about a domain can be expressed as statistical (in)dependencies among attributes. 

\begin{Definition}[Independent Constraints]Independent Constraints refer to independent relationship among variables, and are composed of two independent relationship: \textbf{marginal} independent and \textbf{conditional} independent. We use $I$ to denote the Independent Constraints. 
\vspace{.5em}

\textbf{Marginal independent.} We use  $ X~\indep~Y$  as $I(X,\varnothing,Y)$ to denote that $X$ and $Y$ are marginal independent. Mathematical expression is
\begin{equation}
	p(x,y) = p(x)p(y). 
\end{equation}
	
\textbf{Conditional independent.} We use  $ X~\indep~Y$  as $D(X,\varnothing,Y)$ to denote that $X$ and $Y$ are marginal dependent. Mathematical expression is
\begin{equation}
	p(x,y) \neq p(x)p(y). 
\end{equation}

\end{Definition}

\begin{Definition}[Dependent Constraints]Independent Constraints refer to dependent relationship among variables, and are composed of two dependent relationship: \textbf{marginal} dependent and \textbf{conditional} dependent.  In this paper, we use $D$ to denote the Dependent Constraints.    
\vspace{.5em}
	
\textbf{Marginal dependent.} We use  $ X~\indep~Y~ |~Z $  as $I(X,Z,Y)$ to denote that $X$ and $Y$ are conditional independent given $Z$. Mathematical expression is
\begin{equation}
	p(x,y~|~z) \neq p(x~|~z)p(y~|~z)
\end{equation}
	
\textbf{Conditional dependent.}  We use  $ X~\indep~Y~|~Z$  as $D(X,Z,Y)$ to denote that $X$ and $Y$ are conditional dependent given $Z$. Mathematical expression is
\begin{equation}
	p(x,y~|~z) \neq p(x~|~z)p(y~|~z).
\end{equation}
\end{Definition}
	
Based on the equations from (1) to (4), we can easily find that the relationship $D$ is the counter relationship to $I$. Therefore, the $\neg D(X,Y,Z) = I(X,Y,Z)$. 
%Based on the definition of \textbf{independent constraints} and \textbf{dependent constraints}, it is easy to find that they are not compatible for the same variable. 
\begin{Theorem}[Complementary Relationship]
	Given the Independent Constraints set $Is$ and Dependent Constraints set $Ds$, $Ds^c \cap Is = \emptyset$.
\end{Theorem}

Then we formally introduce the definition of Statistical Constraints. 


 \begin{Definition}[Statistical Constraints]
  Given the attribute set $U=\{X,Y,Z,...\}$ dataset $D$, Statistical Constraints(SCs) over $U$ are both independent constraints and dependent constraints over $U$. Given the Statistical Constraints set $\Sigma$, it can be expressed as $\Sigma = Is \cup Ds$, where $Is$ and $Ds$ are Independent Constraints set  and Dependent Constraints set of $\Sigma$.
%  Let $X$, $Y$ and $Z$ be the random variables. The independent constraints set $Is$ among them and the Dependent constraints set $Ds$ among them are the \textbf{Statistical Constraints} $$. Therefore, the set of statistical constraints can be written as $\Sigma = Is \cup Ds$.
 \end{Definition}
    
    
Please note in this paper, we investigate the statistical constraints among two or three variables which is based on the observations of the real world dataset. We further show that our method can be extended for any relationship among variables in the experiment part.  
    
    
%    
%    $X~\indep~Y$
%    
%    $X~\indep~Y~|~Z$
%    
%    
%    $ X~\indep~Z~|~W$
%    
%    $X~\indep~Z~|~Y$，$ X~\indep~Z~$
%    
%    
%    $X~\indep~Y~|~Z$, $X~\indep~Y$
%    
%   $ X~\indep~Z~$, $X~\indep~Z~|~Y$
%    
%
%    $ X~\indep~Z~$
%    
%    
%    $X~\indep~Z~|~W$
%    
%    $ X~\nindep~Z~$
    
  

   
   \subsection{Example illustration}\label{illustration}
   We use the running example to give the examples of the Statistical Constraints. 
   
   \oliver{Notes: 1) try running example from hockey dataset. for both dependence and independence. 2) learn a bayesian network for hockey data to visualize correlations. 3) Running example should cover going from independence to dependence}
   
   \begin{example}
   	  Dependent
   \end{example}
  
  
   \begin{example}
    Marginal Independent
  \end{example}

    \begin{example}
	 Conditional Independent
   \end{example}



==> scs.tex <==
\section{Statistical Constraints}\label{sec:sc}
In this section, we provide some background definitions, and a formal definition of statistical constraints. We describe how \system leverages \SCs for error-detection.


\subsection{Background Definitions}\label{scd}

A \defterm{variable} $\Xvariable$ is an attribute or feature that can be assigned a value $\xvalue$ from a fixed domain; we write $\Xvariable = \xvalue$ to denote an assignment of a value to a variable. We use boldface vector notation for finite sets of objects. So for example $\set{\Xvariable} = \set{\xvalue} \equiv (\Xvariable_1 = \xvalue_1,\Xvariable_2 = \xvalue_2, \ldots, \Xvariable_n = \xvalue_n)$ denotes the \defterm{joint assignment} where variable $\Xvariable_i$ is assigned value $\xvalue_i$, for each $i=1,\ldots,n$. In relational terms, a variable corresponds to an attribute or column, and a joint assignments to a tuple or row. 

% \oliver{should we have translation table here so they don't miss this point?}

% \na{To Oliver: what do you mean by translation table here? Can you give me one example, so I can draw one?}

A \defterm{random variable} requires a distribution $P(\Xvariable = \xvalue)$ that assigns a probability to each domain value in the domain of $\Xvariable$. A \defterm{joint distribution} $P(\set{\Xvariable} = \set{\xvalue})$ assigns a probability to each joint assignment.
%a vector of values, one for each variable in the list $\set{\Xvariable}$. 
We often abbreviate the probability assignment $P(\set{\Xvariable} = \set{\xvalue}) \equiv P(\set{\xvalue})$ when the relevant set of variables is clear from context.

Given a joint distribution for a set of variables $\set{\Xvariable}$, the \defterm{marginal distribution} over a subset $\set{\Yvariable}$ is defined by $$P(\set{\Yvariable}=\set{\yvalue}) \equiv \sum_{\set{\zvalue}} P(\set{\Yvariable}=\set{\yvalue},\set{\Zvariable}=\set{\zvalue}).$$ Here $\set{\Zvariable} = \set{\Xvariable}- \set{\Yvariable}$ contains the set of variables outside of $\set{\Yvariable}$, and the comma notation $\set{\Yvariable}=\set{\yvalue},\set{\Zvariable}=\set{\zvalue}$ denotes the conjunction of two joint assignments. Here and elsewhere in this paper, the summation applies to variables with discrete domains, and should be replaced by integrals for variables with continuous domains. The \defterm{conditional probability} of an assignment $\set{\Xvariable} = \set{\xvalue}$ given another assignment $P(\set{\Yvariable})=\set{\yvalue}$ is defined as
%
$$P(\set{\Xvariable} = \set{\xvalue}|\set{\Yvariable}=\set{\yvalue}) \equiv P(\set{\Xvariable} = \set{\xvalue},\set{\Yvariable}=\set{\yvalue})/P(\set{\Yvariable}=\set{\yvalue}).$$

A key notion of this paper is the concept of {\em conditional independence among sets of variables.} Intuitively, a set of variables $\set{\Xvariable}$ is independent of another set $\set{\Yvariable}$ given a third conditioning set $\set{\Zvariable}$ if knowing the values of the variables in $\set{\Yvariable}$ adds no information about the values of the variables in $\set{\Xvariable}$, beyond what can be inferred from the values in the set $\set{\Zvariable}$. Formally, for three disjoint sets $\set{\Xvariable}, \set{\Yvariable}, \set{\Zvariable}$  we define %
%
\begin{eqnarray*}
\set{\Xvariable} \indep \set{\Yvariable} | \set{\Zvariable} & \equiv & \\ P(\set{\Xvariable}=\xvalue,\set{\Yvariable}=\yvalue|\set{\Zvariable} = \zvalue) & = \\ P(\set{\Xvariable}=\xvalue|\set{\Zvariable}=\zvalue) \times P(\set{\Yvariable}=\yvalue|\set{\Zvariable} = \zvalue) & \mbox{for all } \xvalue, \yvalue, \zvalue
\end{eqnarray*}

This definition assumes that $P(\set{\Zvariable} = \set{\zvalue}) > 0$ for all possible values $\set{\zvalue}$. 

% \oliver{should we define independence in terms of conditional probabilities?}

% \na{To Oliver: I think we need to define them accordingly.}

% \oliver{not sure what you mean but let's hold off for now}

%\oliver{should we discuss context-sensitive independence here?}

%\na{To Oliver: Maybe we don't have to talk about it here? context-sensitive independence is for the explanation of errors. }

%\oliver{ok let's hold off for now and see if we need it later}

We call $\set{\Xvariable} \indep \set{\Yvariable} | \set{\Zvariable}$ a \defterm{(conditional) independence statement}. The negation of a conditional independence statement is a \defterm{(conditional) dependence statement}, written $\set{\Xvariable} \nindep \set{\Yvariable} | \set{\Zvariable}$. Thus conditional dependence holds if for {\em some} values $\set{\xvalue},\set{\yvalue},\set{\zvalue}$, we have $P(\set{\Yvariable} = \set{\yvalue}|\set{\Zvariable} = \zvalue)>0$ and $$P(\set{\Xvariable}=\xvalue|\set{\Yvariable}=\yvalue,\set{\Zvariable} = \zvalue) \neq P(\set{\Xvariable}=\xvalue|\set{\Zvariable} = \zvalue).$$

% \na{To Oliver, do we need to talk a few more things about conditional independent for continuous variables?}



%Statistical constraints $S$ is composed of two set: the Dependence set $D$ and the Independence $I$, that is $S=D\cup I$. 
\subsection{Statistical Constraints}\label{subsec:sc}

A set of Statistical Constraints (\SCs) comprises a set of independence statements and dependence statements. 

\begin{Definition}[Statistical Constraints] Fix a set of variables $\varset = \{V_1,\ldots,V_n\}$. A finite set of statistical constraints $\Sigma = \IC \cup \DC$ comprises
	\begin{enumerate}
		\item a finite set of independence \SCs, $\IC = \{\phi_1,\ldots,\phi_p\}$, where each $\phi_i$ is of the form $\set{\Xvariable} \indep \set{\Yvariable} | \set{\Zvariable}$, and
		\item a finite set of dependence \SCs, $\DC = \{\lambda_1,\ldots,\lambda_q\}$, where each $\lambda_i$ is of the form $\set{\Xvariable} \nindep \set{\Yvariable} | \set{\Zvariable}$ 
	\end{enumerate}
\end{Definition}

Please note in this paper, we investigate the statistical constraints among two or three variables.
%which is based on the observations of the real world dataset. 
We will extend our approaches to more than three variables in the future work.
%
% \na{To Oliver: do we need to specify that I and U cannot have the intersection?}
%
The main idea of this paper is to detect data quality problems by finding contradictions with domain knowledge supplied by the user in the form of dependence and independence constraints. Such statistical constraints have several advantages. 

\vspace{.25em}

\noindent \textbf{Interpretability.} (In)dependencies are easily interpreted by the user as ir(relevance) among attributes. %As Turing award winner Judea Pearl has stated: ``The mind has evolved to use conditional independence as the most stable way to represent knowledge about the external world." 
Although the probabilistic semantics of a statistical constraint refers to a quantitative probability distribution, specifying an (in)dependence constraint does not require the user to specify or even consider numeric values. The large field of graphical models is based on the insight that (in)dependence constraints can be represented in terms of purely qualitative graphical relations among variables~\cite{pearl2}. 

\vspace{.25em}

\noindent \textbf{Detectability.} The field of statistical hypothesis testing has developed many methods
%, built up over a century, 
for deciding whether a given data set violates an independence constraint~\cite{wasserman2013all}. These methods provide parameters for controlling false positive and false negative error rates.

\vspace{.25em}

\noindent \textbf{Expressive power.} Deterministic constraints such as functional dependencies are powerful but also limited in the relationships among attributes that they allow a user to express. Often they reflect definitions and data recording conventions. In contrast, many important empirical facts about a domain can be expressed as statistical (in)dependencies among attributes. The next section considers the relationship between statistical and integrity constraints in some detail.


\subsection{Integrity vs Statistical Constraints}\label{subsec:ic-vs-sc}
%\na{Shall we incorporate this part into the paper?}
Despite differences in tradition and terminology, integrity and statistical constraints often share underlying intuitions. Generally, integrity constraints enforce Boolean conditions on {\em sets} (relations), whereas statistical constraints impose (in)equalities on (conditional) {\em distributions}.  For example, a functional constraint $\set{X} \rightarrow Y$ entails an independence constraint $\set{X}  \indep Y | \set{X} - \{Y\}$.
% where $\set{Z}$ is the set of variables (columns) outside of $\set{X}$ and $Y$. 
Whereas the functional constraint says that the variables $\set{X}$ determine a unique {\em value} for $Y$ regardless of the $\set{Z}$ values, the independence constraint says that the variables $\set{X}$ determine a unique {\em distribution} for $Y$ regardless of the $\set{Z}$ values. For another example, a marginal independence constraint $X  \indep Y$ entails a {\em multi-valued dependency} between columns $X$ and $Y$~\cite{fagin1977multivalued}. Unlike integrity constraints, the traditional application of statistical constraints is to sample data, where we expect statistical constraints to hold only approximately with exceptions. As will be discussed in Section~\ref{sec:detection}, this is accomplished by defining {\em degrees of dependence} (e.g. correlations in (0,1]). %, in addition to the Boolean \SC concept of dependence. 
%Thus statistical theory provides a strong body of results for defining approximately satisfied constraints in a principled way. %\oliver{I think Jiannan wanted to discuss denial constraints too. Maybe it's true that a denial constraint implies a rank correlation of -1?}


\subsection{CODED Architecture}\label{subsec:sys-arch}
\begin{figure}[t]
   \centering
   \includegraphics[width=1\linewidth]{fig/coded.pdf} \vspace{-1em}
   \caption{\system Architecture}\label{fig:coded}
\end{figure}

Figure~\ref{fig:coded} shows the architecture of our  \SC-based error-detection system.
%whose architecture is depicted in . 
The system consists of three key components: \emph{consistency checking}, \emph{hypothesis testing}, and \emph{error drill down}. In the following, we present an overview of each component. 


\begin{figure}[t]
   \centering
   \includegraphics[width=0.8\linewidth]{fig/running-example.pdf} \vspace{-1em} 
   \begin{align*}
       & \SC_1 = \textsf{Model} \indep \textsf{Color} & & \SC_2 = \textsf{Fuel} \indep \textsf{Model}\\
       & \SC_3 = \textsf{Price} \indep \textsf{Fuel} \mid \textsf{Model}  &  & \SC_4 = \textsf{Price} \nindep \textsf{Fuel}
   \end{align*}\vspace{-1em}
   \caption{ A Running Example ($\SC_2$ could be removed. The highlighted cells are the data errors detected by \system w.r.t. $\SC_4$.). }\label{fig:running-example}%\vspace{-1em}
\end{figure}

%\oliver{move footnote to future work}

\vspace{.25em}


{\noindent \bf Consistency Checking.} \system takes a set of \SCs and a dirty dataset as input. It first checks whether the given \SCs are consistent or not. If not, it helps the user to resolve the conflict. For example, consider the four \SCs in Figure~\ref{fig:running-example}. As will be explained in Section~\ref{cck}, they are actually inconsistent, i.e., $\SC_2$ and $\SC_3$ implies $\textsf{Price} \indep \textsf{Fuel}$, which contradicts $\SC_4$. \system first tells the user that $\{\SC_1, \SC_2, \SC_3, \SC_4\}$ are inconsistent, and then guides the user to resolve the conflict, e.g., removing $\SC_2$.       



\vspace{.5em}

{\noindent \bf Hypothesis Testing.} Once a set of consistent \SCs are obtained, the system enters the hypothesis-testing stage. In this stage, the system checks for each \SC, whether the dataset violates the \SC or not. For example, consider $SC_1 = \textsf{Model} \indep \textsf{Color}$ and the dataset in Figure~\ref{fig:running-example}. The user expects that $\textsf{Model}$ and $\textsf{Color}$ should have an independent relationship. However, a $\chi^2$ hypothesis test on the data indicates that $\textsf{Model}$ and $\textsf{Color}$ are highly correlated. The system will mark $\textsf{Model}$ and $\textsf{Color}$ as erroneous columns. Section~\ref{sec:detection} below discusses hypothesis testing process.     


\vspace{.5em}

{\noindent \bf Error Drill Down.} A user may want to  drill down into individual records so that she can understand why an \SC is violated. Therefore \system provides an error-drill-down component. The user chooses a violated \SC and specifies a threshold $k$. This component aims to return $k$ records that are most likely to cause the \SC's violation. Suppose $\SC_2 = \textsf{Price} \nindep \textsf{Fuel}$ is violated. As will be shown in Section~\ref{sec:drill-down}, if the user specifies $k = 1$, the system will return $r_4$, which is a cheap car with high fuel consumption. The user can examine this record and may find out that unlike the other cars, this is a used car. It is worth noting that given $\SC_4$ the user does not need to write a handcrafted rule like \emph{a cheaper car tends to be more fuel-efficient}.
%because this can be inferred from the joint distribution for \textsf{Price} and \textsf{Fuel}. OS: I found this a bit hard to understand so I cut down on detail. E.g. is the "joint distribution" the data distribution? But the data are dirty right?

% More details will be presented in later sections.


%In the following, we will describe the system architecture and walk through the whole system using an example.



%We further show that our method can be extended for any relationship among variables in the experiment part. 

% \na{To JN: do we need to an example on three variable limits thing?} 
    
    
%    
%    $X~\indep~Y$
%    
%    $X~\indep~Y~|~Z$
%    
%    
%    $ X~\indep~Z~|~W$
%    
%    $X~\indep~Z~|~Y$，$ X~\indep~Z~$
%    
%    
%    $X~\indep~Y~|~Z$, $X~\indep~Y$
%    
%   $ X~\indep~Z~$, $X~\indep~Z~|~Y$
%    
%
%    $ X~\indep~Z~$
%    
%    
%    $X~\indep~Z~|~W$
%    
%    $ X~\nindep~Z~$

==> tmp.tex <==
\subsection{Efficient Implementation}\label{subsec:impl}

\begin{table}[h]
 \centering\small
 \caption{Supported data types and default hypothesis testing methods}
 %\setlength\tabcolsep{3.5pt}
   \begin{tabular}{|m|m|m|m|}
   \hline
       \textbf{X} & \textbf{Y} & \textbf{Z} & \textbf{Default Methods} \\
   \hline
      \hline
   Categorical & Categorical  & / & $\chi^2$ Test\\
   \hline
   Categorical & Categorical  & Categorical & $\chi^2$ Test \\
   \hline
   Numerical & Numerical & / & $\tau$ Test  \\
   \hline
    Numerical & Numerical & Categorical &  $\tau$ Test\\
   \hline
   
   \end{tabular}%
 \label{tab:exp_cph}
\end{table}%


As mentioned in Section~\ref{sec:detection}, there are a large number of hypothesis testing methods proposed in the statistics literature. We dive into two of them: $\chi^2$ test and Kendall's $\tau$ test, and discuss how to implement the K strategy efficiently\footnote{The same implementation can be extended to the NK strategy trivially.}.  Table ~\ref{tab:exp_cph} illustrates their supported data type. We defer an extensive discussion of the other hypothesis testing methods to future work.  %However, it is worth attention that CODED can easily extend to support other data types with the chosen hypothesis test methods by users. 

%In this paper, we focus showing how we employ Kendall's $\tau$ test, G-test and $\chi^2$ testing to locate erroneous records. However, CODED can support a wide range of hypothesis testing methods.

 \begin{figure}[t]
   	\centering
   	\includegraphics[scale=0.36]{fig/car_cat.pdf}
   	\caption{Co-occurrence between car model and car color}\label{fig:car_cat}
\end{figure}

\vspace{0.25em}

\noindent \textbf{Error Detection for Categorical Data.} We use $\chi^2$ to detect errors for categorical data. We propose an optimization technique to reduce the time of selecting the ``best'' record at each iteration. The key observation is that if two records have the same values on the tested columns, there is no difference to choose either one of them. Therefore, we can group the records based on the tested columns, and only need to spend time in deciding which group (rather than which record) should be selected at each iteration. 

For example, consider an \SC: $\textsf{\small Model} \indep \textsf{\small Color}$. We first group the records based on the tested columns (i.e., $\textsf{\small Model}$ and $\textsf{\small Color}$). Suppose there are 3 car models and 4 colors. Then, there will be 12 groups in total. Figure~\ref{fig:car_cat} illustrates the 12 groups where the number in each cell represents the total number of the records that belong to that group. At each iteration, the K strategy only needs to determine which group should be selected and then randomly pick up one record from that group. This optimization technique can significantly reduce the computational cost since the number of groups is typically orders of magnitude smaller than the total number of records. 


\vspace{0.25em}

\noindent \textbf{Error Detection for Numerical Data.} We use Kendall's $\tau$ test to detect errors for numerical data. We find that the main computational bottleneck of the $K$ strategy is on the initialization phase. Consider a dataset with two columns: $D = \langle x_1, y_1 \rangle, \cdots, \langle x_n, y_n\rangle$. We need to initialize the number of concordant (discordant) pairs for each record. For a single record, it requires comparing with the other $n-1$ records, thus leading to a time complexity of $\mathcal{O}(n)$. Since there are $n$ records, a naive implementation of the initialization phase needs $\mathcal{O}(n^2)$ time. For example, suppose there are 1 million records. Then, it requires $\mathcal{O}(10^{12})$ time, which is highly expensive. 

We find that the time complexity of the initialization phase can be reduced to $\mathcal{O}(n \log{n})$ with the help of a segment tree. A segment tree is a tree data structure, where each node stores information about a segment. It allows for inserting a segment and querying a segment with both $\mathcal{O}(\log{n})$ time. To apply this idea, we first sort $D$ by column $X$ and then scan the records in $D$ based on this new order. For each record $\langle x_i, y_i \rangle$, we can get the number of concordant pairs of the record by querying the segment of $(-\infty, y_i)$, and the number of discordant pairs by querying the segment of $(y_i, +\infty)$. Once the two numbers are obtained, we insert a segment $[y_i, y_i]$ to the tree. We need $\mathcal{O}(\log{n})$ time to process each record, thus the total time complexity is $\mathcal{O}(n \log{n})$. With this optimization, the error-drill-down framework can easily handle a dataset with millions of records.     




%\noindent\emph{Data types supported.} Fig.~\ref{fig:data_type} illustrates the data type that can be supported by our default hypothesis testing methods so far.  However, it is worth attention that CODED can easily extend to support other data types with the chosen hypothesis test methods by users. 

%In this paper, we focus showing how we employ Kendall's $\tau$ test, G-test and $\chi^2$ testing to locate erroneous records. However, CODED can support a wide range of hypothesis testing methods.

\iffalse

\subsection{Error Detection for Categorical Data}~\label{num}


In this section, we study how we employ CODED to detect erroneous records in categorical dataset. The default methods that recommended are $G$ test and $\chi^2$ testing. Classical methods try to use a likelihood based statistics to verify whether the relationship among columns violates the relationship implied by \SCs. In reality, the distribution of the co-occurrence between two columns which are supposed to imply the dependent \SCs will be skewed if there are some rare co-occurrences entailed by erroneous records. This means these unusual records will cause these records to be unmoral, and the likelihood statistics will be dominated by that combination term. Therefore, for the categorical dataset, we are more interested in detecting unusual co-occurrences.  The final step is we return Top-$k$ results to users, please be reminded Top-$k$ results here means the combination of tuples instead of the tuples themselves. 



The idea of detecting erroneous combinations in categorical dataset is intuitive: we projecting the impact of all combinations to statistics $S$ ouput by the chosen hypothesis testing method. As mentioned in Sec.~\ref{sec:detection}, we deploy $G$ test or $\chi^2$ test as default tests. Since $S = \sum_{i=1}^{n} {s_i}$ where $n$ is the number of combination, and $s_i$ is normalized, we simply just sort $s_i$ by order. Computational steps can be found in Algorithm.~\ref{alg:top_k_cat}. 

Consider the car example in Fig. ~\ref{fig:car-error}: \emph{Model} and \emph{Color}. We pictured the entire dataset as shown in Fig.~\ref{fig:car_cat}, and two attributes comprise several domain values, $Model = \{BMW, Audi, Benz\}$, $Color=\{White, Black, Red, Blue\}$,. If we simply construct the Function dependency  $F_1: Model \rightarrow Color$, many false positive results will be detected as they violate $F_1$. However, Consider one Statistical Constraint $SC_1: Model \indep Color$. Employing our default method $\chi^2$ testing method, we can easily see whether the relationship implied by data is inconsistent with the natural relationship $SC_1$. In this example, CODED takes the result in Fig.\ref{fig:car_cat} and $\chi^2$ testing as input, and the detection results is that the data implied correlation is against the $SC_1$. The user further takes a look at $S $ and wants to return Top-$3$ suspicious combination, then $S_{BMW, Black}, S_{BMW, Blue}, S_{BMW, red}$ will returned. 


\begin{algorithm}[t]
	\caption{Top-$k$ Error Detection for Categorical Data}\label{alg:top_k_cat}
	\KwIn{Columns: $col_a, col_b$ , Hypothesis Test Method: $T$, $k$}
	\KwOut{Queue $Q$: $k$ combination(s)}
	\vspace{0.2em}
	$Q\leftarrow\emptyset$ \;
	$s_i = H (col_a, col_b)$ \;
	Add each $s_i$ to $Q$ \;
	Sort $Q$ \;
	Keep first $k$ combinations of $Q$\;
	{\bf return} $Q$\;
\end{algorithm}



\subsection{Error Detection Problem for Numerical Data}
In this section, we detailed discuss how we solve the $K$ error problem and $NK$ error problem for numerical data.

As discussed in Sec.~\ref{sec:detection}, we have several hypothesis testing method to measure the correlation between columns. 

\begin{Definition}[Top-$k$ Kendall $\tau$ Based Error Detection]Given dataset $D$, $r_i$ 
	\begin{equation*}
	\begin{aligned}
	& \underset{r_i,r_j \in N^*, N^* \subset D, i<j\leq|N^*|}{\text{maximize}}
	& & |\frac{\sum{\mathds{1}(r_i,r_j)}}{\frac{N^*\cdot(|N^*|-1)}{2}} \cdot v|\\
	& \text{subject to}
	& &N^*=|D|-k
	\end{aligned}
	\end{equation*}
\end{Definition}



\begin{Lemma}[NP-hardness]
    Top-k Error Detection Problem using Kendall's $\tau$ test is a NP-hard problem
\end{Lemma}


\begin{proof}
\na{Finish the proof}
\end{proof}

\noindent \textbf{Negativity Attributed Graph Transformation}
\begin{equation*}
\begin{aligned}
& n_c + n_n + n_t = T \\
& \text{to max:~} ~ n_c-n_n  \\
& \text{replace~}~ n_c~ \text{~by~} ~n_t \\
& n_c-n_n = n_c-(T-n_t-n_c) \\
& n_c-n_n = 2n_c+n_t-T \\
& \text{where}~T= \frac{N\cdot(|N|-1)}{2}
\end{aligned}
\end{equation*}

\noindent \textbf{Greedy Algorithm}

\noindent \textbf{Efficient Implementation}

\noindent \emph{Remark} Compare with Denial Constraints

\subsection{Summary}

\fi
